White-Box Analysis over Machine Learning: Modeling Performance of Configurable Systems

Performance-influence models can help stakeholders understand how and where configuration options and their interactions influence the performance of a system. With this understanding, stakeholders can debug performance behavior and make deliberate configuration decisions. Current black-box techniques to build such models combine various sampling and learning strategies, resulting in tradeoffs between measurement effort, accuracy, and interpretability. We present Comprex, a white-box approach to build performance-influence models for configurable systems, combining insights of local measurements, dynamic taint analysis to track options in the implementation, compositionality, and compression of the configuration space, without relying on machine learning to extrapolate incomplete samples. Our evaluation on 4 widely-used, open-source projects demonstrates that Comprex builds similarly accurate performance-influence models to the most accurate and expensive black-box approach, but at a reduced cost and with additional benefits from interpretable and local models.

==> bibliography.tex <==
% Encoding: UTF-8

@String{ACM           = {ACM}}
@String{ACMAddr       = {New York, NY, USA}}
@String{ACMPress      = {ACM Press}}
@String{AOSD          = {Proc. Int'l Conf. Aspect-Oriented Software Development (AOSD)}}
@String{ASE           = {Proc. Int'l Conf. Automated Software Engineering (ASE)}}
@String{ASPLOS        = {Proc. Int'l Conf. Architectural Support for Programming Languages and Operating Systems (ASPLOS)}}
@String{AWL           = {Addison-Wesley}}
@String{AWLAddr       = {Boston, MA, USA}}
@String{CACM          = {Commun. ACM}}
@String{CHI           = {Proc. Conf. Human Factors in Computing Systems (CHI)}}
@String{CSCW          = {Proc. Conf. Computer Supported Cooperative Work (CSCW)}}
@String{ENHI          = {Elsevier North-Holland, Inc.}}
@String{ENHIAddr      = {Amsterdam, The Netherlands}}
@String{ESECFSE       = {Proc. Europ. Software Engineering Conf. Foundations of Software Engineering (ESEC/FSE)}}
@String{FOSE          = {Proc. Future of Software Engineering (FOSE)}}
@String{FSE           = {Proc. Int'l Symp. Foundations of Software Engineering (FSE)}}
@String{GPCE          = {Proc. Int'l Conf. Generative Programming and Component Engineering (GPCE)}}
@String{ICCPS         = {Proc. Int'l Conf. Cyber-Physical Systems (ICCPS)}}
@String{ICRS          = {Proc. Int'l Reliable Software}}
@String{ICSE          = {Proc. Int'l Conf. Software Engineering (ICSE)}}
@String{ICSME         = {Proc. Int'l Conf. Software Maintance and Evolution (ICSME)}}
@String{ICSR          = {Proc. Int'l Conf. Software Reuse (ICSR)}}
@String{IEEE          = {IEEE}}
@String{IEEEAddr      = {Los Alamitos, CA, USA}}
@String{IEEEAddrW     = {Washington, DC, USA}}
@String{IEEECSP       = {IEEE Computer Society Press}}
@String{IEEEPressAddr = {Piscataway, NJ, USA}}
@String{IEEESoftware  = {IEEE Softw.}}
@String{ISSTA         = {Proc. Int'l Symp. Software Testing and Analysis (ISSTA)}}
@String{ITHINGS       = {Proc. Int'l Conf. Internet of Things (iThings)}}
@String{MIT           = {MIT Press}}
@String{MITAddr       = {Cambridge, MA, USA}}
@String{MSR           = {Proc. Int'l Conf. Mining Software Repositories}}
@String{OOPSLA        = {Proc. Int'l Conf. Object-Oriented Programming, Systems, Languages and Applications (OOPSLA)}}
@String{PLDI          = {Proc. Conf. Programming Language Design and Implementation (PLDI)}}
@String{POPL          = {Proc. Symp. Principles of Programming Languages (POPL)}}
@String{RE            = {Proc. Int'l Requirements Engineering Conf. (RE)}}
@String{SCAM          = {Proc. Int'l Conference Source Code Analysis and Manipulation (SCAM)}}
@String{SCP           = {Sci. Comput. Program.}}
@String{SIGPLANNOT    = {SIGPLAN Notices}}
@String{SIGSOFTNotes  = {SIGSOFT Softw. Eng. Notes}}
@String{SoSyM         = {Softw. Syst. Model. (SoSyM)}}
@String{SPLC          = {Proc. Int'l Software Product Line Conference (SPLC)}}
@String{SV            = {Springer-Verlag}}
@String{SVBAddr       = {Berlin/Heidelberg, Germany}}
@String{SVNJAddr      = {Secaucus, NJ, USA}}
@String{SVNY          = {Springer-Verlag New York, Inc.}}
@String{SVNYAddr      = {New York, NY, USA}}
@String{TOSEM         = {ACM Trans. Softw. Eng. Methodol. (TOSEM)}}
@String{TSE           = {IEEE Trans. Softw. Eng. (TSE)}}
@String{VAMOS         = {Proc. Workshop Variability Modeling of Software-Intensive Systems (VAMOS)}}

@Book{B:DDECS10,
        title     = {The Design of Design: Essays from a Computer Scientist},
        publisher = {Addison-Wesley Professional},
        year      = {2010},
        author    = {Brooks, Frederick P.},
        edition   = {1st},
        }

@Book{FSWGGLLKKNS:ULSSSCF06,
        title     = {Ultra-Large-Scale Systems: The Software Challenge of the Future},
        publisher = {Software Engineering Institute, Carnegie Mellon University},
        year      = {2006},
        author    = {Feiler, Peter and Sullivan, Kevin and Wallnau, Kurt and Gabriel, Richard and Goodenough, John and Linger, Richard and Longstaff, Thomas and Kazman, Rick and Klein, Mark and Northrop, Linda and Schmidt, Douglas},
        }

@Book{S:SA96,
        title     = {The Sciences of the Artificial (3rd Ed.)},
        publisher = MIT,
        year      = {1996},
        author    = {Simon, Herbert A.},
        address   = MITAddr,
        }

@Book{SBN:CS87,
        title     = {Computer structures: principles and examples},
        publisher = {McGraw-Hill},
        year      = {1987},
        author    = {Siewiorek, Daniel P. and Bell, C. Gordon and Newell, Allen},
        series    = {McGraw-Hill computer science series},
        chapter   = {2, Levels and Abstraction},
        }

@Book{BW:TAOSA2,
        title     = {The Architecture of Open Source Applications, Volume II},
        publisher = {Kristian Hermansen},
        year      = {2012},
        author    = {Brown, Amy and Wilson, Greg},
        number    = {v. 2},
        series    = {The Architecture of Open Source Applications},
        }

@Book{BW:TAOSA1,
        title     = {The Architecture of Open Source Applications, Volume I},
        publisher = {CreativeCommons},
        year      = {2011},
        author    = {Brown, Amy and Wilson, Greg},
        number    = {v. 1},
        series    = {The Architecture of Open Source Applications},
        }

@Book{CBBGILMNS:DSA02,
        title     = {Documenting Software Architectures: Views and Beyond},
        publisher = {Pearson Education},
        year      = {2002},
        author    = {Clements, Paul and Felix, Bachmann and Bass, Len and Garlan, David and Ivers, James and Little, Reed and Merson, Paulo and Nord, Robert and Stafford, Judith},
        }

@Book{SG:SAPED96,
        title     = {Software Architecture: Perspectives on an Emerging Discipline},
        publisher = {Prentice-Hall, Inc.},
        year      = {1996},
        author    = {Shaw, Mary and Garlan, David},
        address   = {Upper Saddle River, NJ, USA},
        }

@Book{GHJV:DPEROS95,
        title     = {Design Patterns: Elements of Reusable Object-oriented Software},
        publisher = {Addison-Wesley Longman Publishing Co., Inc.},
        year      = {1995},
        author    = {Gamma, Erich and Helm, Richard and Johnson, Ralph and Vlissides, John},
        address   = {Boston, MA, USA},
        }

@InBook{S:RDS13,
        chapter    = {3},
        title      = {The Role of Design Spaces},
        publisher  = {CRC Press},
        year       = {2013},
        author     = {Shaw, Mary},
        bookauthor = {Petre, Marian and van der Hoek, Andr{\'e}},
        booktitle  = {Software Designers in Action: A Human-Centric Look at Design Work},
        }

@Article{V:HCI06,
        author    = {Visser, Willemien},
        title     = {Designing as construction of representations: A dynamic viewpoint in cognitive design research},
        journal   = {Human--Computer Interaction},
        year      = {2006},
        volume    = {21},
        number    = {1},
        pages     = {103--152},
        month     = dec,
        publisher = {Taylor \& Francis},
        }

@Article{RW:PS73,
        author  = {Rittel, Horst W. J. and Webber, Melvin M.},
        title   = {Dilemmas in a general theory of planning},
        journal = {Policy Sciences},
        year    = {1973},
        volume  = {4},
        number  = {2},
        pages   = {155--169},
        month   = jun,
        issn    = {1573-0891},
        }

@Article{BS:BCS11,
        author     = {Bell, Gordon and Siewiorek, Daniel P.},
        title      = {The Book Computer Structures: Thoughts After 40 Years},
        journal    = {IEEE Ann. Hist. Comput.},
        year       = {2011},
        volume     = {33},
        number     = {2},
        pages      = {89--95},
        month      = apr,
        issn       = {1058-6180},
        acmid      = {1990824},
        address    = IEEEPressAddr,
        issue_date = {April 2011},
        keywords   = {history of computing, Carnegie Mellon University, PMS, ISP, Bell's law, the computer artifact classification, Computer Structures, Computer History Museum},
        numpages   = {7},
        publisher  = {IEEE Educational Activities Department},
        }

@Article{S:PI80,
        author    = {Shaw, Mary},
        title     = {The impact of abstraction concerns on modern programming languages},
        journal   = {Proc. of the IEEE},
        year      = {1980},
        volume    = {68},
        number    = {9},
        pages     = {1119--1130},
        month     = apr,
        publisher = {IEEE},
        }

@Article{H:AI72,
        author  = {Hoare, C. A. R.},
        title   = {Proof of correctness of data representations},
        journal = {Acta Informatica},
        year    = {1972},
        volume  = {1},
        number  = {4},
        pages   = {271--281},
        month   = dec,
        issn    = {1432-0525},
        }

@Article{BGS:SoSyM14,
        author     = {Barnes, Jeffrey M. and Garlan, David and Schmerl, Bradley},
        title      = {Evolution Styles: Foundations and Models for Software Architecture Evolution},
        journal    = SoSyM,
        year       = {2014},
        volume     = {13},
        number     = {2},
        pages      = {649--678},
        month      = may,
        issn       = {1619-1366},
        acmid      = {2617332},
        address    = {SVNJAddr},
        issue_date = {May 2014},
        keywords   = {Software architecture},
        numpages   = {30},
        publisher  = SVNY,
        }

@Article{SAGKY:TSE06,
        author     = {Schmerl, Bradley and Aldrich, Jonathan and Garlan, David and Kazman, Rick and Yan, Hong},
        title      = {Discovering Architectures from Running Systems},
        journal    = TSE,
        year       = {2006},
        volume     = {32},
        number     = {7},
        pages      = {454--466},
        month      = jul,
        issn       = {0098-5589},
        acmid      = {1248748},
        address    = IEEEPressAddr,
        issue_date = {July 2006},
        keywords   = {Software architecture discovery, Software architecture discovery, reverse engineering, architecture design tools and analyses., architecture design tools and analyses., reverse engineering},
        numpages   = {13},
        publisher  = IEEE,
        }

@Article{GCSHSS:C04,
        author     = {Garlan, David and Cheng, Shang-Wen and Huang, An-Cheng and Schmerl, Bradley and Steenkiste, Peter},
        title      = {Rainbow: Architecture-Based Self-Adaptation with Reusable Infrastructure},
        journal    = {Computer},
        year       = {2004},
        volume     = {37},
        number     = {10},
        pages      = {46--54},
        month      = oct,
        issn       = {0018-9162},
        acmid      = {1032348},
        address    = IEEEAddr,
        issue_date = {October 2004},
        numpages   = {9},
        publisher  = IEEECSP,
        }

@Article{GAO:IEEESoftware95,
        author     = {Garlan, David and Allen, Robert and Ockerbloom, John},
        title      = {Architectural Mismatch: Why Reuse Is So Hard},
        journal    = IEEESoftware,
        year       = {1995},
        volume     = {12},
        number     = {6},
        pages      = {17--26},
        month      = nov,
        issn       = {0740-7459},
        acmid      = {625526},
        address    = IEEEAddr,
        issue_date = {November 1995},
        numpages   = {10},
        publisher  = IEEECSP,
        }

@Article{MRZWWW:IEEESoftware05,
        author     = {Maranzano, Joseph F. and Rozsypal, Sandra A. and Zimmerman, Gus H. and Warnken, Guy W. and Wirth, Patricia E. and Weiss, David M.},
        title      = {Architecture Reviews: Practice and Experience},
        journal    = IEEESoftware,
        year       = {2005},
        volume     = {22},
        number     = {2},
        pages      = {34--43},
        month      = mar,
        issn       = {0740-7459},
        acmid      = {1053649},
        address    = IEEEAddr,
        issue_date = {March 2005},
        keywords   = {software architecture, software architecture, software review, software evaluation, software evaluation, software review},
        numpages   = {10},
        publisher  = IEEECSP,
        }

@Article{DK:TSE76,
        author  = {DeRemer, Frank and Kron, Hans},
        title   = {Programming-in-the-Large Versus Programming-in-the-Small},
        journal = TSE,
        year    = {1976},
        volume  = {SE-2},
        number  = {2},
        pages   = {80-86},
        month   = jun,
        issn    = {0098-5589},
        }

@Article{H:SCP87,
        author     = {Harel, David},
        title      = {Statecharts: A Visual Formalism for Complex Systems},
        journal    = SCP,
        year       = {1987},
        volume     = {8},
        number     = {3},
        pages      = {231--274},
        month      = jun,
        issn       = {0167-6423},
        acmid      = {34886},
        address    = ENHIAddr,
        issue_date = {June 1, 1987},
        numpages   = {44},
        publisher  = ENHI,
        }

@Article{P:CACM72,
        author     = {Parnas, D. L.},
        title      = {On the Criteria to Be Used in Decomposing Systems into Modules},
        journal    = CACM,
        year       = {1972},
        volume     = {15},
        number     = {12},
        pages      = {1053--1058},
        month      = dec,
        issn       = {0001-0782},
        acmid      = {361623},
        address    = ACMAddr,
        issue_date = {Dec. 1972},
        keywords   = {KWIC index, modularity, modules, software, software design, software engineering},
        numpages   = {6},
        publisher  = ACM,
        }

@Article{WLS:TSE76,
        author     = {Wulf, W. A. and London, R. L. and Shaw, M.},
        title      = {An Introduction to the Construction and Verification of Alphard Programs},
        journal    = TSE,
        year       = {1976},
        volume     = {2},
        number     = {4},
        pages      = {253--265},
        month      = jul,
        issn       = {0098-5589},
        acmid      = {1313593},
        address    = IEEEPressAddr,
        issue_date = {July 1976},
        keywords   = {Abstract data types, abstraction and representation, assertion, correctness, information hiding, levels of abstraction, modular decomposition, program specifications, program verification, programming languages, programming methodology, structured programming, structured programming, Abstract data types, abstraction and representation, assertion, correctness, information hiding, levels of abstraction, modular decomposition, program specifications, program verification, programming languages, programming methodology},
        numpages   = {13},
        publisher  = IEEE,
        }

@Article{MN:C97,
        author     = {Murphy, Gail C. and Notkin, David},
        title      = {Reengineering with Reflexion Models: A Case Study},
        journal    = {Computer},
        year       = {1997},
        volume     = {30},
        number     = {8},
        pages      = {29--36},
        month      = aug,
        issn       = {0018-9162},
        acmid      = {620775},
        address    = IEEEAddr,
        issue_date = {August 1997},
        numpages   = {8},
        publisher  = IEEECSP,
        }

@InProceedings{MPS:ULSSIS08,
        author    = {M\"{u}ller, Hausi and Pezz\`{e}, Mauro and Shaw, Mary},
        title     = {Visibility of Control in Adaptive Systems},
        booktitle = {Proc. Int'l Workshop Ultra-Large-Scale Software-Intensive Systems (ULSSIS)},
        year      = {2008},
        pages     = {23--26},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        acmid     = {1370707},
        keywords  = {autonomic systems, continuous evolution, self-adaptive systems, software ecosystems, ultra-large scale systems},
        location  = {Leipzig, Germany},
        numpages  = {4},
        }

@InProceedings{PCW:ICSE84,
        author    = {Parnas, D. L. and Clements, P. C. and Weiss, D. M.},
        title     = {The Modular Structure of Complex Systems},
        booktitle = ICSE,
        year      = {1984},
        pages     = {408--417},
        address   = IEEEPressAddr,
        month     = mar,
        publisher = IEEE,
        acmid     = {801999},
        location  = {Orlando, FL, USA},
        numpages  = {10},
        }

@InProceedings{GDRS:LSCIS12,
        author    = {Garlan, David and Dwivedi, Vishal and Ruchkin, Ivan and Schmerl, Bradley},
        title     = {Foundations and Tools for End-user Architecting},
        booktitle = {Proc. Conf. Large-Scale Complex IT Systems: Development, Operation and Management},
        year      = {2012},
        pages     = {157--182},
        address   = SVBAddr,
        month     = mar,
        publisher = SV,
        acmid     = {2427599},
        keywords  = {end-user architecting, end-user architecture, end-user programming, software architecture, software composition, software development tools},
        location  = {Oxford, UK},
        numpages  = {26},
        }

@InProceedings{BKGS:ICCPS11,
        author    = {Bhave, Ajinkya and Krogh, Bruce and Garlan, David and Schmerl, Bradley},
        title     = {View Consistency in Architectures for Cyber-Physical Systems},
        booktitle = ICCPS,
        year      = {2011},
        pages     = {151-160},
        address   = IEEEAddr,
        month     = apr,
        publisher = IEEECSP,
        keywords  = {aircraft;formal verification;graph theory;software architecture;base architecture;connectivity graph;cyber physical system;graph matching;heterogeneous model;model based development;model checking;quadrotor air vehicle;Analytical models;Barium;Computational modeling;Computer architecture;Connectors;Encapsulation;Software;cyber-physical systems;graph morphism;multi-domain modeling;system architecture;view consistency},
        location  = {Chicago, IL, USA},
        }

@InProceedings{AG:ICSE94,
        author    = {Allen, Robert and Garlan, David},
        title     = {Formalizing Architectural Connection},
        booktitle = ICSE,
        year      = {1994},
        pages     = {71--80},
        address   = IEEEAddr,
        month     = may,
        publisher = IEEECSP,
        acmid     = {257745},
        location  = {Sorrento, Italy},
        numpages  = {10},
        }

@InProceedings{GS:SCS06,
        author    = {Garlan, David and Schmerl, Bradley},
        title     = {Architecture-driven Modelling and Analysis},
        booktitle = {Proc. Safety Critical Systems and Software (SCS)},
        year      = {2006},
        pages     = {3--17},
        address   = {Darlinghurst, Australia, Australia},
        month     = aug,
        publisher = {Australian Computer Society, Inc.},
        acmid     = {1274238},
        keywords  = {architecture analysis, software architecture},
        location  = {Melbourne, Australia},
        numpages  = {15},
        }

@InProceedings{G:FOSE14,
        author    = {Garlan, David},
        title     = {Software Architecture: A Travelogue},
        booktitle = FOSE,
        year      = {2014},
        pages     = {29--39},
        address   = ACMAddr,
        month     = jun,
        publisher = ACM,
        acmid     = {2593886},
        keywords  = {Software architecture, architecture and agility, architecture description languages, architecture styles, architecture trends, software frame-works, software product lines},
        location  = {Hyderabad, India},
        numpages  = {11},
        }

@InProceedings{SNSA:OOPSLA11,
        author    = {Sunshine, Joshua and Naden, Karl and Stork, Sven and Aldrich, Jonathan and Tanter, \'{E}ric},
        title     = {First-class State Change in Plaid},
        booktitle = OOPSLA,
        year      = {2011},
        pages     = {713--732},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        acmid     = {2048122},
        keywords  = {plaid, state-chart, typestate},
        location  = {Portland, OR, USA},
        numpages  = {20},
        }

@InProceedings{KK:WSR16,
        author    = {Kawthekar, Prasad and K{\"a}stner, Christian},
        title     = {Sensitivity Analysis For Building Evolving \& Adaptive Robotic Software},
        booktitle = {Proc. Workshop Autonomous Mobile Service Robots (WSR)},
        year      = {2016},
        month     = jul,
        keywords  = {rank4},
        location  = {New York, NY, USA},
        }

@InProceedings{VSIC:FiC16,
        author    = {Velez, Miguel and Sawin, Jason and Ingerson, Alexia and Chiu, David},
        title     = {Improving Bitmap Execution Performance Using Column-Based Metadata},
        booktitle = {Int'l Conf. Future Internet of Things and Cloud (FiCloud)},
        year      = {2016},
        pages     = {371-378},
        month     = aug,
        publisher = IEEE,
        addendum  = {(30\% acceptance rate)},
        keywords  = {rank5},
        location  = {Vienna, Austria},
        }

@Report{KKC:CMU00,
        author      = {Kazman, Rick and Klein, Mark and Clements, Paul},
        title       = {ATAM: Method for Architecture Evaluation},
        year        = {2000},
        address     = {Pittsburgh, PA},
        institution = {Software Engineering Institute, Carnegie Mellon University},
        number      = {CMU/SEI-2000-TR-004},
        type        = {Technical Report},
        }

@Report{GS:CMU94,
        author      = {Garlan, David and Shaw, Mary},
        title       = {An Introduction to Software Architecture},
        month       = jan,
        year        = {1994},
        institution = {Carnegie Mellon University},
        type        = {Technical Report CMU-CS-94-166},
        }

@Misc{VS:IUST16,
        author       = {Velez, Miguel and Sawin, Jason},
        title        = {Improving the Efficiency of CHA through Parallelization},
        howpublished = {Poster. Inquiry at St. Thomas},
        month        = may,
        year         = {2016},
        keywords     = {rank5},
        location     = {St. Paul, MN, USA},
        }

@Misc{VS:CCSC15,
        author       = {Velez, Miguel and Sawin, Jason},
        title        = {Faster {WAH} Compression Querying through the Use of Metadata},
        howpublished = {Poster. Consortium for Computing Sciences in Colleges Midwest Region},
        month        = oct,
        year         = {2015},
        note         = {{1$^{st}$} place Discovery Track},
        keywords     = {rank5},
        location     = {Evansville, IN, USA},
        }

@Misc{VS:MSRP15,
        author       = {Velez, Miguel and Solar-Lezama, Armando},
        title        = {Simpler Implementation of {Sketches} through Enhanced Expressiveness},
        howpublished = {Poster. MIT Summer Research Poster Session},
        month        = aug,
        year         = {2015},
        keywords     = {rank5},
        location     = {Cambridge, MA, USA},
        }

@Misc{V:SUMMA15,
        author       = {Velez, Miguel},
        title        = {Current and Future Relationships Between Robots and Humans},
        howpublished = {Summa Cum Laude Paper},
        month        = apr,
        year         = {2015},
        keywords     = {rank5},
        }

@Misc{VGS:IUST14,
        author       = {Velez, Miguel and Gittins, Peter and Sawin, Jason},
        title        = {Extending {SMILES} to Encode Reaction Mechanisms},
        howpublished = {Poster. Inquiry at St. Thomas},
        month        = may,
        year         = {2014},
        keywords     = {rank5},
        location     = {St. Paul, MN, USA},
        }

@Article{MS:CACM16,
        author       = {Myers, Brad A. and Stylos, Jeffrey},
        title        = {Improving API Usability},
        year         = {2016},
        volume       = {59},
        number       = {6},
        pages        = {62--69},
        month        = may,
        issn         = {0001-0782},
        address      = ACMAddr,
        issue_date   = {June 2016},
        journaltitle = CACM,
        numpages     = {8},
        publisher    = ACM,
        }

@Article{MKLY:C16,
        author       = {Myers, Brad A. and Ko, Andrew J. and LaToza, Thomas D. and Yoon, YoungSeok},
        title        = {Programmers Are Users Too: Human-Centered Methods for Improving Programming Tools},
        year         = {2016},
        volume       = {49},
        number       = {7},
        pages        = {44-52},
        month        = jul,
        issn         = {0018-9162},
        address      = IEEEAddr,
        journaltitle = {Computer},
        publisher    = IEEECSP,
        }

@InProceedings{YYZPB:ESECFSE11,
        author    = {Yin, Zuoning and Yuan, Ding and Zhou, Yuanyuan and Pasupathy, Shankar and Bairavasundaram, Lakshmi},
        title     = {How Do Fixes Become Bugs?},
        booktitle = ESECFSE,
        year      = {2011},
        pages     = {26--36},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        location  = {Szeged, Hungary},
        numpages  = {11},
        }

@InProceedings{SRA:GPCE13,
        author    = {Siegmund, Norbert and {von Rhein}, Alexander and Apel, Sven},
        title     = {Family-Based Performance Measurement},
        booktitle = GPCE,
        year      = {2013},
        publisher = ACM,
        location  = {Indianapolis, IN, USA},
        month     = oct,
        pages     = {95-104},
        address   = ACMAddr,
        keywords  = {rank4},
        numpages  = {10},
        }

@InProceedings{EHMG:ESECFSE15,
        author    = {Eichberg, Michael and Hermann, Ben and Mezini, Mira and Glanz, Leonid},
        title     = {Hidden Truths in Dead Software Paths},
        booktitle = ESECFSE,
        year      = {2015},
        pages     = {474--484},
        address   = ACMAddr,
        month     = aug,
        publisher = ACM,
        acmid     = {2786865},
        location  = {Bergamo, Italy},
        numpages  = {11},
        }

@InProceedings{SGAK:ESECFSE15,
        author    = {Siegmund, Norbert and Grebhahn, Alexander and Apel, Sven and K\"{a}stner, Christian},
        title     = {Performance-influence Models for Highly Configurable Systems},
        booktitle = ESECFSE,
        year      = {2015},
        pages     = {284--294},
        address   = ACMAddr,
        month     = aug,
        publisher = ACM,
        keywords  = {Performance-influence models, machine learning, sampling},
        location  = {Bergamo, Italy},
        numpages  = {11},
        }

@InProceedings{DH:ICSE09,
        author    = {Dekel, Uri and Herbsleb, James D.},
        title     = {Improving API Documentation Usability with Knowledge Pushing},
        booktitle = ICSE,
        year      = {2009},
        pages     = {320--330},
        address   = IEEEAddr,
        month     = may,
        publisher = IEEECSP,
        location  = {Vancouver, Canada},
        numpages  = {11},
        }

@InProceedings{GF:RE95,
        author    = {Gotel, Orlena and Finkelstein, Anthony},
        title     = {Contribution Structures},
        booktitle = RE,
        year      = {1995},
        pages     = {100--107},
        address   = IEEEAddrW,
        month     = mar,
        publisher = IEEE,
        location  = {York, U.K.},
        }

@InProceedings{J:ICSE95,
        author    = {Jackson, Michael},
        title     = {The World and the Machine},
        booktitle = ICSE,
        year      = {1995},
        pages     = {283--292},
        address   = ACMAddr,
        month     = apr,
        publisher = ACM,
        location  = {Seattle, WA, USA},
        numpages  = {10},
        }

@InProceedings{PN:RE97,
        author    = {Potts, Colin and Newstetter, Wendy C.},
        title     = {Naturalistic Inquiry and Requirements Engineering: Reconciling Their Theoretical Foundations},
        booktitle = RE,
        year      = {1997},
        pages     = {118--127},
        address   = IEEEAddrW,
        month     = jan,
        publisher = IEEE,
        keywords  = {formal specification, requirements engineering, naturalistic inquiry, ethnography, social and contextual factors},
        location  = {Annapolis, MD, USA},
        }

@InProceedings{AEW:RE07,
        author    = {Aranda, Jorge and Easterbrook, Steve and Wilson, Greg},
        title     = {Requirements in the wild: How small companies do it},
        booktitle = RE,
        year      = {2007},
        pages     = {39-48},
        address   = IEEEAddrW,
        month     = oct,
        publisher = IEEE,
        issn      = {1090-705X},
        location  = {New Delhi, India},
        }

@InProceedings{AKLRU:ICSE12,
        author    = {Alrajeh, Dalal and Kramer, Jeff and Lamsweerde, Axel van and Russo, Alessandra and Uchitel, Sebasti\'{a}n},
        title     = {Generating Obstacle Conditions for Requirements Completeness},
        booktitle = ICSE,
        year      = {2012},
        pages     = {705--715},
        address   = IEEEPressAddr,
        month     = jun,
        publisher = IEEE,
        location  = {Zurich, Switzerland},
        numpages  = {11},
        }

@InProceedings{NB:RE12,
        author    = {Niknafs, Ali and Berry, Daniel M.},
        title     = {The impact of domain knowledge on the effectiveness of requirements idea generation during requirements elicitation},
        booktitle = RE,
        year      = {2012},
        pages     = {181-190},
        address   = IEEEAddrW,
        month     = sep,
        publisher = IEEE,
        issn      = {1090-705X},
        location  = {Chicago, IL, USA},
        }

@Book{Y:CSRDM09,
        title     = {Case Study Research: Design and Methods},
        publisher = {SAGE Publications},
        year      = {2009},
        author    = {Yin, Robert},
        series    = {Applied Social Research Methods},
        edition   = {4th},
        }

@InProceedings{WLC:ASE16,
        author    = {Wei, Lili and Liu, Yepang and Cheung, Shing-Chi},
        title     = {Taming Android Fragmentation: Characterizing and Detecting Compatibility Issues for Android Apps},
        booktitle = ASE,
        year      = {2016},
        pages     = {226--237},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        keywords  = {Android fragmentation, compatibility issues},
        location  = {Singapore, Singapore},
        numpages  = {12},
        }

@InProceedings{V:RE01,
        author    = {Van Lamsweerde, Axel},
        title     = {Goal-Oriented Requirements Engineering: A Guided Tour},
        booktitle = RE,
        year      = {2001},
        pages     = {249--262},
        address   = IEEEAddrW,
        month     = aug,
        publisher = IEEE,
        location  = {Toronto, Canada},
        }

@InProceedings{MJKNZM:RE10,
        author    = {Maiden, Neil and Jones, Sara and Karlsen, Kristine and Neill, Roger and Zachos, Konstantinos and Milne, Alastair},
        title     = {Requirements Engineering As Creative Problem Solving: A Research Agenda for Idea Finding},
        booktitle = RE,
        year      = {2010},
        pages     = {57--66},
        address   = IEEEAddrW,
        month     = sep,
        publisher = IEEE,
        location  = {Sydney, Australia},
        numpages  = {10},
        }

@InProceedings{SBWLKF:RE10,
        author    = {Sawyer, Pete and Bencomo, Nelly and Whittle, Jon and Letier, Emmanuel and Finkelstein, Anthony},
        title     = {Requirements-Aware Systems: A Research Agenda for RE for Self-adaptive Systems},
        booktitle = RE,
        year      = {2010},
        pages     = {95--103},
        address   = IEEEAddrW,
        month     = sep,
        publisher = IEEE,
        location  = {Sydney, Australia},
        numpages  = {9},
        }

@Article{CKI:CACM88,
        author     = {Curtis, Bill and Krasner, Herb and Iscoe, Neil},
        title      = {A Field Study of the Software Design Process for Large Systems},
        journal    = CACM,
        year       = {1988},
        volume     = {31},
        number     = {11},
        pages      = {1268--1287},
        month      = nov,
        issn       = {0001-0782},
        address    = ACMAddr,
        issue_date = {Nov. 1988},
        numpages   = {20},
        publisher  = ACM,
        }

@Article{C:D68,
        author  = {Conway, Melvin E},
        title   = {How do committees invent?},
        journal = {Datamation},
        year    = {1968},
        volume  = {14},
        number  = {4},
        pages   = {28--31},
        }

@Article{KS:CACM95,
        author     = {Kraut, Robert E. and Streeter, Lynn A.},
        title      = {Coordination in Software Development},
        journal    = CACM,
        year       = {1995},
        volume     = {38},
        number     = {3},
        pages      = {69--81},
        month      = mar,
        issn       = {0001-0782},
        address    = ACMAddr,
        issue_date = {March 1995},
        numpages   = {13},
        publisher  = ACM,
        }

@Article{MFH:TOSEM02,
        author     = {Mockus, Audris and Fielding, Roy T. and Herbsleb, James D.},
        title      = {Two Case Studies of Open Source Software Development: Apache and Mozilla},
        journal    = TOSEM,
        year       = {2002},
        volume     = {11},
        number     = {3},
        pages      = {309--346},
        month      = jul,
        issn       = {1049-331X},
        address    = ACMAddr,
        issue_date = {July 2002},
        keywords   = {Apache, Mozilla, Open source software, code ownership, defect density, repair interval},
        numpages   = {38},
        publisher  = ACM,
        }

@InProceedings{VBXCDDK:ICSE16,
        author    = {Vasilescu, Bogdan and Blincoe, Kelly and Xuan, Qi and Casalnuovo, Casey and Damian, Daniela and Devanbu, Premkumar and Filkov, Vladimir},
        title     = {The Sky is Not the Limit: Multitasking Across GitHub Projects},
        booktitle = ICSE,
        year      = {2016},
        pages     = {994--1005},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        acmid     = {2884875},
        keywords  = {GitHub, multitasking, productivity},
        location  = {Austin, TX, USA},
        numpages  = {12},
        }

@InProceedings{HBSGD:ICSE12,
        author    = {Hindle, Abram and Barr, Earl T. and Su, Zhendong and Gabel, Mark and Devanbu, Premkumar},
        title     = {On the Naturalness of Software},
        booktitle = ICSE,
        year      = {2012},
        pages     = {837--847},
        address   = IEEEPressAddr,
        month     = jun,
        publisher = IEEE,
        location  = {Zurich, Switzerland},
        numpages  = {11},
        }

@InProceedings{NMB:ICSE08,
        author    = {Nagappan, Nachiappan and Murphy, Brendan and Basili, Victor},
        title     = {The Influence of Organizational Structure on Software Quality: An Empirical Case Study},
        booktitle = ICSE,
        year      = {2008},
        pages     = {521--530},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Leipzig, Germany},
        numpages  = {10},
        }

@InProceedings{AV:ICSE09,
        author    = {Aranda, Jorge and Venolia, Gina},
        title     = {The Secret Life of Bugs: Going Past the Errors and Omissions in Software Repositories},
        booktitle = ICSE,
        year      = {2009},
        pages     = {298--308},
        address   = IEEEAddrW,
        month     = may,
        publisher = IEEE,
        location  = {Vancouver, Canada},
        numpages  = {11},
        }

@InProceedings{DSTH:CSCW12,
        author    = {Dabbish, Laura and Stuart, Colleen and Tsay, Jason and Herbsleb, Jim},
        title     = {Social Coding in GitHub: Transparency and Collaboration in an Open Software Repository},
        booktitle = CSCW,
        year      = {2012},
        pages     = {1277--1286},
        address   = ACMAddr,
        month     = feb,
        publisher = ACM,
        location  = {Seattle, WA, USA},
        numpages  = {10},
        }

@Article{D:CSCW05,
        author     = {Ducheneaut, Nicolas},
        title      = {Socialization in an Open Source Software Community: A Socio-Technical Analysis},
        journal    = {Comput. Supported Coop. Work},
        year       = {2005},
        volume     = {14},
        number     = {4},
        pages      = {323--368},
        month      = aug,
        issn       = {0925-9724},
        address    = {Norwell, MA, USA},
        issue_date = {August 2005},
        keywords   = {Open Source, actor-network, learning, socialization, software development},
        numpages   = {46},
        publisher  = {Kluwer Academic Publishers},
        }

@Article{B:C87,
        author     = {Brooks,Jr., Frederick P.},
        title      = {No Silver Bullet Essence and Accidents of Software Engineering},
        journal    = {Computer},
        year       = {1987},
        volume     = {20},
        number     = {4},
        pages      = {10--19},
        month      = apr,
        issn       = {0018-9162},
        address    = IEEEAddr,
        issue_date = {April 1987},
        numpages   = {10},
        publisher  = IEEECSP,
        }

@Book{NR:NATO69,
        title     = {Software Engineering: Report of a Conference Sponsored by the NATO Science Committee, Garmisch, Germany, 7-11 Oct. 1968, Brussels, Scientific Affairs Division, NATO},
        publisher = {NATO},
        year      = {1969},
        author    = {Naur, Peter and Randell, Brian},
        }

@InProceedings{B:ICSR94,
        author    = {Ted Biggerstaff},
        title     = {The Library Scaling Problem and the Limits of Concrete Component Reuse},
        booktitle = ICSR,
        year      = {1994},
        pages     = {102--109},
        address   = IEEEAddr,
        publisher = IEEE,
        location  = {Rio de Janeiro, Brazil},
        }

@Book{ABKS:FOSPL13,
        title     = {Feature-Oriented Software Product Lines: Concepts and Implementation},
        publisher = SV,
        year      = {2013},
        author    = {Apel, Sven and Batory,Don and K{\"a}stner, Christian and Saake, Gunter},
        address   = SVBAddr,
        }

@Book{B:MMM95,
        title     = {The Mythical Man-Month},
        publisher = AWL,
        year      = {1995},
        author    = {Brooks, Jr., Frederick P.},
        address   = AWLAddr,
        edition   = {anniversary},
        }

@Book{C:CS02,
        title     = {Component Software: Beyond Object-Oriented Programming},
        publisher = AWL,
        year      = {2002},
        author    = {Clemens Szyperski},
        address   = AWLAddr,
        edition   = {2nd},
        }

@Book{CE:GP00,
        title     = {Generative Programming: Methods, Tools, and Applications},
        publisher = {ACM Press/Addison-Wesley},
        year      = {2000},
        author    = {Czarnecki, Krzysztof and Eisenecker, Ulrich},
        address   = ACMAddr,
        }

@Article{JF:JOOP88,
        author  = {Johnson, Ralph and Foote, Brian},
        title   = {Designing Reusable Classes},
        journal = {Journal of Object-Oriented Programming SIGS},
        year    = {1988},
        volume  = {1},
        number  = {5},
        pages   = {22-35},
        month   = jun,
        }

@InProceedings{ZZB:PROMISE11,
        author    = {Zeller, Andreas and Zimmermann, Thomas and Bird, Christian},
        title     = {Failure is a Four-letter Word},
        booktitle = {Proc. Int'l Conf. Predictive Models in Software Engineering (PROMISE)},
        year      = {2011},
        pages     = {5:1--5:7},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        artlceno  = {5},
        location  = {Banff, Alberta, Canada},
        numpages  = {7},
        }

@InProceedings{F:ANIPS01,
        author    = {Fox, Dieter},
        title     = {KLD-Sampling: Adaptive Particle Filters},
        booktitle = {Advances in Neural Information Processing Systems 14},
        year      = {2001},
        publisher = MIT,
        keywords  = {rank4},
        }

@InProceedings{NKCFP:FSE16,
        author    = {Nguyen, Thanhvu and Koc, Thanhvu and Cheng, Javran and Foster, Jeffrey S. and Porter, Adam A.},
        title     = {i{G}en Dynamic Interaction Inference for Configurable Software},
        booktitle = FSE,
        year      = {2016},
        publisher = IEEE,
        location  = {Seattle, WA, USA},
        month     = nov,
        address   = IEEEAddr,
        }

@InProceedings{BSR:ICSE03,
        author    = {Batory, Don and Sarvela, Jacob Neal and Rauschmayer, Axel},
        title     = {Scaling Step-wise Refinement},
        booktitle = ICSE,
        year      = {2003},
        pages     = {187--197},
        address   = IEEEAddr,
        month     = may,
        publisher = IEEE,
        location  = {Portland, OR, USA},
        numpages  = {11},
        }

@Report{FF:RIACS00,
        author      = {Filman, Robert E. and Friedman, Daniel P.},
        title       = {Aspect-Oriented Programming is Quantification and Obliviousness},
        year        = {2000},
        institution = {NASA},
        publisher   = {RIACS},
        type        = {Technical Report},
        }

@Book{L:AA03,
        title     = {{AspectJ} in Action: Practical Aspect-Oriented Programming},
        publisher = {Manning Publications},
        year      = {2003},
        author    = {Ramnivas Laddad},
        address   = {Greenwich, CT, USA},
        }

@InProceedings{S:OOPSLA06,
        author    = {Steimann, Friedrich},
        title     = {The Paradoxical Success of Aspect-oriented Programming},
        booktitle = OOPSLA,
        year      = {2006},
        pages     = {481--497},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        location  = {Portland, OR, USA},
        numpages  = {17},
        }

@InProceedings{TOHS:ICSE99,
        author    = {Tarr, Peri and Ossher, Harold and Harrison, William and Sutton,Jr., Stanley M.},
        title     = {N Degrees of Separation: Multi-dimensional Separation of Concerns},
        booktitle = ICSE,
        year      = {1999},
        pages     = {107--119},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Los Angeles, CA, USA},
        numpages  = {13},
        }

@InProceedings{C:POPL97,
        author    = {Cardelli, Luca},
        title     = {Program Fragments, Linking, and Modularization},
        booktitle = POPL,
        year      = {1997},
        pages     = {266--277},
        address   = ACMAddr,
        month     = jan,
        publisher = ACM,
        location  = {Paris, France},
        numpages  = {12},
        }

@InProceedings{GDS:ICSE12,
        author    = {Greiler, Michaela and Deursen, Arie van and Storey, Margaret-Anne},
        title     = {Test Confessions: A Study of Testing Practices for Plug-in Systems},
        booktitle = ICSE,
        year      = {2012},
        pages     = {244--254},
        address   = IEEE,
        month     = jun,
        publisher = IEEE,
        location  = {Zurich, Switzerland},
        numpages  = {11},
        }

@Article{NLN:PI08,
        author     = {Nhlabatsi, Armstrong and Laney, Robin and Nuseibeh, Bashar},
        title      = {Feature Interaction: The Security Threat from within Software Systems},
        journal    = {Progress in Informatics},
        year       = {2008},
        number     = {5},
        pages      = {75--89},
        month      = mar,
        issue_date = {March 2008},
        numpages   = {15},
        }

@InProceedings{RR:ICSE85,
        author    = {Redwine,Jr., Samuel T. and Riddle, William E.},
        title     = {Software Technology Maturation},
        booktitle = ICSE,
        year      = {1985},
        pages     = {189--200},
        address   = IEEEAddr,
        month     = aug,
        publisher = IEEECSP,
        location  = {London, England},
        numpages  = {12},
        }

@InProceedings{S:ICSE03,
        author    = {Shaw, Mary},
        title     = {Writing Good Software Engineering Research Papers: Minitutorial},
        booktitle = ICSE,
        year      = {2003},
        pages     = {726--736},
        address   = IEEEAddrW,
        month     = may,
        publisher = IEEE,
        location  = {Portland, Oregon},
        numpages  = {11},
        }

@Article{B:C88,
        author     = {Boehm, Barry W.},
        title      = {A Spiral Model of Software Development and Enhancement},
        journal    = {Computer},
        year       = {1988},
        volume     = {21},
        number     = {5},
        pages      = {61--72},
        month      = may,
        issn       = {0018-9162},
        address    = IEEEAddr,
        issue_date = {May 1988},
        numpages   = {12},
        publisher  = IEEECSP,
        }

@Article{H:IEEESoftware88,
        author     = {Humphrey, Watts S.},
        title      = {Characterizing the Software Process: A Maturity Framework},
        journal    = IEEESoftware,
        year       = {1988},
        volume     = {5},
        number     = {2},
        pages      = {73--79},
        month      = mar,
        issn       = {0740-7459},
        address    = IEEEAddr,
        issue_date = {March 1988},
        numpages   = {7},
        publisher  = IEEECSP,
        }

@InProceedings{O:ICSE87,
        author    = {Osterweil, L.},
        title     = {Software Processes Are Software Too},
        booktitle = ICSE,
        year      = {1987},
        pages     = {2--13},
        address   = IEEEAddr,
        month     = mar,
        publisher = IEEECSP,
        location  = {Monterey, CA, USA},
        numpages  = {12},
        }

@InProceedings{R:ICSE87,
        author    = {Royce, W. W.},
        title     = {Managing the Development of Large Software Systems: Concepts and Techniques},
        booktitle = ICSE,
        year      = {1987},
        pages     = {328--338},
        address   = IEEEAddr,
        month     = mar,
        publisher = IEEECSP,
        location  = {Monterey, CA, USA},
        numpages  = {11},
        }

@Book{SSS:GAESE07,
        title     = {Guide to Advanced Empirical Software Engineering},
        publisher = SVNY,
        year      = {2007},
        author    = {Shull, Forrest and Singer, Janice and Sj{\o}berg, Dag I.K.},
        address   = SVNJAddr,
        }

@Article{H:IEEESoftware90,
        author     = {Hall, Anthony},
        title      = {Seven Myths of Formal Methods},
        journal    = IEEESoftware,
        year       = {1990},
        volume     = {7},
        number     = {5},
        pages      = {11--19},
        month      = sep,
        issn       = {0740-7459},
        address    = IEEEAddr,
        issue_date = {September 1990},
        numpages   = {9},
        publisher  = IEEECSP,
        }

@Article{CR:ESE94,
        author  = {Caldiera, Victor R Basili-Gianluigi and Rombach, H Dieter},
        title   = {Goal question metric paradigm},
        journal = {Encyclopedia of Software Engineering},
        year    = {1994},
        volume  = {1},
        pages   = {528--532},
        }

@Article{DLP:CACM79,
        author     = {De Millo, Richard A. and Lipton, Richard J. and Perlis, Alan J.},
        title      = {Social Processes and Proofs of Theorems and Programs},
        journal    = CACM,
        year       = {1979},
        volume     = {22},
        number     = {5},
        pages      = {271--280},
        month      = may,
        issn       = {0001-0782},
        address    = ACMAddr,
        issue_date = {May 1979},
        numpages   = {10},
        publisher  = ACM,
        }

@Article{T:NIST02,
        author    = {Tassey, Gregory},
        title     = {The economic impacts of inadequate infrastructure for software testing},
        journal   = {National Institute of Standards and Technology, RTI Project},
        year      = {2002},
        volume    = {7007},
        number    = {011},
        publisher = {Citeseer},
        }

@InProceedings{ANHL:ITHINGS14,
        author    = {Anon, Fabrice and Navarathinarasah, Vijith and Hoang, Minh and Lung, Chung-Horng},
        title     = {Building a Framework for Internet of Things and Cloud Computing},
        booktitle = ITHINGS,
        year      = {2014},
        pages     = {132--139},
        address   = IEEEAddrW,
        month     = sep,
        publisher = IEEE,
        keywords  = {rank4},
        location  = {Taipei, Taiwan},
        numpages  = {8},
        }

@InProceedings{GCASW:ASE13,
  author    = {Guo, Jianmei and Czarnecki, Krzysztof and Apel, Sven and Siegmund, Norbert and W{\k{a}}sowski, Andrzej},
  booktitle = ASE,
  title     = {Variability-aware performance prediction: A statistical learning approach},
  year      = {2013},
  address   = ACMAddr,
  month     = nov,
  pages     = {301--311},
  publisher = ACM,
  location  = {Silicon Valley, CA, USA},
}

@Article{H:CACM,
        author     = {Hoos, Holger H.},
        title      = {Programming by Optimization},
        journal    = CACM,
        year       = {2012},
        volume     = {55},
        number     = {2},
        pages      = {70--80},
        month      = feb,
        issn       = {0001-0782},
        address    = ACMAddr,
        issue_date = {February 2012},
        numpages   = {11},
        publisher  = ACM,
        }

@Article{BLR:CACM11,
        author     = {Ball, Thomas and Levin, Vladimir and Rajamani, Sriram K.},
        title      = {A Decade of Software Model Checking with SLAM},
        journal    = CACM,
        year       = {2011},
        volume     = {54},
        number     = {7},
        pages      = {68--76},
        month      = jul,
        issn       = {0001-0782},
        acmid      = {1965743},
        address    = ACMAddr,
        issue_date = {July 2011},
        numpages   = {9},
        publisher  = ACM,
        }

@InProceedings{SS:PPOPP10,
        author    = {Sutherland, Dean F. and Scherlis, William L.},
        title     = {Composable Thread Coloring},
        booktitle = {Proc. Symp. Principles and Practice of Parallel Programming},
        year      = {2010},
        pages     = {233--244},
        address   = ACMAddr,
        month     = jan,
        publisher = ACM,
        location  = {Bangalore, India},
        numpages  = {12},
        }

@InProceedings{BGMRMT:GPCE16,
        author    = {Braz, Larissa and Gheyi, Rohit and Mongiovi, Melina and Ribeiro, M\'{a}rcio and Medeiros, Fl\'{a}vio and Teixeira, Leopoldo},
        title     = {A Change-centric Approach to Compile Configurable Systems with \#Ifdefs},
        booktitle = GPCE,
        year      = {2016},
        pages     = {109--119},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        comment   = {Maybe we can use this approach to find bugs? Just check the previous and current commit to see differences?},
        location  = {Amsterdam, Netherlands},
        numpages  = {11},
        }

@Article{SCK:TDSC04,
        author     = {Siewiorek, Daniel P. and Chillarege, Ram and T. Kalbarczyk, Zbigniew},
        title      = {Reflections on Industry Trends and Experimental Research in Dependability},
        journal    = {IEEE Trans. Dependable Secur. Comput.},
        year       = {2004},
        volume     = {1},
        number     = {2},
        pages      = {109--127},
        month      = apr,
        issn       = {1545-5971},
        acmid      = {1032594},
        address    = IEEEAddr,
        issue_date = {April 2004},
        numpages   = {19},
        publisher  = IEEECSP,
        }

@Article{SN:NASA05,
        author  = {Siewiorek, Daniel P and Narasimhan, Priya},
        title   = {Fault-tolerant architectures for space and avionics applications},
        journal = {NASA Ames Research},
        year    = {2005},
        }

@Book{M:ML97,
        title     = {Machine Learning},
        publisher = {McGraw-Hill, Inc.},
        year      = {1997},
        author    = {Mitchell, Thomas M.},
        address   = {New York, NY, USA},
        edition   = {1st},
        }

@Book{HS:AMP08,
        title     = {The Art of Multiprocessor Programming},
        publisher = {Morgan Kaufmann Publishers Inc.},
        year      = {2008},
        author    = {Herlihy, Maurice and Shavit, Nir},
        address   = {San Francisco, CA, USA},
        }

@Book{M:MLPP12,
        title     = {Machine Learning: A Probabilistic Perspective},
        publisher = MIT,
        year      = {2012},
        author    = {Murphy, Kevin P.},
        }

@Book{ST:DPENPOOD02,
        title     = {Design Patterns Explained: A New Perspective on Object-Oriented Design},
        publisher = AWL,
        year      = {2002},
        author    = {Shalloway, Alan and Trott, James R.},
        address   = AWLAddr,
        }

@Book{B:PRML06,
        title     = {Pattern Recognition and Machine Learning (Information Science and Statistics)},
        publisher = SVNY,
        year      = {2006},
        author    = {Bishop, Christopher M.},
        address   = SVNJAddr,
        }

@Book{M:ITILA02,
        title     = {Information Theory, Inference \& Learning Algorithms},
        publisher = {Cambridge University Press},
        year      = {2002},
        author    = {MacKay, David J. C.},
        address   = {New York, NY, USA},
        }

@Book{WFH:DMPMLTT11,
        title     = {Data Mining: Practical Machine Learning Tools and Techniques},
        publisher = {Morgan Kaufmann Publishers Inc.},
        year      = {2011},
        author    = {Witten, Ian H. and Frank, Eibe and Hall, Mark A.},
        address   = {San Francisco, CA, USA},
        edition   = {3rd},
        }

@Article{CES:ACMTPLS86,
        author     = {Clarke, E. M. and Emerson, E. A. and Sistla, A. P.},
        title      = {Automatic Verification of Finite-state Concurrent Systems Using Temporal Logic Specifications},
        journal    = {ACM Trans. Program. Lang. Syst.},
        year       = {1986},
        volume     = {8},
        number     = {2},
        pages      = {244--263},
        month      = apr,
        issn       = {0164-0925},
        address    = ACMAddr,
        issue_date = {April 1986},
        numpages   = {20},
        publisher  = ACM,
        }

@InProceedings{HJMS:POPL02,
        author    = {Henzinger, Thomas A. and Jhala, Ranjit and Majumdar, Rupak and Sutre, Gr{\'e}goire},
        title     = {Lazy Abstraction},
        booktitle = POPL,
        year      = {2002},
        pages     = {58--70},
        address   = ACMAddr,
        month     = jan,
        publisher = ACM,
        location  = {Portland, OR, USA},
        numpages  = {13},
        }

@Article{AHMPP:IEEESoftware08,
        author     = {Ayewah, Nathaniel and Hovemeyer, David and Morgenthaler, J. David and Penix, John and Pugh, William},
        title      = {Using Static Analysis to Find Bugs},
        journal    = IEEESoftware,
        year       = {2008},
        volume     = {25},
        number     = {5},
        pages      = {22--29},
        month      = sep,
        issn       = {0740-7459},
        address    = IEEEAddr,
        issue_date = {September 2008},
        numpages   = {8},
        publisher  = IEEECSP,
        }

@InProceedings{W:ICSE81,
        author    = {Weiser, Mark},
        title     = {Program Slicing},
        booktitle = ICSE,
        year      = {1981},
        pages     = {439--449},
        address   = IEEEPressAddr,
        month     = mar,
        publisher = IEEE,
        location  = {San Diego, CA, USA},
        numpages  = {11},
        }

@Article{BBCCFHHKME:CACM10,
        author     = {Bessey, Al and Block, Ken and Chelf, Ben and Chou, Andy and Fulton, Bryan and Hallem, Seth and Henri-Gros, Charles and Kamsky, Asya and McPeak, Scott and Engler, Dawson},
        title      = {A Few Billion Lines of Code Later: Using Static Analysis to Find Bugs in the Real World},
        journal    = CACM,
        year       = {2010},
        volume     = {53},
        number     = {2},
        pages      = {66--75},
        month      = feb,
        issn       = {0001-0782},
        acmid      = {1646374},
        address    = ACMAddr,
        issue_date = {February 2010},
        numpages   = {10},
        publisher  = ACM,
        }

@InProceedings{BR:SPIN01,
        author    = {Ball, Thomas and Rajamani, Sriram K.},
        title     = {Automatically Validating Temporal Safety Properties of Interfaces},
        booktitle = {Proc. Int'l Workshop Model Checking of Software (SPIN)},
        year      = {2001},
        pages     = {103--122},
        address   = SVNYAddr,
        month     = may,
        publisher = SVNY,
        location  = {Toronto, Canada},
        numpages  = {20},
        }

@InProceedings{ECGN:ICSE99,
        author    = {Ernst, Michael D. and Cockrell, Jake and Griswold, William G. and Notkin, David},
        title     = {Dynamically Discovering Likely Program Invariants to Support Program Evolution},
        booktitle = ICSE,
        year      = {1999},
        pages     = {213--224},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Los Angeles, CA, USA},
        numpages  = {12},
        }

@InProceedings{PO:ISSTA11,
        author    = {Parnin, Chris and Orso, Alessandro},
        title     = {Are Automated Debugging Techniques Actually Helping Programmers?},
        booktitle = ISSTA,
        year      = {2011},
        pages     = {199--209},
        address   = ACMAddr,
        month     = jul,
        publisher = ACM,
        location  = {Toronto, Canada},
        numpages  = {11},
        }

@InProceedings{JSGMA:GREENS15,
        author    = {Jabbarvand, Reyhaneh and Sadeghi, Alireza and Garcia, Joshua and Malek, Sam and Ammann, Paul},
        title     = {EcoDroid: An Approach for Energy-based Ranking of Android Apps},
        booktitle = {Proc. Int'l Workshop Green and Sustainable Software (GREENS)},
        year      = {2015},
        pages     = {8--14},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {Florence, Italy},
        numpages  = {7},
        }

@InProceedings{P:ICSE78,
        author    = {Parnas, David L.},
        title     = {Designing Software for Ease of Extension and Contraction},
        booktitle = ICSE,
        year      = {1978},
        pages     = {264--277},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {Atlanta, GA, USA},
        numpages  = {14},
        }

@InProceedings{HLHG:ICSE13,
        author    = {Hao, Shuai and Li, Ding and Halfond, William G. J. and Govindan, Ramesh},
        title     = {Estimating Mobile Application Energy Consumption Using Program Analysis},
        booktitle = ICSE,
        year      = {2013},
        pages     = {92--101},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {San Francisco, CA, USA},
        numpages  = {10},
        }

@InProceedings{HPHL:ICSE15,
        author    = {Henard, Christopher and Papadakis, Mike and Harman, Mark and Le Traon, Yves},
        title     = {Combining Multi-objective Search and Constraint Solving for Configuring Large Software Product Lines},
        booktitle = ICSE,
        year      = {2015},
        pages     = {517--528},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {Florence, Italy},
        numpages  = {12},
        }

@Article{SRKKAS:SQJ12,
  author     = {Siegmund, Norbert and Rosenm\"{u}ller, Marko and Kuhlemann, Martin and K\"{a}stner, Christian and Apel, Sven and Saake, Gunter},
  journal    = {Software Quality Journal},
  title      = {{SPLC}onqueror: Toward Optimization of Non-functional Properties in Software Product Lines},
  year       = {2012},
  issn       = {0963-9314},
  month      = sep,
  number     = {3-4},
  pages      = {487--517},
  volume     = {20},
  address    = {Hingham, MA, USA},
  issue_date = {September 2012},
  numpages   = {31},
  publisher  = {Kluwer Academic Publishers},
}

@InProceedings{HSCMAR:ASPLOS11,
        author    = {Hoffmann, Henry and Sidiroglou, Stelios and Carbin, Michael and Misailovic, Sasa and Agarwal, Anant and Rinard, Martin},
        title     = {Dynamic Knobs for Responsive Power-aware Computing},
        booktitle = ASPLOS,
        year      = {2011},
        pages     = {199--212},
        address   = ACMAddr,
        month     = mar,
        publisher = ACM,
        location  = {Newport Beach, CA, USA},
        numpages  = {14},
        }

@InProceedings{KMKBSBD:ESECFSE13,
  author    = {Kim, Chang Hwan Peter and Marinov, Darko and Khurshid, Sarfraz and Batory, Don and Souto, Sabrina and Barros, Paulo and d'Amorim, Marcelo},
  booktitle = ESECFSE,
  title     = {{SPL}at: Lightweight Dynamic Analysis for Reducing Combinatorics in Testing Configurable Systems},
  year      = {2013},
  address   = ACMAddr,
  month     = aug,
  pages     = {257--267},
  publisher = ACM,
  location  = {Saint Petersburg, Russia},
  numpages  = {11},
}

@InProceedings{ERP:FSE14,
        author    = {Elbaum, Sebastian and Rothermel, Gregg and Penix, John},
        title     = {Techniques for Improving Regression Testing in Continuous Integration Development Environments},
        booktitle = FSE,
        year      = {2014},
        pages     = {235--245},
        address   = ACMAddr,
        month     = nov,
        publisher = ACM,
        location  = {Hong Kong, China},
        numpages  = {11},
        }

@InProceedings{GKS:PLDI05,
        author    = {Godefroid, Patrice and Klarlund, Nils and Sen, Koushik},
        title     = {DART: Directed Automated Random Testing},
        booktitle = PLDI,
        year      = {2005},
        pages     = {213--223},
        address   = ACMAddr,
        month     = jun,
        publisher = ACM,
        location  = {Chicago, IL, USA},
        numpages  = {11},
        }

@Article{K:CACM76,
        author     = {King, James C.},
        title      = {Symbolic Execution and Program Testing},
        journal    = CACM,
        year       = {1976},
        volume     = {19},
        number     = {7},
        pages      = {385--394},
        month      = jul,
        issn       = {0001-0782},
        address    = ACMAddr,
        issue_date = {July 1976},
        numpages   = {10},
        publisher  = ACM,
        }

@Article{W:TSE86,
        author     = {Weyuker, E J},
        title      = {Axiomatizing Software Test Data Adequacy},
        journal    = TSE,
        year       = {1986},
        volume     = {12},
        number     = {12},
        pages      = {1128--1138},
        month      = dec,
        issn       = {0098-5589},
        address    = IEEEPressAddr,
        issue_date = {December 1986},
        numpages   = {11},
        publisher  = IEEE,
        }

@InProceedings{LDFW:ICSE12,
        author    = {Le Goues, Claire and Dewey-Vogt, Michael and Forrest, Stephanie and Weimer, Westley},
        title     = {A Systematic Study of Automated Program Repair: Fixing 55 out of 105 Bugs for \$8 Each},
        booktitle = ICSE,
        year      = {2012},
        pages     = {3--13},
        address   = IEEEPressAddr,
        month     = jun,
        publisher = IEEE,
        location  = {Zurich, Switzerland},
        numpages  = {11},
        }

@InProceedings{LKB:ASE14,
        author    = {Lillack, Max and K\"{a}stner, Christian and Bodden, Eric},
        title     = {Tracking Load-time Configuration Options},
        booktitle = ASE,
        year      = {2014},
        pages     = {445--456},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        location  = {Vasteras, Sweden},
        numpages  = {12},
        }

@Book{M:DAE06,
        title     = {Design and Analysis of Experiments},
        publisher = {John Wiley \& Sons},
        year      = {2006},
        author    = {Montgomery, Douglas C.},
        }

@Book{AS:SICP96,
        title     = {Structure and Interpretation of Computer Programs},
        publisher = MIT,
        year      = {1996},
        author    = {Abelson, Harold and Sussman, Gerald J.},
        address   = MITAddr,
        edition   = {2nd},
        }

@Book{ALSU:CPTT86,
        title     = {Compilers: Principles, Techniques, and Tools (2nd Edition)},
        publisher = AWL,
        year      = {2006},
        author    = {Aho, Alfred V. and Lam, Monica S. and Sethi, Ravi and Ullman, Jeffrey D.},
        address   = AWLAddr,
        }

@Book{CLRS:IA09,
        title     = {Introduction to Algorithms, Third Edition},
        publisher = MIT,
        year      = {2009},
        author    = {Cormen, Thomas H. and Leiserson, Charles E. and Rivest, Ronald L. and Stein, Clifford},
        edition   = {3rd},
        }

@Book{K:TACP197,
        title     = {The Art of Computer Programming, Volume 1 (3rd Ed.): Fundamental Algorithms},
        publisher = AWL,
        year      = {1997},
        author    = {Knuth, Donald E.},
        address   = {Redwood City, CA, USA},
        }

@Book{K:TACP297,
        title     = {The Art of Computer Programming, Volume 2 (3rd Ed.): Seminumerical Algorithms},
        publisher = AWL,
        year      = {1997},
        author    = {Knuth, Donald E.},
        address   = AWLAddr,
        }

@Book{K:TACP398,
        title     = {The Art of Computer Programming, Volume 3: (2Nd Ed.) Sorting and Searching},
        publisher = AWL,
        year      = {1998},
        author    = {Knuth, Donald E.},
        address   = {Redwood City, CA, USA},
        }

@Book{L:IDAA12,
        title     = {Introduction to the Design and Analysis of Algorithms (3rd Edition)},
        publisher = AWL,
        year      = {2012},
        author    = {Levitin, Anany V.},
        address   = AWLAddr,
        }

@Book{MSG:PIE12,
        title     = {Programming Interviews Exposed},
        publisher = {Wiley Publishing, Inc.},
        year      = {2012},
        author    = {Mongan, John and Suojanen, Noah and Giguere, Eric},
        }

@Book{P:LIP09,
        title     = {Language Implementation Patterns: Create Your Own Domain-Specific and General Programming Languages},
        publisher = {Pragmatic Bookshelf},
        year      = {2009},
        author    = {Parr, Terence},
        edition   = {1st},
        }

@Book{P:DAR07,
        title     = {The Definitive ANTLR Reference: Building Domain-Specific Languages},
        publisher = {Pragmatic Bookshelf},
        year      = {2007},
        author    = {Parr, Terence},
        }

@Book{P:DA4R13,
        title     = {The Definitive ANTLR 4 Reference},
        publisher = {Pragmatic Bookshelf},
        year      = {2013},
        author    = {Parr, Terence},
        edition   = {2nd},
        }

@InProceedings{MWKTS:ASE16,
        author    = {Meinicke, Jens and Wong, Chu-Pan and K\"{a}stner, Christian and Th\"{u}m, Thomas and Saake, Gunter},
        title     = {On Essential Configuration Complexity: Measuring Interactions in Highly-configurable Systems},
        booktitle = ASE,
        year      = {2016},
        pages     = {483--494},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        acmid     = {2970322},
        location  = {Singapore, Singapore},
        numpages  = {12},
        }

@Article{BK:SIGPLANNOT14,
  author     = {Bell, Jonathan and Kaiser, Gail},
  journal    = SIGPLANNOT,
  title      = {Phosphor: Illuminating Dynamic Data Flow in Commodity {JVM}s},
  year       = {2014},
  issn       = {0362-1340},
  month      = oct,
  number     = {10},
  pages      = {83--101},
  volume     = {49},
  acmid      = {2660212},
  address    = ACMAddr,
  issue_date = {October 2014},
  numpages   = {19},
  publisher  = ACM,
}

@InProceedings{KBK:AOSD11,
        author    = {Kim, Chang Hwan Peter and Batory, Don S. and Khurshid, Sarfraz},
        title     = {Reducing Combinatorics in Testing Product Lines},
        booktitle = AOSD,
        year      = {2011},
        pages     = {57--68},
        address   = ACMAddr,
        month     = mar,
        publisher = ACM,
        location  = {Porto de Galinhas, Brazil},
        numpages  = {12},
        }

@InProceedings{HHL:LION11,
        author    = {Hutter, Frank and Hoos, Holger H. and Leyton-Brown, Kevin},
        title     = {Sequential Model-based Optimization for General Algorithm Configuration},
        booktitle = {Proc. Int'l Conf. Learning and Intelligent Optimization},
        year      = {2011},
        pages     = {507--523},
        address   = SVBAddr,
        month     = jan,
        publisher = SV,
        location  = {Rome, Italy},
        numpages  = {17},
        }

@Article{WW:SS95,
        author    = {Wang, JC and Wu, CF Jeff},
        title     = {A hidden projection property of Plackett-Burman and related designs},
        journal   = {Statistica Sinica},
        year      = {1995},
        pages     = {235--250},
        publisher = {JSTOR},
        }

@InProceedings{SGSAC:ASE15,
        author    = {Sarkar, Atri and Guo, Jianmei and Siegmund, Norbert and Apel, Sven and Czarnecki, Krzysztof},
        title     = {Cost-Efficient Sampling for Performance Prediction of Configurable Systems},
        booktitle = ASE,
        year      = {2015},
        pages     = {342--352},
        address   = IEEEAddrW,
        month     = nov,
        publisher = IEEE,
        acmid     = {2916264},
        numpages  = {11},
        }

@InProceedings{LZLWZZ:ASE15,
        author    = {Lv, Fei and Zhang, Hongyu and Lou, Jian-guang and Wang, Shaowei and Zhang, Dongmei and Zhao, Jianjun},
        title     = {CodeHow: Effective Code Search Based on API Understanding and Extended Boolean Model},
        booktitle = ASE,
        year      = {2015},
        pages     = {260--270},
        address   = IEEEAddrW,
        month     = nov,
        publisher = IEEE,
        numpages  = {11},
        }

@InProceedings{BOR:ESECFSE13,
        author    = {B\"{o}hme, Marcel and Oliveira, Bruno C. d. S. and Roychoudhury, Abhik},
        title     = {Regression Tests to Expose Change Interaction Errors},
        booktitle = ESECFSE,
        year      = {2013},
        pages     = {334--344},
        address   = ACMAddr,
        month     = aug,
        publisher = ACM,
        location  = {Saint Petersburg, Russia},
        numpages  = {11},
        }

@Article{HXHL:AI14,
        author     = {Hutter, Frank and Xu, Lin and Hoos, Holger H. and Leyton-Brown, Kevin},
        title      = {Algorithm Runtime Prediction: Methods \& Evaluation},
        journal    = {Artif. Intell.},
        year       = {2014},
        volume     = {206},
        pages      = {79--111},
        month      = jan,
        issn       = {0004-3702},
        acmid      = {2562747},
        address    = {Essex, UK},
        issue_date = {January, 2014},
        numpages   = {33},
        publisher  = {Elsevier Science Publishers Ltd.},
        }

@InProceedings{XJFZPT:ESECFSE15,
        author    = {Xu, Tianyin and Jin, Long and Fan, Xuepeng and Zhou, Yuanyuan and Pasupathy, Shankar and Talwadker, Rukma},
        title     = {Hey, You Have Given Me Too Many Knobs!: Understanding and Dealing with Over-designed Configuration in System Software},
        booktitle = ESECFSE,
        year      = {2015},
        pages     = {307--319},
        address   = ACMAddr,
        month     = aug,
        publisher = ACM,
        location  = {Bergamo, Italy},
        numpages  = {13},
        }

@InProceedings{XZHZSYZP:SOSP13,
        author    = {Xu, Tianyin and Zhang, Jiaqi and Huang, Peng and Zheng, Jing and Sheng, Tianwei and Yuan, Ding and Zhou, Yuanyuan and Pasupathy, Shankar},
        title     = {Do Not Blame Users for Misconfigurations},
        booktitle = {Proc. Symp. Operating Systems Principles},
        year      = {2013},
        pages     = {244--259},
        address   = ACMAddr,
        month     = nov,
        publisher = ACM,
        location  = {Farminton, PA, USA},
        numpages  = {16},
        }

@InCollection{RSMFP:ICSE10,
        author    = {Reisner, Elnatan and Song, Charles and Ma, Kin-Keung and Foster, Jeffrey S. and Porter, Adam},
        title     = {Using Symbolic Evaluation to Understand Behavior in Configurable Software Systems},
        booktitle = ICSE,
        publisher = ACM,
        year      = {2010},
        pages     = {445--454},
        address   = ACMAddr,
        month     = may,
        location  = {Cape Town, South Africa},
        numpages  = {10},
        }

@InProceedings{BASO:ICMLA15,
        author    = {Bahnsen, A. C. and Aouada, D. and Stojanovic, A. and Ottersten, B.},
        title     = {Detecting Credit Card Fraud Using Periodic Features},
        booktitle = {Int'l Conf. Machine Learning and Applications (ICMLA)},
        year      = {2015},
        pages     = {208-213},
        address   = IEEEPressAddr,
        month     = dec,
        publisher = IEEE,
        location  = {Miami, FL, USA},
        }

@Book{K:PL03,
        title     = {Programming Languages: Application and Interpretation},
        publisher = {e-book},
        year      = {2003},
        author    = {Shriram Krishnamurthi},
        }

@InProceedings{SAB:SP10,
        author    = {Schwartz, Edward J. and Avgerinos, Thanassis and Brumley, David},
        title     = {All You Ever Wanted to Know About Dynamic Taint Analysis and Forward Symbolic Execution (but Might Have Been Afraid to Ask)},
        booktitle = {Proc. Symp. Security and Privacy (SP)},
        year      = {2010},
        pages     = {317--331},
        address   = IEEEAddrW,
        month     = may,
        publisher = IEEE,
        keywords  = {taint analysis, symbolic execution, dynamic analysis},
        location  = {Oakland, CA, USA},
        numpages  = {15},
        }

@InProceedings{ARFBBKLOM:PLDI14,
  author    = {Arzt, Steven and Rasthofer, Siegfried and Fritz, Christian and Bodden, Eric and Bartel, Alexandre and Klein, Jacques and Le Traon, Yves and Octeau, Damien and McDaniel, Patrick},
  booktitle = PLDI,
  title     = {Flow{D}roid: Precise Context, Flow, Field, Object-sensitive and Lifecycle-aware Taint Analysis for {A}ndroid Apps},
  year      = {2014},
  address   = ACMAddr,
  month     = jun,
  pages     = {259--269},
  publisher = ACM,
  location  = {Edinburgh, UK},
  numpages  = {11},
}

@Book{NNH:PPA10,
        title     = {Principles of Program Analysis},
        publisher = {Springer Publishing Company, Incorporated},
        year      = {2010},
        author    = {Nielson, Flemming and Nielson, Hanne R. and Hankin, Chris},
        }

@Misc{S:LNSA08,
        author = {Schwartzbach, Michael I.},
        title  = {Lecture Notes on Static Analysis},
        year   = {2008},
        }

@Report{NS:CMU05,
        author      = {Newsome, James and Song, Dawn},
        title       = {Dynamic Taint Analysis for Automatic Detection, Analysis, and Signature Generation of Exploits on Commodity Software},
        year        = {2005},
        institution = {Carnegie Mellon University},
        type        = {CMU-CS-04-140},
        }

@InProceedings{EGCCJMS:OSDI10,
        author    = {Enck, William and Gilbert, Peter and Chun, Byung-Gon and Cox, Landon P. and Jung, Jaeyeon and McDaniel, Patrick and Sheth, Anmol N.},
        title     = {TaintDroid: An Information-flow Tracking System for Realtime Privacy Monitoring on Smartphones},
        booktitle = {Proc. Conf. Operating Systems Design and Implementation (OSDI)},
        year      = {2010},
        pages     = {393--407},
        address   = {Berkeley, CA, USA},
        publisher = {USENIX Association},
        location  = {Vancouver, BC, Canada},
        numpages  = {15},
        }

@InProceedings{JVKSK:SEAMS17,
        author    = {Jamshidi, Pooyan and Velez, Miguel and K\"{a}stner, Christian and Siegmund, Norbert and Kawthekar, Prasad},
        title     = {Transfer Learning for Improving Model Predictions in Highly Configurable Software},
        booktitle = {Proc. Int'l Symp. Software Engineering for Adaptive and Self-Managing Systems (SEAMS)},
        year      = {2017},
        pages     = {31--41},
        address   = IEEEAddr,
        month     = may,
        publisher = IEEE,
        addendum  = {(23\% acceptance rate)},
        location  = {Buenos Aires, Argentina},
        numpages  = {11},
        }

@Article{GS:AS90,
        author    = {Gopen, George D and Swan, Judith A},
        title     = {The science of scientific writing},
        journal   = {American Scientist},
        year      = {1990},
        volume    = {78},
        number    = {6},
        pages     = {550--558},
        publisher = {JSTOR},
        }

@Book{D:TB13,
        title     = {Think Bayes},
        publisher = {" O'Reilly Media, Inc."},
        year      = {2013},
        author    = {Downey, Allen},
        }

@InProceedings{ML:PEPM00,
        author    = {Murphy, Brian R. and Lam, Monica S.},
        title     = {Program Analysis with Partial Transfer Functions},
        booktitle = {Proc. Workshop Partial Evaluation and Semantics-based Program Manipulation},
        year      = {2000},
        pages     = {94--103},
        address   = ACMAddr,
        month     = jan,
        publisher = ACM,
        location  = {Boston, MA, USA},
        numpages  = {10},
        }

@InProceedings{K:POPL73,
        author    = {Kildall, Gary A.},
        title     = {A Unified Approach to Global Program Optimization},
        booktitle = POPL,
        year      = {1973},
        pages     = {194--206},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        location  = {Boston, MA, USA},
        numpages  = {13},
        }

@InProceedings{KMJ:FSE16,
        author    = {Kang, Eunsuk and Milicevic, Aleksandar and Jackson, Daniel},
        title     = {Multi-representational Security Analysis},
        booktitle = FSE,
        year      = {2016},
        pages     = {181--192},
        address   = ACMAddr,
        month     = nov,
        publisher = ACM,
        location  = {Seattle, WA, USA},
        numpages  = {12},
        }

@Article{PYIS:CoRR16,
        author  = {Polikarpova, Nadia and Yang, Jean and Itzhaky, Shachar and Solar{-}Lezama, Armando},
        title   = {Type-Driven Repair for Information Flow Security},
        journal = {CoRR},
        year    = {2016},
        volume  = {abs/1607.03445},
        }

@InProceedings{DRS:ICSE16,
        author    = {Dhok, Monika and Ramanathan, Murali Krishna and Sinha, Nishant},
        title     = {Type-aware Concolic Testing of JavaScript Programs},
        booktitle = ICSE,
        year      = {2016},
        pages     = {168--179},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        acmid     = {2884859},
        location  = {Austin, TX, USA},
        numpages  = {12},
        }

@InProceedings{DJ:OOPSLA16,
        author    = {De Rosso, Santiago Perez and Jackson, Daniel},
        title     = {Purposes, Concepts, Misfits, and a Redesign of Git},
        booktitle = OOPSLA,
        year      = {2016},
        pages     = {292--310},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        location  = {Amsterdam, Netherlands},
        numpages  = {19},
        }

@InProceedings{NMSA:ESECFSE17,
  author    = {Nair, Vivek and Menzies, Tim and Siegmund, Norbert and Apel, Sven},
  booktitle = ESECFSE,
  title     = {Using Bad Learners to Find Good Configurations},
  year      = {2017},
  address   = ACMAddr,
  month     = aug,
  pages     = {257–267},
  publisher = ACM,
  series    = {ESEC/FSE 2017},
  location  = {Paderborn, Germany},
  numpages  = {11},
}

@InProceedings{AKTLS:GPCE16,
        author    = {Al-Hajjaji, Mustafa and Krieter, Sebastian and Th\"{u}m, Thomas and Lochau, Malte and Saake, Gunter},
        title     = {IncLing: Efficient Product-line Testing Using Incremental Pairwise Sampling},
        booktitle = GPCE,
        year      = {2016},
        pages     = {144--155},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        location  = {Amsterdam, Netherlands},
        numpages  = {12},
        }

@InProceedings{TMHL:ICSE16,
        author    = {Thongtanunam, Patanamon and McIntosh, Shane and Hassan, Ahmed E. and Iida, Hajimu},
        title     = {Revisiting Code Ownership and Its Relationship with Software Quality in the Scope of Modern Code Review},
        booktitle = ICSE,
        year      = {2016},
        pages     = {1039--1050},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Austin, TX, USA},
        numpages  = {12},
        }

@InProceedings{RDZL:GPCE16,
        author    = {Rothberg, Valentin and Dietrich, Christian and Ziegler, Andreas and Lohmann, Daniel},
        title     = {Towards Scalable Configuration Testing in Variable Software},
        booktitle = GPCE,
        year      = {2016},
        pages     = {156--167},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        location  = {Amsterdam, Netherlands},
        numpages  = {12},
        }

@Misc{MS:SPA17,
        author = {Møller Anders and Schwartzbach, Michael I.},
        title  = {Static Program Analysis},
        year   = {2017},
        }

@Book{LYBB:JVMS15,
  author    = {Lindholm, Tim and Yellin, Frank and Bracha, Gilad and Buckley, Alex},
  title     = {The Java Virtual Machine Specification, Java SE 8 Edition},
  year      = {2015},
  edition   = {1st},
  publisher = {Addison-Wesley Professional},
}

@Book{OSV:PS11,
        title     = {Programming in Scala: A Comprehensive Step-by-Step Guide, 2nd Edition},
        publisher = {Artima Incorporation},
        year      = {2011},
        author    = {Odersky, Martin and Spoon, Lex and Venners, Bill},
        address   = {USA},
        edition   = {2nd},
        }

@InProceedings{BORK:NDSS16,
        author    = {Buyukkayhan, Ahmet Salih and Onarlioglu, Kaan and Robertson, William and Kirda, Engin},
        title     = {CrossFire: An Analysis of Firefox Extension-Reuse Vulnerabilities},
        booktitle = {Network and Distributed System Security Symposium (NDSS)},
        year      = {2016},
        month     = feb,
        publisher = {Internet Society},
        location  = {San Diego, CA, USA},
        }

@PhdThesis{K:PHD10,
        author      = {Christian K{\"a}stner},
        title       = {Virtual Separation of Concerns: Toward Preprocessors 2.0},
        year        = {2010},
        address     = {Magdeburg, Germany},
        month       = may,
        note        = {Logos Verlag Berlin},
        institution = {University of Magdeburg},
        publisher   = {University of Magdeburg},
        }

@PhdThesis{S:PHD12,
        author = {Siegmund, Norbert},
        title  = {Measuring and Predicting Non-Functional Properties of Customizable Programs},
        school = {University of Magdeburg},
        year   = {2012},
        }

@Misc{ROS:AMCL16,
        author  = {ROS.org},
        title   = {amcl},
        date    = {2016-08-18},
        editor  = {FlorianSteinhardt},
        urldate = {2016-09-01},
        }

@Manual{B:ASM4JBEL11,
        title        = {ASM 4.0 A Java bytecode engineering library},
        author       = {Eric Bruneton},
        organization = {ASM},
        edition      = {2nd},
        month        = sep,
        year         = {2011},
        }

@Article{LKB:TSE18,
  author  = {Lillack, Max and K\"{a}stner, Christian and Bodden, Eric},
  journal = {IEEE Transactions on Software Engineering},
  title   = {Tracking Load-time Configuration Options},
  year    = {2018},
  issn    = {0098-5589},
  month   = {12},
  number  = {12},
  pages   = {1269-1291},
  volume  = {44},
}

@InProceedings{XJHZLJP:OSDI16,
        author    = {Xu, Tianyin and Jin, Xinxin and Huang, Peng and Zhou, Yuanyuan and Lu, Shan and Jin, Long and Pasupathy, Shankar},
        title     = {Early Detection of Configuration Errors to Reduce Failure Damage},
        booktitle = {Proc. Conf.Operating Systems Design and Implementation (OSDI)},
        year      = {2016},
        pages     = {619--634},
        address   = {Berkeley, CA, USA},
        month     = nov,
        publisher = {USENIX Association},
        location  = {Savannah, GA, USA},
        numpages  = {16},
        }

@InProceedings{RK:ICSE11,
        author    = {Rabkin, Ariel and Katz, Randy},
        title     = {Static Extraction of Program Configuration Options},
        booktitle = ICSE,
        year      = {2011},
        pages     = {131--140},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Waikiki, Honolulu, HI, USA},
        numpages  = {10},
        }

@Article{BSR:TSE04,
        author  = {D. Batory and J. N. Sarvela and A. Rauschmayer},
        title   = {Scaling Step-wise Refinement},
        journal = TSE,
        year    = {2004},
        volume  = {30},
        number  = {6},
        pages   = {355-371},
        month   = jun,
        issn    = {0098-5589},
        }

@Book{CN:SPL02,
        title     = {Software Product Lines},
        publisher = AWL,
        year      = {2002},
        author    = {Clements, Paul and Northrop, Linda},
        }

@Misc{TURTLEBOT:TURTLEBOT16,
        author  = {TurtleBot},
        title   = {What is TurtleBot?},
        urldate = {2016-09-01},
        }

@InProceedings{B:SPLC05,
        author    = {Batory, Don},
        title     = {Feature Models, Grammars, and Propositional Formulas},
        booktitle = SPLC,
        year      = {2005},
        pages     = {7--20},
        address   = SVBAddr,
        month     = sep,
        publisher = SV,
        location  = {Rennes, France},
        numpages  = {14},
        }

@Article{Z:SRDWMJ09,
        author  = {Zave, Pamela},
        title   = {Modularity in distributed feature composition},
        journal = {Software Requirements and Design: The Work of Michael Jackson},
        year    = {2009},
        pages   = {267--290},
        }

@InProceedings{TL:SANER17,
        author    = {Yutian Tang and Hareton Leung},
        title     = {StiCProb: A novel feature mining approach using conditional probability},
        booktitle = {Int'l Conf. Software Analysis, Evolution and Reengineering (SANER)},
        year      = {2017},
        pages     = {45-55},
        address   = IEEEAddr,
        month     = feb,
        publisher = IEEE,
        location  = {Klagenfurt, Austria},
        }

@Book{W:NDDB08,
        title     = {The Non-designer's Design Book, Third Edition},
        publisher = {Peachpit Press},
        year      = {2008},
        author    = {Williams, Robin},
        address   = {Berkeley, CA, USA},
        edition   = {Third},
        }

@Article{TZH:CoRR17,
        author  = {Tomkins, Andrew and Zhang, Min and Heavlin, William D.},
        title   = {Single versus Double Blind Reviewing at {WSDM} 2017},
        journal = {CoRR},
        year    = {2017},
        volume  = {abs/1702.00502},
        }

@InProceedings{SRP:ICSE17,
        author    = {Sedano, Todd and Ralph, Paul and P{\'e}raire, C{\'e}cile},
        title     = {Software Development Waste},
        booktitle = ICSE,
        year      = {2017},
        pages     = {130--140},
        address   = {Piscataway, NJ, USA},
        month     = may,
        publisher = IEEE,
        acmid     = {3097385},
        location  = {Buenos Aires, Argentina},
        numpages  = {11},
        }

@InProceedings{SDG:ICSE17,
        author    = {Souto, Sabrina and d'Amorim, Marcelo and Gheyi, Rohit},
        title     = {Balancing Soundness and Efficiency for Practical Testing of Configurable Systems},
        booktitle = ICSE,
        year      = {2017},
        pages     = {632--642},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {Buenos Aires, Argentina},
        numpages  = {11},
        }

@InProceedings{ICSME:HRAEDV15,
  author    = {A. Hora and R. Robbes and N. Anquetil and A. Etien and S. Ducasse and M. T. Valente},
  booktitle = ICSME,
  title     = {How do developers react to API evolution? The Pharo ecosystem case},
  year      = {2015},
  address   = IEEEAddr,
  month     = sep,
  pages     = {251-260},
  publisher = IEEE,
  location  = {Bremen, Germany},
  numpages  = {10},
}

@InProceedings{RSG:KDD16,
  author    = {Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle = {Proc. Int'l Conf. Knowledge Discovery and Data Mining (KDD)},
  title     = {"{W}hy Should {I} Trust You?": Explaining the Predictions of Any Classifier},
  year      = {2016},
  address   = ACMAddr,
  month     = aug,
  pages     = {1135--1144},
  publisher = ACM,
  location  = {San Francisco, CA, USA},
  numpages  = {10},
}

@InProceedings{SDFGCG:PLDI11,
  author    = {Sampson, Adrian and Dietl, Werner and Fortuna, Emily and Gnanapragasam, Danushen and Ceze, Luis and Grossman, Dan},
  title     = {EnerJ: Approximate Data Types for Safe and General Low-power Computation},
  booktitle = PLDI,
  year      = {2011},
  publisher = ACM,
  location  = {San Jose, CA, USA},
  month     = jun,
  pages     = {164--174},
  address   = ACMAddr,
  numpages  = {11},
}

@InProceedings{RHS:POPL95,
        author    = {Reps, Thomas and Horwitz, Susan and Sagiv, Mooly},
        title     = {Precise Interprocedural Dataflow Analysis via Graph Reachability},
        booktitle = POPL,
        year      = {1995},
        pages     = {49--61},
        address   = ACMAddr,
        month     = jan,
        publisher = ACM,
        location  = {San Francisco, CA, USA},
        numpages  = {13},
        }

@InProceedings{B:SOAP12,
        author    = {Bodden, Eric},
        title     = {Inter-procedural Data-flow Analysis with IFDS/IDE and Soot},
        booktitle = {Proc. Int'l Workshop State of the Art in Java Program Analysis (SOAP)},
        year      = {2012},
        pages     = {3--8},
        address   = ACMAddr,
        month     = jun,
        publisher = ACM,
        location  = {Beijing, China},
        numpages  = {6},
        }

@InProceedings{B:PLAS12,
  author    = {Bodden, Eric},
  booktitle = {Proc. Workshop Programming Languages and Analysis for Security (PLAS)},
  title     = {Position Paper: Static Flow-sensitive, Context-sensitive Information-flow Analysis for Software Product Lines},
  year      = {2012},
  address   = ACMAddr,
  month     = jun,
  pages     = {6:1--6:6},
  publisher = ACM,
  articleno = {6},
  location  = {Beijing, China},
  numpages  = {6},
}

@TechReport{FARBBKLOM:ECSPRIDE13,
        author      = {Christian Fritz and Steven Arzt and Siegfried Rasthofer and Eric Bodden and Alexandre Bartel and Jacques Klein and Yves le Traon and Damien Octeau and Patrick McDaniel},
        title       = {Highly Precise Taint Analysis for Android Applications},
        institution = {EC SPRIDE},
        year        = {2013},
        number      = {TUD-CS-2013-0113},
        month       = may,
        }

@InProceedings{ANWMS:ESECFSE17,
        author    = {Abdalkareem, Rabe and Nourry, Olivier and Wehaibi, Sultan and Mujahid, Suhaib and Shihab, Emad},
        title     = {Why Do Developers Use Trivial Packages? An Empirical Case Study on npm},
        booktitle = ESECFSE,
        year      = {2017},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        location  = {Paderborn, Germany},
        }

@Book{BO:CSPP15,
        title     = {Computer Systems: A Programmer's Perspective},
        publisher = {Pearson},
        year      = {2015},
        author    = {Bryant, Randal E. and O'Hallaron, David R.},
        edition   = {3rd},
        }

@InProceedings{JSVKPA:ASE17,
        author    = {Pooyan Jamshidi and Norbert Siegmund and Miguel Velez and Christian K\"{a}stner and Akshay Patel and Yuvraj Agarwal},
        title     = {Transfer Learning for Performance Modeling of Configurable Systems: An Exploratory Analysis},
        booktitle = ASE,
        year      = {2017},
        publisher = ACM,
        location  = {Urbana-Champaign, IL, USA},
        month     = oct,
        addendum  = {(21\% acceptance rate)},
        address   = ACMAddr,
        numpages  = {13},
        }

@InProceedings{TR:ASE14,
        author    = {Tarvo, Alexander and Reiss, Steven P.},
        title     = {Automated Analysis of Multithreaded Programs for Performance Modeling},
        booktitle = ASE,
        year      = {2014},
        pages     = {7--18},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        location  = {Vasteras, Sweden},
        numpages  = {12},
        }

@InProceedings{LRK:HICSS17,
        author    = {Christoph Luckeneder and Michael Rathmair and Hermann Kaindl},
        title     = {Investigating and Coordinating Safety-critical Feature Interactions in Automotive Systems Using Simulation},
        booktitle = {Hawaii Int'l Conf. System Sciences (HICSS)},
        year      = {2017},
        pages     = {10},
        month     = jan,
        location  = {Hilton Waikoloa Village, HI, USA},
        }

@Article{PF:CACM17,
        author     = {Price, Simon and Flach, Peter A.},
        title      = {Computational Support for Academic Peer Review: A Perspective from Artificial Intelligence},
        journal    = CACM,
        year       = {2017},
        volume     = {60},
        number     = {3},
        pages      = {70--79},
        month      = feb,
        address    = ACMAddr,
        issue_date = {March 2017},
        numpages   = {10},
        publisher  = ACM,
        }

@Article{FW:CACM86,
        author     = {Fleming, Philip J. and Wallace, John J.},
        title      = {How Not to Lie with Statistics: The Correct Way to Summarize Benchmark Results},
        journal    = CACM,
        year       = {1986},
        volume     = {29},
        number     = {3},
        pages      = {218--221},
        month      = mar,
        issn       = {0001-0782},
        acmid      = {5673},
        address    = ACMAddr,
        issue_date = {March 1986},
        numpages   = {4},
        publisher  = ACM,
        }

@Book{WRHORW:ESEAI00,
        title     = {Experimentation in Software Engineering: An Introduction},
        publisher = {Kluwer Academic Publishers},
        year      = {2000},
        author    = {Wohlin, Claes and Runeson, Per and H\"{o}st, Martin and Ohlsson, Magnus C. and Regnell, Bj\"{o}orn and Wessl{\'e}n, Anders},
        address   = {Norwell, MA, USA},
        }

@InProceedings{ZZB:PROMISEF11,
        author    = {Zeller, Andreas and Zimmermann, Thomas and Bird, Christian},
        title     = {Failure is a Four-letter Word: A Parody in Empirical Research},
        booktitle = {Proc. Int'l Conf. Predictive Models in Software Engineering (PROMISE)},
        year      = {2011},
        pages     = {5:1--5:7},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        articleno = {5},
        location  = {Banff, Alberta, Canada},
        numpages  = {7},
        }

@Article{SF:SCP15,
        author    = {Stol, Klaas-Jan and Fitzgerald, Brian},
        title     = {Theory-Oriented Software Engineering},
        journal   = {Science of Computer Programming},
        year      = {2015},
        volume    = {101},
        month     = apr,
        publisher = {Elsevier},
        }

@InProceedings{RVV:SCAM14,
        author    = {Raemaekers, Steven and van Deursen, Arie and Visser, Joost},
        title     = {Semantic Versioning Versus Breaking Changes: A Study of the Maven Repository},
        booktitle = SCAM,
        year      = {2014},
        pages     = {215--224},
        address   = {Washington, DC, USA},
        month     = sep,
        publisher = IEEE,
        location  = {Victoria, BC, Canada},
        numpages  = {10},
        }

@Book{S:EDA12,
        title     = {Experimental Design and Analysis},
        publisher = {Carnegie Mellon University},
        year      = {2012},
        author    = {Seltman, Howard J},
        }

@InProceedings{CNNBCH:CHI10,
  author    = {Chen, Jilin and Nairn, Rowan and Nelson, Les and Bernstein, Michael and Chi, Ed},
  title     = {Short and Tweet: Experiments on Recommending Content from Information Streams},
  booktitle = CHI,
  year      = {2010},
  pages     = {1185--1194},
  address   = ACMAddr,
  month     = apr,
  publisher = ACM,
  location  = {Atlanta, GA, USA},
  numpages  = {10},
}

@InProceedings{BKHT:FSE16,
        author    = {Bogart, Christopher and K\"{a}stner, Christian and Herbsleb, James and Thung, Ferdian},
        title     = {How to Break an API: Cost Negotiation and Community Values in Three Software Ecosystems},
        booktitle = FSE,
        year      = {2016},
        pages     = {109--120},
        address   = ACMAddr,
        month     = nov,
        publisher = ACM,
        acmid     = {2950325},
        location  = {Seattle, WA, USA},
        numpages  = {12},
        }

@InProceedings{GP:CSCW02,
        author    = {Grinter, Rebecca E. and Palen, Leysia},
        title     = {Instant Messaging in Teen Life},
        booktitle = CSCW,
        year      = {2002},
        pages     = {21--30},
        address   = ACMAddr,
        month     = nov,
        publisher = ACM,
        location  = {New Orleans, LA, USA},
        numpages  = {10},
        }

@InProceedings{MBZSJSPC:ICSE16,
        author    = {Manotas, Irene and Bird, Christian and Zhang, Rui and Shepherd, David and Jaspan, Ciera and Sadowski, Caitlin and Pollock, Lori and Clause, James},
        title     = {An Empirical Study of Practitioners' Perspectives on Green Software Engineering},
        booktitle = ICSE,
        year      = {2016},
        pages     = {237--248},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Austin, TX, USA},
        numpages  = {12},
        }

@Article{LT:JIE02,
        author    = {Lerner, Josh and Tirole, Jean},
        title     = {Some Simple Economics of Open Source},
        journal   = {The Journal of Industrial Economics},
        year      = {2002},
        volume    = {50},
        number    = {2},
        pages     = {197--234},
        issn      = {1467-6451},
        publisher = {Blackwell Publishers Ltd},
        }

@Article{D:JCMC07,
        author     = {Donath, Judith},
        title      = {Signals in Social Supernets},
        journal    = {J. Comp.-Med. Commun.},
        year       = {2007},
        volume     = {13},
        number     = {1},
        pages      = {231--251},
        month      = oct,
        issn       = {1083-6101},
        acmid      = {3047537},
        address    = {New York, NY, USA},
        issue_date = {October 2007},
        numpages   = {21},
        publisher  = {John Wiley \& Sons, Inc.},
        }

@InProceedings{MW:CSCW13,
        author    = {Marlow, Jennifer and Dabbish, Laura},
        title     = {Activity Traces and Signals in Software Developer Recruitment and Hiring},
        booktitle = CSCW,
        year      = {2013},
        pages     = {145--156},
        address   = ACMAddr,
        month     = feb,
        publisher = ACM,
        location  = {San Antonio, TX, USA},
        numpages  = {12},
        }

@InProceedings{VSDF:CSCW14,
        author    = {Vasilescu, Bogdan and Serebrenik, Alexander and Devanbu, Prem and Filkov, Vladimir},
        title     = {How Social Q\&\#38;A Sites Are Changing Knowledge Sharing in Open Source Software Communities},
        booktitle = CSCW,
        year      = {2014},
        pages     = {342--354},
        address   = ACMAddr,
        month     = feb,
        publisher = ACM,
        location  = {Baltimore, MA, USA},
        numpages  = {13},
        }

@InProceedings{TPTVF:ACSAC16,
        author    = {Tsankov, Petar and Pistoia, Marco and Tripp, Omer and Vechev, Martin and Ferrara, Pietro},
        title     = {FASE: Functionality-aware Security Enforcement},
        booktitle = {Proc. Conf. Computer Security Applications (ACSAC)},
        year      = {2016},
        pages     = {471--483},
        address   = ACMAddr,
        month     = dec,
        publisher = ACM,
        location  = {Los Angeles, CA, USA},
        numpages  = {13},
        }

@InProceedings{SZ:ICSE13,
        author    = {Sumner, William N. and Zhang, Xiangyu},
        title     = {Comparative Causality: Explaining the Differences Between Executions},
        booktitle = ICSE,
        year      = {2013},
        pages     = {272--281},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {San Francisco, CA, USA},
        numpages  = {10},
        }

@InProceedings{OBMS:ESECFSE17,
        author    = {Oh, Jeho and Batory, Don and Myers, Margaret and Siegmund, Norbert},
        title     = {Finding Near-optimal Configurations in Product Lines by Random Sampling},
        booktitle = ESECFSE,
        year      = {2017},
        pages     = {61--71},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        location  = {Paderborn, Germany},
        numpages  = {11},
        }

@InProceedings{RHGTVD:ICSE16,
        author    = {Ray, Baishakhi and Hellendoorn, Vincent and Godhane, Saheel and Tu, Zhaopeng and Bacchelli, Alberto and Devanbu, Premkumar},
        title     = {On the "Naturalness" of Buggy Code},
        booktitle = ICSE,
        year      = {2016},
        pages     = {428--439},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Austin, TX, USA},
        numpages  = {12},
        }

@InProceedings{CV:ESECFSE17,
        author    = {Coelho, Jailton and Valente, Marco Tulio},
        title     = {Why Modern Open Source Projects Fail},
        booktitle = ESECFSE,
        year      = {2017},
        pages     = {186--196},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        location  = {Paderborn, Germany},
        numpages  = {11},
        }

@InProceedings{WZSZH:ISSTA17,
        author    = {Wang, Bo and Xiong, Yingfei and Shi, Yangqingwei and Zhang, Lu and Hao, Dan},
        title     = {Faster Mutation Analysis via Equivalence Modulo States},
        booktitle = ISSTA,
        year      = {2017},
        pages     = {295--306},
        address   = ACMAddr,
        month     = jul,
        publisher = ACM,
        location  = {Santa Barbara, CA, USA},
        numpages  = {12},
        }

@Article{NV:CACM14,
        author     = {Narayanan, Arvind and Vallor, Shannon},
        title      = {Why Software Engineering Courses Should Include Ethics Coverage},
        journal    = CACM,
        year       = {2014},
        volume     = {57},
        number     = {3},
        pages      = {23--25},
        month      = mar,
        issn       = {0001-0782},
        acmid      = {2566966},
        address    = ACMAddr,
        issue_date = {March 2014},
        numpages   = {3},
        publisher  = ACM,
        }

@InProceedings{KHHJ:ICISS08,
        author    = {King, Dave and Hicks, Boniface and Hicks, Michael and Jaeger, Trent},
        title     = {Implicit Flows: Can'T Live with `Em, Can'T Live Without `Em},
        booktitle = {Proc. Int'l Conf. Information Systems Security (ICISS)},
        year      = {2008},
        pages     = {56--70},
        address   = SVBAddr,
        month     = dec,
        publisher = SV,
        location  = {Hyderabad, India},
        numpages  = {15},
        }

@InProceedings{JSMEB:ICSE13,
        author    = {Johnson, Brittany and Song, Yoonki and Murphy-Hill, Emerson and Bowdidge, Robert},
        title     = {Why Don't Software Developers Use Static Analysis Tools to Find Bugs?},
        booktitle = ICSE,
        year      = {2013},
        pages     = {672--681},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {San Francisco, CA, USA},
        numpages  = {10},
        }

@InProceedings{SBVLPO:ASE17,
        author    = {Scalabrino, Simone and Bavota, Gabriele and Vendome, Christopher and Linares-Vásquez, Mario and Poshyvanyk, Denys and Oliveto, Rocco},
        title     = {Automatically Assessing Code Understandability: How Far Are We?},
        booktitle = ASE,
        year      = {2017},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        location  = {Singapore, Singapore},
        numpages  = {11},
        }

@Article{GBE:SIGPLANNOT07,
  author     = {Georges, Andy and Buytaert, Dries and Eeckhout, Lieven},
  journal    = SIGPLANNOT,
  title      = {Statistically Rigorous {J}ava Performance Evaluation},
  year       = {2007},
  issn       = {0362-1340},
  month      = oct,
  number     = {10},
  pages      = {57--76},
  volume     = {42},
  acmid      = {1297033},
  address    = ACMAddr,
  issue_date = {October 2007},
  numpages   = {20},
  publisher  = ACM,
}

@Misc{VJKSSA-BRASS17,
        author       = {Velez, Miguel and Jamshidi, Pooyan and K\"{a}stner, Christian and Siegmund, Norbert and Sattler, Florian and Apel, Sven},
        title        = {White-Box Performance Discovery},
        howpublished = {Poster. BRASS PI Meeting},
        month        = nov,
        year         = {2017},
        keywords     = {rank5},
        location     = {Seattle, WA, USA},
        }

@InProceedings{MBDVDLT:ASE06,
        author    = {Mancinelli, Fabio and Boender, Jaap and di Cosmo, Roberto and Vouillon, Jerome and Durak, Berke and Leroy, Xavier and Treinen, Ralf},
        title     = {Managing the Complexity of Large Free and Open Source Package-Based Software Distributions},
        booktitle = ASE,
        year      = {2006},
        pages     = {199--208},
        address   = IEEEAddrW,
        month     = sep,
        publisher = IEEE,
        numpages  = {10},
        }

@InProceedings{VCGHLS:CASCON99,
        author    = {Vall{\'e}e-Rai, Raja and Co, Phong and Gagnon, Etienne and Hendren, Laurie and Lam, Patrick and Sundaresan, Vijay},
        title     = {Soot - a Java Bytecode Optimization Framework},
        booktitle = {Proc. Conf. Centre for Advanced Studies on Collaborative Research (CASCON)},
        year      = {1999},
        pages     = {13--},
        month     = nov,
        publisher = {IBM Press},
        acmid     = {782008},
        location  = {Mississauga, Ontario, Canada},
        }

@Article{BGBNT:CORR16,
        author  = {Balog, Matej and Gaunt, Alexander L and Brockschmidt, Marc and Nowozin, Sebastian and Tarlow, Daniel},
        title   = {Deepcoder: Learning to write programs},
        journal = {arXiv preprint arXiv:1611.01989},
        year    = {2016},
        }

@Article{BLC:AECS02,
        author  = {Bruneton, Eric and Lenglet, Romain and Coupaye, Thierry},
        title   = {ASM: a code manipulation tool to implement adaptable systems},
        journal = {Adaptable and extensible component systems},
        year    = {2002},
        volume  = {30},
        number  = {19},
        }

@InProceedings{JHF:SPLC12,
        author    = {Johansen, Martin Fagereng and Haugen, Oystein and Fleurey, Franck},
        title     = {An Algorithm for Generating T-wise Covering Arrays from Large Feature Models},
        booktitle = SPLC,
        year      = {2012},
        pages     = {46--55},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        location  = {Salvador, Brazil},
        numpages  = {10},
        }

@Article{C:MOS79,
        author     = {Chvatal, V.},
        title      = {A Greedy Heuristic for the Set-Covering Problem},
        journal    = {Math. Oper. Res.},
        year       = {1979},
        volume     = {4},
        number     = {3},
        pages      = {233--235},
        month      = aug,
        issn       = {0364-765X},
        acmid      = {2842451},
        address    = {Institute for Operations Research and the Management Sciences (INFORMS), Linthicum, MA, USA},
        issue_date = {August 1979},
        numpages   = {3},
        publisher  = {INFORMS},
        }

@Article{GCD:ESE11,
        author     = {Garvin, Brady J. and Cohen, Myra B. and Dwyer, Matthew B.},
        title      = {Evaluating Improvements to a Meta-heuristic Search for Constrained Interaction Testing},
        journal    = {Empirical Softw. Engg.},
        year       = {2011},
        volume     = {16},
        number     = {1},
        pages      = {61--102},
        month      = feb,
        issn       = {1382-3256},
        acmid      = {1960701},
        address    = {Hingham, MA, USA},
        issue_date = {February 2011},
        numpages   = {42},
        publisher  = {Kluwer Academic Publishers},
        }

@InProceedings{LKKOL:ECBS07,
        author    = {Lei, Yu and Kacker, Raghu and Kuhn, D. Richard and Okun, Vadim and Lawrence, James},
        title     = {IPOG: A General Strategy for T-Way Software Testing},
        booktitle = {Proc. Int'l Conf. and Workshops Engineering of Computer-Based Systems (ECBS)},
        year      = {2007},
        pages     = {549--556},
        address   = IEEEAddrW,
        month     = mar,
        publisher = IEEE,
        location  = {Tucson, AZ, USA},
        numpages  = {8},
        }

@InProceedings{OZML:VAMOS11,
        author    = {Oster, Sebastian and Zorcic, Ivan and Markert, Florian and Lochau, Malte},
        title     = {MoSo-PoLiTe: Tool Support for Pairwise and Model-based Software Product Line Testing},
        booktitle = VAMOS,
        year      = {2011},
        pages     = {79--82},
        address   = ACMAddr,
        month     = jan,
        publisher = ACM,
        location  = {Namur, Belgium},
        numpages  = {4},
        }

@Article{CDS:TSE08,
        author     = {Cohen, Myra B. and Dwyer, Matthew B. and Shi, Jiangfan},
        title      = {Constructing Interaction Test Suites for Highly-Configurable Systems in the Presence of Constraints: A Greedy Approach},
        journal    = TSE,
        year       = {2008},
        volume     = {34},
        number     = {5},
        pages      = {633--650},
        month      = sep,
        issn       = {0098-5589},
        address    = IEEEPressAddr,
        issue_date = {September 2008},
        numpages   = {18},
        publisher  = IEEE,
        }

@InProceedings{AKKGZARB:ICSE15,
        author    = {Avdiienko, Vitalii and Kuznetsov, Konstantin and Gorla, Alessandra and Zeller, Andreas and Arzt, Steven and Rasthofer, Siegfried and Bodden, Eric},
        title     = {Mining Apps for Abnormal Usage of Sensitive Data},
        booktitle = ICSE,
        year      = {2015},
        pages     = {426--436},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        acmid     = {2818808},
        location  = {Florence, Italy},
        numpages  = {11},
        }

@InProceedings{MKRGA:ICSE16,
        author    = {Medeiros, Fl\'{a}vio and K\"{a}stner, Christian and Ribeiro, M\'{a}rcio and Gheyi, Rohit and Apel, Sven},
        title     = {A Comparison of 10 Sampling Algorithms for Configurable Systems},
        booktitle = ICSE,
        year      = {2016},
        pages     = {643--654},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Austin, TX, USA},
        numpages  = {12},
        }

@InProceedings{SKKABRS:ICSE12,
        author    = {Siegmund, Norbert and Kolesnikov, Sergiy S. and K\"{a}stner, Christian and Apel, Sven and Batory, Don and Rosenm\"{u}ller, Marko and Saake, Gunter},
        title     = {Predicting Performance via Automated Feature-interaction Detection},
        booktitle = ICSE,
        year      = {2012},
        pages     = {167--177},
        address   = IEEEPressAddr,
        month     = jun,
        publisher = IEEE,
        acmid     = {2337243},
        location  = {Zurich, Switzerland},
        numpages  = {11},
        }

@InProceedings{JC:MASCOTS16,
  author    = {Jamshidi, Pooyan and Casale, Giuliano},
  booktitle = {Int'l Symp. Modeling, Analysis and Simulation of Computer and Telecommunication Systems (MASCOTS)},
  title     = {An Uncertainty-Aware Approach to Optimal Configuration of Stream Processing Systems},
  year      = {2016},
  month     = sep,
  pages     = {39--48},
  location  = {London, UK},
}

@InProceedings{SRF:ICSE16,
        author    = {Stol, Klaas-Jan and Ralph, Paul and Fitzgerald, Brian},
        title     = {Grounded Theory in Software Engineering Research: A Critical Review and Guidelines},
        booktitle = ICSE,
        year      = {2016},
        pages     = {120--131},
        address   = ACMAddr,
        publisher = ACM,
        location  = {Austin, TX, USA},
        numpages  = {12},
        }

@InProceedings{KKSKSZX:ASPLOS16,
  author    = {Kwon, Yonghwi and Kim, Dohyeong and Sumner, William Nick and Kim, Kyungtae and Saltaformaggio, Brendan and Zhang, Xiangyu and Xu, Dongyan},
  booktitle = ASPLOS,
  title     = {{LDX}: Causality Inference by Lightweight Dual Execution},
  year      = {2016},
  address   = ACMAddr,
  month     = apr,
  pages     = {503--515},
  publisher = ACM,
  location  = {Atlanta, GA, USA},
  numpages  = {13},
}

@InProceedings{SOOBGLKDFOLP:ICSE18,
        author    = {Sousa, Leonardo and Oliveira, Anderson and Oizumi, Willian and Barbosa, Simone and Garcia, Alessandro and Lee, Jaejoon and Kalinowski, Marcos and de Mello, Rafael and Fonseca, Baldoino and Oliveira, Roberto and Lucena, Carlos and Paes, Rodrigo},
        title     = {Identifying Design Problems in the Source Code: A Grounded Theory},
        booktitle = ICSE,
        year      = {2018},
        publisher = ACM,
        location  = {Gothenburg, Sweden},
        month     = may,
        pages     = {921--931},
        address   = ACMAddr,
        numpages  = {11},
        }

@InProceedings{DBFAB:CCS17,
        author    = {Derr, Erik and Bugiel, Sven and Fahl, Sascha and Acar, Yasemin and Backes, Michael},
        title     = {Keep Me Updated: An Empirical Study of Third-Party Library Updatability on Android},
        booktitle = {Proc. Conf. Computer and Communications Security (CCS)},
        year      = {2017},
        pages     = {2187--2200},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        location  = {Dallas, TX, USA},
        numpages  = {14},
        }

@Article{KSKGA:SOSYM18,
        author  = {Kolesnikov, Sergiy and Siegmund, Norbert and K{\"a}stner, Christian and Grebhahn, Alexander and Apel, Sven},
        title   = {Tradeoffs in modeling performance of highly configurable software systems},
        journal = {Software and System Modeling (SoSyM)},
        year    = {2018},
        month   = feb,
        day     = {08},
        }

@Article{LKKOL:STVR08,
        author     = {Lei, Yu and Kacker, Raghu and Kuhn, D. Richard and Okun, Vadim and Lawrence, James},
        title      = {IPOG-IPOG-D: Efficient Test Generation for Multi-way Combinatorial Testing},
        journal    = {Softw. Test. Verif. Reliab.},
        year       = {2008},
        volume     = {18},
        number     = {3},
        pages      = {125--148},
        month      = sep,
        issn       = {0960-0833},
        acmid      = {1405569},
        address    = {Chichester, UK},
        issue_date = {September 2008},
        numpages   = {24},
        publisher  = {John Wiley and Sons Ltd.},
        }

@InProceedings{PHZBW:EUROSYS11,
        author    = {Pathak, Abhinav and Hu, Y. Charlie and Zhang, Ming and Bahl, Paramvir and Wang, Yi-Min},
        title     = {Fine-grained Power Modeling for Smartphones Using System Call Tracing},
        booktitle = {Proc. Conf. Computer Systems (EuroSys)},
        year      = {2011},
        pages     = {153--168},
        address   = ACMAddr,
        month     = apr,
        publisher = ACM,
        location  = {Salzburg, Austria},
        numpages  = {16},
        }

@InProceedings{PHZ:EUROSYS12,
        author    = {Pathak, Abhinav and Hu, Y. Charlie and Zhang, Ming},
        title     = {Where is the Energy Spent Inside My App?: Fine Grained Energy Accounting on Smartphones with Eprof},
        booktitle = {Pro. Conf. Computer Systems (EuroSys},
        year      = {2012},
        pages     = {29--42},
        address   = ACMAddr,
        month     = apr,
        publisher = ACM,
        location  = {Bern, Switzerland},
        numpages  = {14},
        }

@Article{TMW:VLSI94,
        author  = {V. Tiwari and S. Malik and A. Wolfe},
        title   = {Power analysis of embedded software: a first step towards software power minimization},
        journal = {IEEE Trans. Very Large Scale Integration (VLSI) Systems},
        year    = {1994},
        volume  = {2},
        number  = {4},
        pages   = {437-445},
        month   = dec,
        issn    = {1063-8210},
        }

@Article{TAKSS:CSUR14,
        author     = {Th\"{u}m, Thomas and Apel, Sven and K\"{a}stner, Christian and Schaefer, Ina and Saake, Gunter},
        title      = {A Classification and Survey of Analysis Strategies for Software Product Lines},
        journal    = {ACM Comput. Surv. (CSUR)},
        year       = {2014},
        volume     = {47},
        number     = {1},
        pages      = {6:1--6:45},
        month      = jun,
        issn       = {0360-0300},
        address    = ACMAddr,
        articleno  = {6},
        issue_date = {July 2014},
        numpages   = {45},
        publisher  = ACM,
        }

@Book{KKL:ICT13,
        title     = {Introduction to Combinatorial Testing},
        publisher = {Chapman \& Hall/CRC},
        year      = {2013},
        author    = {Kuhn, D. Richard and Kacker, Raghu N. and Lei, Yu},
        edition   = {1st},
        }

@Article{NL:CSUR11,
        author     = {Nie, Changhai and Leung, Hareton},
        title      = {A Survey of Combinatorial Testing},
        journal    = {ACM Comput. Surv. (CSUR)},
        year       = {2011},
        volume     = {43},
        number     = {2},
        pages      = {11:1--11:29},
        month      = feb,
        issn       = {0360-0300},
        acmid      = {1883618},
        address    = ACMAddr,
        articleno  = {11},
        issue_date = {January 2011},
        numpages   = {29},
        publisher  = ACM,
        }

@Article{KHB:EJS12,
        author    = {Konietschke, Frank and Hothorn, Ludwig A and Brunner, Edgar},
        title     = {Rank-based multiple test procedures and simultaneous confidence intervals},
        journal   = {Electronic Journal of Statistics},
        year      = {2012},
        volume    = {6},
        pages     = {738--759},
        publisher = {The Institute of Mathematical Statistics and the Bernoulli Society},
        }

@Online{S:LJ17,
  author       = {Pierre-Yves Saumont},
  lastaccessed = {January 24, 2018},
  month        = feb,
  title        = {Lazy Computations in Java with a Lazy Type},
  url          = {www.sitepoint.com/lazy-computations-in-java-with-a-lazy-type/},
  year         = {2017},
}

@InProceedings{JSBM:ISSTA16,
        author    = {Jabbarvand, Reyhaneh and Sadeghi, Alireza and Bagheri, Hamid and Malek, Sam},
        title     = {Energy-aware Test-suite Minimization for Android Apps},
        booktitle = ISSTA,
        year      = {2016},
        pages     = {425--436},
        address   = ACMAddr,
        month     = jul,
        publisher = ACM,
        location  = {Saarbr\&\#252;cken, Germany},
        numpages  = {12},
        }

@Online{MV:ASE20SM,
  title = {See supplementary material in HotCRP},
}

@InProceedings{JCQR:ASE14,
        author    = {Jin, Dongpu and Cohen, Myra B. and Qu, Xiao and Robinson, Brian},
        title     = {PrefFinder: Getting the Right Preference in Configurable Software Systems},
        booktitle = ASE,
        year      = {2014},
        pages     = {151--162},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        location  = {Vasteras, Sweden},
        numpages  = {12},
        }

@InProceedings{JQCR:CICSE14,
        author    = {Jin, Dongpu and Qu, Xiao and Cohen, Myra B. and Robinson, Brian},
        title     = {Configurations Everywhere: Implications for Testing and Debugging in Practice},
        booktitle = {Companion Proc. Int'l Conf. Software Engineering},
        year      = {2014},
        pages     = {215--224},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Hyderabad, India},
        numpages  = {10},
        }

@InProceedings{SMM:PERCOM08,
        author    = {C. Seo and S. Malek and N. Medvidovic},
        title     = {Estimating the Energy Consumption in Pervasive Java-Based Systems},
        booktitle = {Proc. Int'l Conf. Pervasive Computing and Communications (PerCom)},
        year      = {2008},
        pages     = {243-247},
        month     = mar,
        }

@InProceedings{SMM:CBSE08,
        author    = {Seo, Chiyoung and Malek, Sam and Medvidovic, Nenad},
        title     = {Component-Level Energy Consumption Estimation for Distributed Java-Based Software Systems},
        booktitle = {Pro. Int'l Symposium Component-Based Software Engineering (CBSE)},
        year      = {2008},
        publisher = SV,
        location  = {Karlsruhe, Germany},
        month     = oct,
        pages     = {97--113},
        address   = SVBAddr,
        numpages  = {17},
        }

@InProceedings{GZBNBE:ESEM14,
        author    = {Gupta, Ashish and Zimmermann, Thomas and Bird, Christian and Nagappan, Nachiappan and Bhat, Thirumalesh and Emran, Syed},
        title     = {Mining Energy Traces to Aid in Software Development: An Empirical Case Study},
        booktitle = {Proc. Int'l Symposium Empirical Software Engineering and Measurement (ESEM)},
        year      = {2014},
        pages     = {40:1--40:8},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        articleno = {40},
        location  = {Torino, Italy},
        numpages  = {8},
        }

@InProceedings{SKA:ICSE17,
        author    = {Sayagh, Mohammed and Kerzazi, Noureddine and Adams, Bram},
        title     = {On Cross-stack Configuration Errors},
        booktitle = ICSE,
        year      = {2017},
        pages     = {255--265},
        address   = IEEEPressAddr,
        publisher = IEEE,
        location  = {Buenos Aires, Argentina},
        numpages  = {11},
        }

@InProceedings{LBBODP:MSR14,
        author    = {Linares-V\'{a}squez, Mario and Bavota, Gabriele and Bernal-C\'{a}rdenas, Carlos and Oliveto, Rocco and Di Penta, Massimiliano and Poshyvanyk, Denys},
        title     = {Mining Energy-greedy API Usage Patterns in Android Apps: An Empirical Study},
        booktitle = {Proc. Conf. Mining Software Repositories (MSR)},
        year      = {2014},
        pages     = {2--11},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Hyderabad, India},
        numpages  = {10},
        }

@InProceedings{DALC:ISSRE16,
  author    = {Z. Dong and A. Andrzejak and D. Lo and D. Costa},
  booktitle = {Proc. Int'l Symposium Software Reliability Engineering (ISSRE)},
  title     = {{ORPL}ocator: Identifying Read Points of Configuration Options via Static Analysis},
  year      = {2016},
  month     = oct,
  pages     = {185-195},
  publisher = IEEE,
}

@InProceedings{SA:SCAM15,
        author    = {M. Sayagh and B. Adams},
        title     = {Multi-layer software configuration: Empirical study on wordpress},
        booktitle = {Proc. Int'l Conf. Source Code Analysis and Manipulation (SCAM)},
        year      = {2015},
        pages     = {31-40},
        month     = sep,
        }

@InProceedings{GZHK:CHI18,
  author    = {Glassman, Elena and Zhangk, Tianyi and Hartmann, Björn and Kim, Miryung},
  title     = {Visualizing API Usage Examples at Scale},
  booktitle = CHI,
  year      = {2018},
  address   = ACMAddr,
  month     = apr,
  publisher = ACM,
  location  = {Montreal, Canada},
}

@TechReport{VJSSAK:ARCHIVE20,
  author      = {Velez, Miguel and Jamshidi, Pooyan and Sattler, Florian and Siegmund, Norbert and Apel, Sven and Kästner, Christian},
  institution = {arXiv},
  title       = {ConfigCrusher: Towards White-Box Performance Analysis for Configurable Systems},
  year        = {2020},
  month       = {7},
  number      = {1905.02066v2},
}

@InProceedings{OL:ASE13,
        author       = {P. Ohmann and B. Liblit},
        title        = {Lightweight control-flow instrumentation and postmortem analysis in support of debugging},
        booktitle    = ASE,
        year         = {2013},
        address      = ACMAddr,
        month        = nov,
        organization = IEEE,
        publisher    = ACM,
        location     = {Silicon Valley, CA, USA},
        }

@Article{Z:SIGSOFTNotes99,
        author     = {Zeller, Andreas},
        title      = {Yesterday, My Program Worked. Today, It Does Not. Why?},
        journal    = {SIGSOFT Softw. Eng. Notes},
        year       = {1999},
        volume     = {24},
        number     = {6},
        pages      = {253--267},
        month      = oct,
        issn       = {0163-5948},
        acmid      = {318946},
        address    = {New York, NY, USA},
        issue_date = {Nov. 1999},
        numpages   = {15},
        publisher  = {ACM},
        }

@InProceedings{MHBO:OOPSLA13,
        author    = {Miller, Heather and Haller, Philipp and Burmako, Eugene and Odersky, Martin},
        title     = {Instant Pickles: Generating Object-oriented Pickler Combinators for Fast and Extensible Serialization},
        booktitle = OOPSLA,
        year      = {2013},
        pages     = {183--202},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        location  = {Indianapolis, IN, USA},
        numpages  = {20},
        }

@InProceedings{RKHN:PLDI18,
        author    = {Raghothaman, Mukund and Kulkarni, Sulekha and Heo, Kihong and Naik, Mayur},
        title     = {Interactive program reasoning using Bayesian inference},
        booktitle = PLDI,
        year      = {2018},
        address   = ACMAddr,
        month     = jun,
        publisher = ACM,
        location  = {Philadelphia, PA, USA},
        numpages  = {11},
        }

@InProceedings{ZTZGBXZ:ASPLOS14,
        author    = {Zhang, Jiaqi and Renganarayana, Lakshminarayanan and Zhang, Xiaolan and Ge, Niyu and Bala, Vasanth and Xu, Tianyin and Zhou, Yuanyuan},
        title     = {EnCore: Exploiting System Environment and Correlation Information for Misconfiguration Detection},
        booktitle = ASPLOS,
        year      = {2014},
        pages     = {687--700},
        address   = ACMAddr,
        month     = mar,
        publisher = ACM,
        location  = {Salt Lake City, UT, USA},
        numpages  = {14},
        }

@InProceedings{JSSSL:PLDI12,
        author    = {Jin, Guoliang and Song, Linhai and Shi, Xiaoming and Scherpelz, Joel and Lu, Shan},
        title     = {Understanding and Detecting Real-world Performance Bugs},
        booktitle = PLDI,
        year      = {2012},
        pages     = {77--88},
        address   = ACMAddr,
        month     = jun,
        publisher = ACM,
        location  = {Beijing, China},
        numpages  = {12},
        }

@InProceedings{NJT:MSR13,
  author    = {Nistor, Adrian and Jiang, Tian and Tan, Lin},
  booktitle = MSR,
  title     = {Discovering, Reporting, and Fixing Performance Bugs},
  year      = {2013},
  address   = IEEEPressAddr,
  month     = may,
  pages     = {237--246},
  publisher = IEEE,
  location  = {San Francisco, CA, USA},
  numpages  = {10},
}

@InProceedings{HDGZX:ICSE12,
  author    = {Han, Shi and Dang, Yingnong and Ge, Song and Zhang, Dongmei and Xie, Tao},
  booktitle = ICSE,
  title     = {Performance Debugging in the Large via Mining Millions of Stack Traces},
  year      = {2012},
  address   = IEEEPressAddr,
  month     = jun,
  pages     = {145--155},
  publisher = IEEE,
  location  = {Zurich, Switzerland},
  numpages  = {11},
}

@InProceedings{LXC:ICSE14,
        author    = {Liu, Yepang and Xu, Chang and Cheung, Shing-Chi},
        title     = {Characterizing and Detecting Performance Bugs for Smartphone Applications},
        booktitle = ICSE,
        year      = {2014},
        series    = {ICSE 2014},
        pages     = {1013--1024},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        acmid     = {2568229},
        location  = {Hyderabad, India},
        numpages  = {12},
        }

@InProceedings{NCRL:ICSE15,
        author    = {Nistor, Adrian and Chang, Po-Chun and Radoi, Cosmin and Lu, Shan},
        title     = {Caramel: Detecting and Fixing Performance Problems That Have Non-intrusive Fixes},
        booktitle = ICSE,
        year      = {2015},
        pages     = {902--912},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {Florence, Italy},
        numpages  = {11},
        }

@InProceedings{HY:ESEM16,
        author    = {Han, Xue and Yu, Tingting},
        title     = {An Empirical Study on Performance Bugs for Highly Configurable Software Systems},
        booktitle = {Proc. Int'l Symposium Empirical Software Engineering and Measurement (ESEM)},
        year      = {2016},
        pages     = {23:1--23:10},
        address   = ACMAddr,
        month     = sep,
        publisher = ACM,
        articleno = {23},
        location  = {Ciudad Real, Spain},
        numpages  = {10},
        }

@InProceedings{SL:ICSE17,
        author    = {Song, Linhai and Lu, Shan},
        title     = {Performance Diagnosis for Inefficient Loops},
        booktitle = ICSE,
        year      = {2017},
        pages     = {370--380},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {Buenos Aires, Argentina},
        numpages  = {11},
        }

@InProceedings{KLYKYCHMNP:USENIXATC13,
        author    = {Kwon, Yongin and Lee, Sangmin and Yi, Hayoon and Kwon, Donghyun and Yang, Seungjun and Chun, Byung-Gon and Huang, Ling and Maniatis, Petros and Naik, Mayur and Paek, Yunheung},
        title     = {Mantis: Automatic Performance Prediction for Smartphone Applications},
        booktitle = {Proc. Conf. Annual Technical Conference (USENIX ATC)},
        year      = {2013},
        pages     = {297--308},
        address   = {Berkeley, CA, USA},
        month     = jun,
        publisher = {USENIX Association},
        location  = {San Jose, CA, USA},
        numpages  = {12},
        }

@InProceedings{AF:OSDI10,
        author    = {Attariyan, Mona and Flinn, Jason},
        title     = {Automating Configuration Troubleshooting with Dynamic Information Flow Analysis},
        booktitle = {Proc. Conf. Operating Systems Design and Implementation (OSDI)},
        year      = {2010},
        pages     = {237--250},
        address   = {Berkeley, CA, USA},
        month     = oct,
        publisher = {USENIX Association},
        location  = {Vancouver, BC, Canada},
        numpages  = {14},
        }

@MastersThesis{K:AFBPM17,
        author = {Christian Kapfhammer},
        title  = {Adjustable Family-based Performance Measurement},
        school = {University of Passau},
        year   = {2017},
        }

@InProceedings{ZE:ICSE13,
        author    = {Zhang, Sai and Ernst, Michael D.},
        title     = {Automated Diagnosis of Software Configuration Errors},
        booktitle = ICSE,
        year      = {2013},
        pages     = {312--321},
        address   = IEEEPressAddr,
        month     = may,
        publisher = IEEE,
        location  = {San Francisco, CA, USA},
        numpages  = {10},
        }

@InProceedings{ZE:ICSE14,
        author    = {Zhang, Sai and Ernst, Michael D.},
        title     = {Which Configuration Option Should I Change?},
        booktitle = ICSE,
        year      = {2014},
        pages     = {152--163},
        address   = ACMAddr,
        month     = may,
        publisher = ACM,
        location  = {Hyderabad, India},
        numpages  = {12},
        }

@InProceedings{JJIEHF:FSE14,
        author    = {Just, Ren{\'e} and Jalali, Darioush and Inozemtseva, Laura and Ernst, Michael D. and Holmes, Reid and Fraser, Gordon},
        title     = {Are Mutants a Valid Substitute for Real Faults in Software Testing?},
        booktitle = FSE,
        year      = {2014},
        pages     = {654--665},
        address   = ACMAddr,
        month     = nov,
        publisher = ACM,
        location  = {Hong Kong, China},
        numpages  = {12},
        }

@InProceedings{ZE:ISSTA15,
        author    = {Zhang, Sai and Ernst, Michael D.},
        title     = {Proactive Detection of Inadequate Diagnostic Messages for Software Configuration Errors},
        booktitle = ISSTA,
        year      = {2015},
        pages     = {12--23},
        address   = ACMAddr,
        month     = jul,
        publisher = ACM,
        location  = {Baltimore, MD, USA},
        numpages  = {12},
        }

@InProceedings{BK:ISSTA15,
        author    = {Bell, Jonathan and Kaiser, Gail},
        title     = {Dynamic Taint Tracking for Java with Phosphor (Demo)},
        booktitle = ISSTA,
        year      = {2015},
        pages     = {409--413},
        address   = ACMAddr,
        month     = jul,
        publisher = ACM,
        acmid     = {2784768},
        location  = {Baltimore, MD, USA},
        numpages  = {5},
        }

@InProceedings{SFB:PLDI07,
        author    = {Sridharan, Manu and Fink, Stephen J. and Bodik, Rastislav},
        title     = {Thin Slicing},
        booktitle = PLDI,
        year      = {2007},
        pages     = {112--122},
        address   = ACMAddr,
        month     = jun,
        publisher = ACM,
        acmid     = {1250748},
        location  = {San Diego, CA, USA},
        numpages  = {11},
        }

@InProceedings{KM:ICSE08,
        author    = {Ko, Andrew J. and Myers, Brad A.},
        title     = {Debugging Reinvented: Asking and Answering Why and Why Not Questions About Program Behavior},
        booktitle = ICSE,
        year      = {2008},
        pages     = {301--310},
        address   = ACMAddr,
        month     = oct,
        publisher = ACM,
        acmid     = {1368130},
        location  = {Leipzig, Germany},
        numpages  = {10},
        }

@InProceedings{DPH:ICSE12,
        author    = {Downs, John and Plimmer, Beryl and Hosking, John G.},
        title     = {Ambient Awareness of Build Status in Collocated Software Teams},
        booktitle = ICSE,
        year      = {2012},
        pages     = {507--517},
        address   = IEEEPressAddr,
        month     = jun,
        publisher = IEEE,
        acmid     = {2337283},
        location  = {Zurich, Switzerland},
        numpages  = {11},
        }

@Article{AMSBRW:TOSEM18,
  author     = {Abal, Iago and Melo, Jean and St\u{a}nciulescu, \c{S}tefan and Brabrand, Claus and Ribeiro, M\'{a}rcio and W\k{a}sowski, Andrzej},
  title      = {Variability Bugs in Highly Configurable Systems: A Qualitative Analysis},
  journal    = TOSEM,
  year       = {2018},
  volume     = {26},
  number     = {3},
  month      = jan,
  pages      = {10:1--10:34},
  issn       = {1049-331X},
  acmid      = {3149119},
  address    = ACMAddr,
  articleno  = {10},
  issue_date = {January 2018},
  numpages   = {34},
  publisher  = ACM,
}

@InProceedings{ADW:CHASE18,
        author    = {Alami, Adam and Dittrich, Yvonne and W\k{a}sowski, Andrzej},
        title     = {Influencers of Quality Assurance in an Open Source Community},
        booktitle = {Proc. Int'l Workshop Cooperative and Human Aspects of Software Engineering (CHASE)},
        year      = {2018},
        publisher = ACM,
        location  = {Gothenburg, Sweden},
        month     = may,
        pages     = {61--68},
        address   = ACMAddr,
        numpages  = {8},
        }

@InProceedings{WLHLSK:ASPLOS18,
        author    = {Wang, Shu and Li, Chi and Hoffmann, Henry and Lu, Shan and Sentosa, William and Kistijantoro, Achmad Imam},
        title     = {Understanding and Auto-Adjusting Performance-Sensitive Configurations},
        booktitle = ASPLOS,
        year      = {2018},
        pages     = {154--168},
        address   = ACMAddr,
        month     = mar,
        publisher = ACM,
        acmid     = {3173206},
        location  = {Williamsburg, VA, USA},
        numpages  = {15},
        }

@TechReport{ADJF:TR11,
        author      = {Thomas H. Austin and Tim Disney and Alan Jeffrey and Cormac Flanagan},
        title       = {Dynamic Information Flow Analysis for Featherweight JavaScript},
        institution = {University of California Santa Cruz},
        year        = {2011},
        }

@InProceedings{AF:PLAS09,
        author    = {Austin, Thomas H. and Flanagan, Cormac},
        title     = {Efficient Purely-dynamic Information Flow Analysis},
        booktitle = {Proc. Workshop Programming Languages and Analysis for Security (PLAS)},
        year      = {2009},
        pages     = {113--124},
        address   = ACMAddr,
        month     = jun,
        publisher = ACM,
        acmid     = {1554353},
        location  = {Dublin, Ireland},
        numpages  = {12},
        }

@InProceedings{TOMMGMMWM:MSR18,
        author    = {Middleton, Justin and Murphy-Hill, Emerson and Green, Demetrius and Meade, Adam and Mayer, Roger and White, David and McDonald, Steve},
        title     = {Which Contributions Predict Whether Developers Are Accepted into Github Teams},
        booktitle = MSR,
        year      = {2018},
        publisher = ACM,
        location  = {Gothenburg, Sweden},
        month     = may,
        pages     = {403--413},
        address   = ACMAddr,
        numpages  = {11},
        }

@InProceedings{AF:PLAS10,
        author    = {Austin, Thomas H. and Flanagan, Cormac},
        title     = {Permissive Dynamic Information Flow Analysis},
        booktitle = {Proc. Workshop Programming Languages and Analysis for Security (PLAS)},
        year      = {2010},
        pages     = {3:1--3:12},
        address   = ACMAddr,
        month     = jun,
        publisher = ACM,
        acmid     = {1814220},
        articleno = {3},
        location  = {Toronto, Canada},
        numpages  = {12},
        }

@InProceedings{AFA:APLAS12,
        author    = {Austin, Thomas H. and Flanagan, Cormac and Abadi, Mart{\'i}n},
        title     = {A Functional View of Imperative Information Flow},
        booktitle = {Asian Symp. Programming Languages and Systems (APLAS)},
        year      = {2012},
        editor    = {Jhala, Ranjit and Igarashi, Atsushi},
        pages     = {34--49},
        address   = {Berlin, Heidelberg},
        month     = dec,
        publisher = {Springer Berlin Heidelberg},
        location  = {Kyoto, Japan},
        }

@InProceedings{YHASFC:PLDI16,
        author    = {Yang, Jean and Hance, Travis and Austin, Thomas H. and Solar-Lezama, Armando and Flanagan, Cormac and Chong, Stephen},
        title     = {Precise, Dynamic Information Flow for Database-backed Applications},
        booktitle = PLDI,
        year      = {2016},
        pages     = {631--647},
        address   = ACMAddr,
        month     = jun,
        publisher = ACM,
        acmid     = {2908098},
        location  = {Santa Barbara, CA, USA},
        numpages  = {17},
        }

@InProceedings{AF:POPL12,
        author    = {Austin, Thomas H. and Flanagan, Cormac},
        title     = {Multiple Facets for Dynamic Information Flow},
        booktitle = POPL,
        year      = {2012},
        pages     = {165--178},
        address   = ACMAddr,
        month     = jan,
        publisher = ACM,
        acmid     = {2103677},
        location  = {Philadelphia, PA, USA},
        numpages  = {14},
        }

@InProceedings{JVKS:FSE18,
  author    = {Jamshidi, Pooyan and Velez, Miguel and K\"{a}stner, Christian and Siegmund, Norbert},
  title     = {Learning to Sample: Exploiting Similarities Across Environments to Learn Performance Models for Configurable Systems},
  booktitle = FSE,
  year      = {2018},
  publisher = ACM,
  location  = {Lake Buena Vista, FL, USA},
  month     = nov,
  pages     = {71--82},
  addendum  = {(21\% acceptance rate)},
  address   = ACMAddr,
  numpages  = {12},
}

@InProceedings{DALBSM:ISSTA17,
  author    = {Do, Lisa Nguyen Quang and Ali, Karim and Livshits, Benjamin and Bodden, Eric and Smith, Justin and Murphy-Hill, Emerson},
  title     = {Just-in-time Static Analysis},
  booktitle = ISSTA,
  year      = {2017},
  publisher = ACM,
  location  = {Santa Barbara, CA, USA},
  pages     = {307--317},
  address   = ACMAddr,
  numpages  = {11},
}

@InProceedings{QWR:ISSTA18,
        author    = {Qiu, Lina and Wang, Yingying and Rubin, Julia},
        title     = {Analyzing the Analyzers: FlowDroid/IccTA, AmanDroid, and DroidSafe},
        booktitle = ISSTA,
        year      = {2018},
        publisher = ACM,
        location  = {Amsterdam, Netherlands},
        pages     = {176--186},
        address   = ACMAddr,
        numpages  = {11},
        }

@InProceedings{B:ICSENIER18,
        author    = {Bodden, Eric},
        title     = {Self-adaptive Static Analysis},
        booktitle = {Proc. Int'l Conf. Software Engineering (ICSE): New Ideas and Emerging Results},
        year      = {2018},
        publisher = ACM,
        location  = {Gothenburg, Sweden},
        pages     = {45--48},
        address   = ACMAddr,
        numpages  = {4},
        }

@InProceedings{LSBM:ASE15,
        author    = {J. Lerch and J. Späth and E. Bodden and M. Mezini},
        title     = {Access-Path Abstraction: Scaling Field-Sensitive Data-Flow Analysis with Unbounded Access Paths (T)},
        booktitle = ASE,
        year      = {2015},
        publisher = IEEE,
        month     = nov,
        pages     = {619-629},
        address   = IEEEAddrW,
        }

@InProceedings{WZR:SOAP16,
        author    = {Wang, Yan and Zhang, Hailong and Rountev, Atanas},
        title     = {On the Unsoundness of Static Analysis for Android GUIs},
        booktitle = {Proc. Int'l Workshop State Of the Art in Program Analysis (SOAP)},
        year      = {2016},
        publisher = ACM,
        location  = {Santa Barbara, CA, USA},
        pages     = {18--23},
        address   = ACMAddr,
        numpages  = {6},
        }

@Online{MV:O,
        title = {Link to supplementary {GitHub} repository. {O}mitted for double-blind review.},
        }

@Article{YFCPDK:C14,
        author  = {C. Yilmaz and S. Fouché and M. B. Cohen and A. Porter and G. Demiroz and U. Koc},
        title   = {Moving Forward with Combinatorial Interaction Testing},
        journal = {Computer},
        year    = {2014},
        volume  = {47},
        number  = {2},
        month   = feb,
        pages   = {37-45},
        }

@Article{Y:TSE13,
        author  = {C. Yilmaz},
        title   = {Test Case-Aware Combinatorial Interaction Testing},
        journal = TSE,
        year    = {2013},
        volume  = {39},
        number  = {5},
        month   = may,
        pages   = {684-706},
        issn    = {0098-5589},
        }

@InProceedings{SPF:ICSE12,
        author    = {Song, Charles and Porter, Adam and Foster, Jeffrey S.},
        title     = {iTree: Efficiently Discovering High-coverage Configurations Using Interaction Trees},
        booktitle = ICSE,
        year      = {2012},
        publisher = IEEE,
        location  = {Zurich, Switzerland},
        month     = {6},
        pages     = {903--913},
        address   = IEEEAddr,
        numpages  = {11},
        }

@InProceedings{HBG:SRE11,
  author    = {A. Hervieu and B. Baudry and A. Gotlieb},
  booktitle = {Proc. Int'l Symposium Software Reliability Engineering},
  title     = {{PACOGEN}: Automatic Generation of Pairwise Test Configurations from Feature Models},
  year      = {2011},
  month     = nov,
  pages     = {120-129},
  issn      = {2332-6549},
}

@Article{HNADPB:ESE18,
  author    = {Halin, Axel and Nuttinck, Alexandre and Acher, Mathieu and Devroey, Xavier and Perrouin, Gilles and Baudry, Benoit},
  journal   = {Empirical Software Engineering},
  title     = {Test them all, is it worth it? Assessing configuration sampling on the {JH}ipster Web development stack},
  year      = {2018},
  month     = Jul,
  publisher = {Springer Verlag},
}

@InProceedings{CLO:ISSTA07,
        author    = {Clause, James and Li, Wanchun and Orso, Alessandro},
        title     = {Dytan: A Generic Dynamic Taint Analysis Framework},
        booktitle = ISSTA,
        year      = {2007},
        publisher = ACM,
        location  = {London, United Kingdom},
        pages     = {196--206},
        address   = ACMAddr,
        numpages  = {11},
        }

@InProceedings{AGPG:ASE15,
        author    = {Angerer, Florian and Grimmer, Andreas and Pr\"{a}hofer, Herbert and Gr\"{u}nbacher, Paul},
        title     = {Configuration-Aware Change Impact Analysis},
        booktitle = ASE,
        year      = {2015},
        publisher = IEEE,
        pages     = {385--395},
        address   = IEEEAddrW,
        numpages  = {11},
        }

@InProceedings{APLGG:SPLC14,
        author    = {Angerer, Florian and Pr\"{a}hofer, Herbert and Lettner, Daniela and Grimmer, Andreas and Gr\"{u}nbacher, Paul},
        title     = {Identifying Inactive Code in Product Lines with Configuration-aware System Dependence Graphs},
        booktitle = SPLC,
        year      = {2014},
        publisher = ACM,
        location  = {Florence, Italy},
        pages     = {52--61},
        address   = ACMAddr,
        numpages  = {10},
        }

@Article{MCC:CLSS17,
        author     = {Martnez, Salvador and Cosentino, Valerio and Cabot, Jordi},
        title      = {Model-based Analysis of Java EE Web Security Misconfigurations},
        journal    = {Comput. Lang. Syst. Struct.},
        year       = {2017},
        volume     = {49},
        number     = {C},
        month      = sep,
        pages      = {36--61},
        issn       = {1477-8424},
        address    = {Amsterdam, The Netherlands},
        issue_date = {September 2017},
        numpages   = {26},
        publisher  = {Elsevier Science Publishers B. V.},
        }

@InProceedings{AZCHS:CASCON14,
        author    = {Aggarwal, Karan and Zhang, Chenlei and Campbell, Joshua Charles and Hindle, Abram and Stroulia, Eleni},
        title     = {The Power of System Call Traces: Predicting the Software Energy Consumption Impact of Changes},
        booktitle = {Proc. Int'l Conf. Computer Science and Software Engineering (CASCON)},
        year      = {2014},
        publisher = {IBM Corp.},
        location  = {Markham, Ontario, Canada},
        pages     = {219--233},
        address   = {Riverton, NJ, USA},
        numpages  = {15},
        }

@InProceedings{RLT:SAS15,
        author    = {Marianna Rapoport and Ondrej Lhot{\'a}k and Frank Tip},
        title     = {Precise Data Flow Analysis in the Presence of Correlated Method Calls},
        booktitle = {SAS},
        year      = {2015},
        publisher = {Springer Berlin Heidelberg},
        pages     = {54--71},
        address   = {Berlin, Heidelberg},
        }

@InProceedings{LW:RV13,
        author    = {Lixin Li and Chao Wang},
        title     = {Dynamic Analysis and Debugging of Binary Code for Security Applications},
        booktitle = {RV},
        year      = {2013},
        }

@InProceedings{CB:ASE16,
        author    = {Christakis, Maria and Bird, Christian},
        title     = {What Developers Want and Need from Program Analysis: An Empirical Study},
        booktitle = ASE,
        year      = {2016},
        publisher = ACM,
        location  = {Singapore, Singapore},
        pages     = {332--343},
        address   = ACMAddr,
        numpages  = {12},
        }

@InProceedings{BJMVDDE:ASE15,
        author    = {Barros, Paulo and Just, Rene and Millstein, Suzanne and Vines, Paul and Dietl, Werner and dAmorim, Marcelo and Ernst, Michael D.},
        title     = {Static Analysis of Implicit Control Flow: Resolving Java Reflection and Android Intents (T)},
        booktitle = ASE,
        year      = {2015},
        publisher = IEEE,
        pages     = {669--679},
        address   = IEEEAddrW,
        numpages  = {11},
        }

@InProceedings{B:ICSESEET18,
  author    = {Borsotti, Valeria},
  title     = {Barriers to Gender Diversity in Software Development Education: Actionable Insights from a Danish Case Study},
  booktitle = {Proc. Int'l Conf. Software Engineering: Software Engineering Education and Training (ICSE-SEET)},
  year      = {2018},
  publisher = ACM,
  location  = {Gothenburg, Sweden},
  month     = may,
  isbn      = {978-1-4503-5660-2},
  pages     = {146--152},
  address   = ACMAddr,
  numpages  = {7},
}

@InProceedings{ST:WISEC14,
  author    = {Sun, Mengtao and Tan, Gang},
  title     = {NativeGuard: Protecting Android Applications from Third-party Native Libraries},
  booktitle = {Proc. Conf. Security and Privacy in Wireless \&\#38; Mobile Networks (WiSec)},
  year      = {2014},
  publisher = ACM,
  location  = {Oxford, United Kingdom},
  month     = {7},
  isbn      = {978-1-4503-2972-9},
  pages     = {165--176},
  address   = ACMAddr,
  numpages  = {12},
}

@Book{B:EJ08,
  author    = {Bloch, Joshua},
  title     = {Effective Java\texttrademark, Second Edition},
  year      = {2008},
  edition   = {Second},
  publisher = {Prentice Hall Press},
  isbn      = {9780137150021},
  address   = {Upper Saddle River, NJ, USA},
}

@Book{B:EJ18,
  author    = {Bloch, Joshua},
  title     = {Effective Java\texttrademark, Third Edition},
  year      = {2018},
  edition   = {Third},
  publisher = {Addison-Wesley},
}

@InProceedings{BMNBB:ICSME18,
  author    = {Businge, John and Moses, O and Nadi, Sarah and Bainomugisha, Engineer and Berger, Thorsten},
  booktitle = ICSME,
  title     = {Clone-Based Variability Managementin the Android Ecosystem},
  year      = {2018},
  month     = sep,
  comment   = {TODO},
  location  = {Madrid, Spain},
}

@InProceedings{CCRC:ASE18,
  author    = {Cashman, Mikaela and Cohen, Myra B. and Ranjan, Priya and Cottingham, Robert W.},
  title     = {Navigating the Maze: The Impact of Configurability in Bioinformatics Software},
  booktitle = ASE,
  year      = {2018},
  publisher = ACM,
  location  = {Montpellier, France},
  month     = {9},
  pages     = {757--767},
  address   = ACMAddr,
  numpages  = {11},
}

@InProceedings{SPWG:ICSE18,
  author    = {Steinmacher, Igor and Pinto, Gustavo and Wiese, Igor Scaliante and Gerosa, Marco A.},
  title     = {Almost There: A Study on Quasi-contributors in Open Source Software Projects},
  booktitle = ICSE,
  year      = {2018},
  publisher = ACM,
  location  = {Gothenburg, Sweden},
  month     = may,
  pages     = {256--266},
  address   = ACMAddr,
  numpages  = {11},
}

@InProceedings{VR:CHI16,
  author    = {Vaniea, Kami and Rashidi, Yasmeen},
  title     = {Tales of Software Updates: The Process of Updating Software},
  booktitle = CHI,
  year      = {2016},
  publisher = ACM,
  location  = {San Jose, CA, USA},
  month     = {5},
  pages     = {3215--3226},
  address   = ACMAddr,
  numpages  = {12},
}

@InProceedings{MNMBS:ASE18,
  author    = {Mukelabai, Mukelabai and Ne\v{s}i\'{c}, Damir and Maro, Salome and Berger, Thorsten and Stegh\"{o}fer, Jan-Philipp},
  title     = {Tackling Combinatorial Explosion: A Study of Industrial Needs and Practices for Analyzing Highly Configurable Systems},
  booktitle = ASE,
  year      = {2018},
  publisher = ACM,
  location  = {Montpellier, France},
  month     = {9},
  pages     = {155--166},
  address   = ACMAddr,
  numpages  = {12},
}

@Article{BKRSF:TSE18,
  author  = {A. Barcomb and A. Kaufmann and D. Riehle and K. Stol and B. Fitzgerald},
  title   = {Uncovering the Periphery: A Qualitative Survey of Episodic Volunteering in Free/Libre and Open Source Software Communities},
  journal = {IEEE Transactions on Software Engineering},
  year    = {2018},
  month   = {10},
  pages   = {1-1},
}

@Book{LYBB:JVMS13,
  author    = {Lindholm, Tim and Yellin, Frank and Bracha, Gilad and Buckley, Alex},
  title     = {The Java Virtual Machine Specification, Java SE 7 Edition},
  year      = {2013},
  edition   = {1st},
  publisher = {Addison-Wesley Professional},
}

@InProceedings{NSML:ICSE13,
  author    = {Nistor, Adrian and Song, Linhai and Marinov, Darko and Lu, Shan},
  title     = {Toddler: Detecting Performance Problems via Similar Memory-access Patterns},
  booktitle = ICSE,
  year      = {2013},
  publisher = IEEE,
  location  = {San Francisco, CA, USA},
  month     = {5},
  pages     = {562--571},
  address   = IEEEPressAddr,
  numpages  = {10},
}

@InProceedings{AZSH:CSCW17,
  author    = {Arciniegas-Mendez, Maryi and Zagalsky, Alexey and Storey, Margaret-Anne and Hadwin, Allyson Fiona},
  title     = {Using the Model of Regulation to Understand Software Development Collaboration Practices and Tool Support},
  booktitle = CSCW,
  year      = {2017},
  publisher = ACM,
  location  = {Portland, OR, USA},
  month     = {2},
  isbn      = {978-1-4503-4335-0},
  pages     = {1049--1065},
  address   = ACMAddr,
  numpages  = {17},
}

@InProceedings{ZLGBMLSY:SOCC17,
  author    = {Zhu, Yuqing and Liu, Jianxun and Guo, Mengying and Bao, Yungang and Ma, Wenlong and Liu, Zhuoyue and Song, Kunpeng and Yang, Yingchun},
  title     = {BestConfig: Tapping the Performance Potential of Systems via Automatic Configuration Tuning},
  booktitle = {Proc. Symposium Cloud Computing (SoCC)},
  year      = {2017},
  publisher = ACM,
  location  = {Santa Clara, CA, USA},
  month     = {9},
  isbn      = {978-1-4503-5028-0},
  pages     = {338--350},
  address   = ACMAddr,
  numpages  = {13},
}

@Article{ABDS:CSUR18,
  author     = {Allamanis, Miltiadis and Barr, Earl T. and Devanbu, Premkumar and Sutton, Charles},
  title      = {A Survey of Machine Learning for Big Code and Naturalness},
  journal    = {ACM Computing Surveys (CSUR)},
  year       = {2018},
  volume     = {51},
  number     = {4},
  month      = jul,
  pages      = {81:1--81:37},
  issn       = {0360-0300},
  address    = ACMAddr,
  articleno  = {81},
  issue_date = {September 2018},
  numpages   = {37},
  publisher  = ACM,
}

@Article{HMGB:IST16,
  author    = {Hervieu, Aymeric and Marijan, Dusica and Gotlieb, Arnaud and Baudry, Benoit},
  journal   = {{Information and Software Technology}},
  title     = {{Optimal Minimisation of Pairwise-covering Test Configurations Using Constraint Programming}},
  year      = {2016},
  month     = Mar,
  pages     = {129 - 146},
  volume    = {71},
  publisher = {Elsevier},
}

@InProceedings{AMN:SOAP17,
  author    = {Andreasen, Esben Sparre and M{\o}ller, Anders and Nielsen, Benjamin Barslev},
  booktitle = {Proc. Int'l Workshop State Of the Art in Program Analysis (SOAP)},
  title     = {Systematic Approaches for Increasing Soundness and Precision of Static Analyzers},
  year      = {2017},
  address   = ACMAddr,
  month     = {6},
  pages     = {31--36},
  publisher = ACM,
  acmid     = {3088521},
  doi       = {10.1145/3088515.3088521},
  isbn      = {978-1-4503-5072-3},
  location  = {Barcelona, Spain},
  numpages  = {6},
}

@Article{SAB:ACMPL17,
  author     = {Sp\"{a}th, Johannes and Ali, Karim and Bodden, Eric},
  journal    = {Proc. ACM Program. Lang.},
  title      = {IDEal: Efficient and Precise Alias-aware Dataflow Analysis},
  year       = {2017},
  issn       = {2475-1421},
  month      = oct,
  number     = {OOPSLA},
  pages      = {99:1--99:27},
  volume     = {1},
  acmid      = {3133923},
  address    = ACMAddr,
  articleno  = {99},
  doi        = {10.1145/3133923},
  issue_date = {October 2017},
  numpages   = {27},
  publisher  = ACM,
}

@InProceedings{GZL:ESECFSE17,
  author    = {Garbervetsky, Diego and Zoppi, Edgardo and Livshits, Benjamin},
  booktitle = ESECFSE,
  title     = {Toward Full Elasticity in Distributed Static Analysis: The Case of Callgraph Analysis},
  year      = {2017},
  address   = ACMAddr,
  month     = {9},
  pages     = {442--453},
  publisher = ACM,
  acmid     = {3106261},
  doi       = {10.1145/3106237.3106261},
  isbn      = {978-1-4503-5105-8},
  location  = {Paderborn, Germany},
  numpages  = {12},
}

@InProceedings{WPXCZZ:SPLC13,
  author    = {Wang, Bo and Passos, Leonardo and Xiong, Yingfei and Czarnecki, Krzysztof and Zhao, Haiyan and Zhang, Wei},
  booktitle = SPLC,
  title     = {SmartFixer: Fixing Software Configurations Based on Dynamic Priorities},
  year      = {2013},
  address   = ACMAddr,
  month     = {8},
  pages     = {82--90},
  publisher = ACM,
  acmid     = {2491640},
  doi       = {10.1145/2491627.2491640},
  isbn      = {978-1-4503-1968-3},
  location  = {Tokyo, Japan},
  numpages  = {9},
}

@InProceedings{HXC:VAMOS12,
  author    = {Hubaux, Arnaud and Xiong, Yingfei and Czarnecki, Krzysztof},
  booktitle = VAMOS,
  title     = {A User Survey of Configuration Challenges in {L}inux and e{C}os},
  year      = {2012},
  address   = ACMAddr,
  month     = jan,
  pages     = {149--155},
  publisher = ACM,
  acmid     = {2110164},
  isbn      = {978-1-4503-1058-1},
  location  = {Leipzig, Germany},
  numpages  = {7},
}

@InProceedings{ZS:POPL17,
  author    = {Zhang, Qirun and Su, Zhendong},
  booktitle = POPL,
  title     = {Context-sensitive Data-dependence Analysis via Linear Conjunctive Language Reachability},
  year      = {2017},
  address   = ACMAddr,
  month     = {1},
  pages     = {344--358},
  publisher = ACM,
  acmid     = {3009848},
  doi       = {10.1145/3009837.3009848},
  isbn      = {978-1-4503-4660-3},
  location  = {Paris, France},
  numpages  = {15},
}

@Article{SD:JSS18,
  author  = {Souto, S. and d'Amorim, M.},
  title   = {Time-space efficient regression testing for configurable systems},
  journal = {Journal of Systems and Software},
  year    = {2018},
}

@InProceedings{SHGDPECYCD:NIPS15,
  author    = {Sculley, D. and Holt, Gary and Golovin, Daniel and Davydov, Eugene and Phillips, Todd and Ebner, Dietmar and Chaudhary, Vinay and Young, Michael and Crespo, Jean-Francois and Dennison, Dan},
  title     = {Hidden Technical Debt in Machine Learning Systems},
  booktitle = {Proc. Int'l Conf. Neural Information Processing Systems (NIPS)},
  year      = {2015},
  publisher = MIT,
  location  = {Montreal, Canada},
  month     = {12},
  pages     = {2503--2511},
  address   = MITAddr,
  numpages  = {9},
}

@InProceedings{MWX:ISSTA17,
  author    = {Mostafa, Shaikh and Wang, Xiaoyin and Xie, Tao},
  title     = {PerfRanker: Prioritization of Performance Regression Tests for Collection-intensive Software},
  booktitle = ISSTA,
  year      = {2017},
  publisher = ACM,
  location  = {Santa Barbara, CA, USA},
  month     = {7},
  isbn      = {978-1-4503-5076-1},
  pages     = {23--34},
  address   = ACMAddr,
  numpages  = {12},
}

@Article{YP:EMSE18,
  author     = {Yu, Tingting and Pradel, Michael},
  title      = {Pinpointing and Repairing Performance Bottlenecks in Concurrent Programs},
  journal    = {Empirical Softw. Eng.},
  year       = {2018},
  volume     = {23},
  number     = {5},
  month      = oct,
  pages      = {3034--3071},
  issn       = {1382-3256},
  address    = {Norwell, MA, USA},
  issue_date = {October 2018},
  numpages   = {38},
  publisher  = {Kluwer Academic Publishers},
}

@InProceedings{CLBKMG:ICSECP18,
  author    = {Cito, J\"{u}rgen and Leitner, Philipp and Bosshard, Christian and Knecht, Markus and Mazlami, Genc and Gall, Harald C.},
  booktitle = {Proc. Int'l Conf. Software Engineering: Companion Proceeedings},
  title     = {Performance{H}at: Augmenting Source Code with Runtime Performance Traces in the {IDE}},
  year      = {2018},
  address   = ACMAddr,
  pages     = {41--44},
  publisher = ACM,
  isbn      = {978-1-4503-5663-3},
  location  = {Gothenburg, Sweden},
  numpages  = {4},
}

@Article{CAPPJ:TACO15,
  author     = {Castro, Pablo De Oliveira and Akel, Chadi and Petit, Eric and Popov, Mihail and Jalby, William},
  title      = {CERE: LLVM-Based Codelet Extractor and REplayer for Piecewise Benchmarking and Optimization},
  journal    = {ACM Trans. Archit. Code Optim. (TACO)},
  year       = {2015},
  volume     = {12},
  number     = {1},
  month      = apr,
  pages      = {6:1--6:24},
  issn       = {1544-3566},
  address    = ACMAddr,
  articleno  = {6},
  issue_date = {April 2015},
  numpages   = {24},
  publisher  = ACM,
}

@Article{G:CAMC16,
  author     = {Gregg, Brendan},
  title      = {The Flame Graph},
  journal    = CACM,
  year       = {2016},
  volume     = {59},
  number     = {6},
  pages      = {48--57},
  month      = may,
  issn       = {0001-0782},
  address    = ACMAddr,
  issue_date = {June 2016},
  numpages   = {10},
  publisher  = ACM,
}

@InProceedings{HYL:ASE18,
  author    = {Han, Xue and Yu, Tingting and Lo, David},
  title     = {PerfLearner: Learning from Bug Reports to Understand and Generate Performance Test Frames},
  booktitle = ASE,
  year      = {2018},
  publisher = ACM,
  location  = {Montpellier, France},
  month     = {9},
  isbn      = {978-1-4503-5937-5},
  pages     = {17--28},
  address   = ACMAddr,
  numpages  = {12},
}

@InProceedings{PBW:FSE18,
  author    = {Pauck, Felix and Bodden, Eric and Wehrheim, Heike},
  booktitle = FSE,
  title     = {Do Android Taint Analysis Tools Keep Their Promises?},
  year      = {2018},
  address   = ACMAddr,
  month     = {11},
  pages     = {331--341},
  publisher = ACM,
  acmid     = {3236029},
  doi       = {10.1145/3236024.3236029},
  isbn      = {978-1-4503-5573-5},
  location  = {Lake Buena Vista, FL, USA},
  numpages  = {11},
}

@InProceedings{PCAM:ASIACCS18,
  author    = {Pariwono, Elkana and Chiba, Daiki and Akiyama, Mitsuaki and Mori, Tatsuya},
  title     = {Don'T Throw Me Away: Threats Caused by the Abandoned Internet Resources Used by Android Apps},
  booktitle = {Proc. Asia Conf. Computer and Communications Security (ASIACCS)},
  year      = {2018},
  publisher = ACM,
  location  = {Incheon, Republic of Korea},
  month     = {6},
  isbn      = {978-1-4503-5576-6},
  pages     = {147--158},
  doi       = {10.1145/3196494.3196554},
  url       = {http://doi.acm.org/10.1145/3196494.3196554},
  acmid     = {3196554},
  address   = ACMAddr,
  numpages  = {12},
}

@Article{BT:OOPSLA18,
  author     = {Bornholt, James and Torlak, Emina},
  title      = {Finding Code That Explodes Under Symbolic Evaluation},
  journal    = OOPSLA,
  year       = {2018},
  volume     = {2},
  month      = oct,
  pages      = {149:1--149:26},
  issn       = {2475-1421},
  doi        = {10.1145/3276519},
  url        = {http://doi.acm.org/10.1145/3276519},
  address    = ACMAddr,
  articleno  = {149},
  issue_date = {November 2018},
  numpages   = {26},
  publisher  = ACM,
}

@InProceedings{MLLZG:FSE18,
  author    = {Ma, Shiqing and Liu, Yingqi and Lee, Wen-Chuan and Zhang, Xiangyu and Grama, Ananth},
  title     = {MODE: Automated Neural Network Model Debugging via State Differential Analysis and Input Selection},
  booktitle = ESECFSE,
  year      = {2018},
  publisher = ACM,
  location  = {Lake Buena Vista, FL, USA},
  month     = {11},
  isbn      = {978-1-4503-5573-5},
  pages     = {175--186},
  url       = {http://doi.acm.org/10.1145/3236024.3236082},
  address   = ACMAddr,
  numpages  = {12},
}

@InProceedings{CLZMDMBN:ESECFSE17,
  author    = {Chaparro, Oscar and Lu, Jing and Zampetti, Fiorella and Moreno, Laura and Di Penta, Massimiliano and Marcus, Andrian and Bavota, Gabriele and Ng, Vincent},
  title     = {Detecting Missing Information in Bug Descriptions},
  booktitle = ESECFSE,
  year      = {2017},
  publisher = ACM,
  location  = {Paderborn, Germany},
  month     = {9},
  isbn      = {978-1-4503-5105-8},
  pages     = {396--407},
  address   = ACMAddr,
  numpages  = {12},
}

@InProceedings{CMB:UIST18,
  author    = {Chasins, Sarah E. and Mueller, Maria and Bodik, Rastislav},
  title     = {Rousillon: Scraping Distributed Hierarchical Web Data},
  booktitle = {Proc. Symposium User Interface Software and Technology (UIST)},
  year      = {2018},
  publisher = ACM,
  location  = {Berlin, Germany},
  month     = {10},
  isbn      = {978-1-4503-5948-1},
  pages     = {963--975},
  address   = ACMAddr,
  numpages  = {13},
}

@InProceedings{RQRA:MSR16,
  author    = {Rahman, Md Tajmilur and Querel, Louis-Philippe and Rigby, Peter C. and Adams, Bram},
  title     = {Feature Toggles: Practitioner Practices and a Case Study},
  booktitle = MSR,
  year      = {2016},
  publisher = ACM,
  location  = {Austin, TX, USA},
  month     = {5},
  isbn      = {978-1-4503-4186-8},
  pages     = {201--211},
  address   = ACMAddr,
  numpages  = {11},
}

@InProceedings{GIYDZYC:ESECFSE17,
  author    = {Gopstein, Dan and Iannacone, Jake and Yan, Yu and DeLong, Lois and Zhuang, Yanyan and Yeh, Martin K.-C. and Cappos, Justin},
  title     = {Understanding Misunderstandings in Source Code},
  booktitle = ESECFSE,
  year      = {2017},
  publisher = ACM,
  location  = {Paderborn, Germany},
  month     = {9},
  isbn      = {978-1-4503-5105-8},
  pages     = {129--139},
  address   = ACMAddr,
  numpages  = {11},
}

@InProceedings{JPDE:ISSTA18,
  author    = {Just, Ren{\'e} and Parnin, Chris and Drosos, Ian and Ernst, Michael D.},
  title     = {Comparing Developer-provided to User-provided Tests for Fault Localization and Automated Program Repair},
  booktitle = ISSTA,
  year      = {2018},
  publisher = ACM,
  location  = {Amsterdam, Netherlands},
  month     = {7},
  isbn      = {978-1-4503-5699-2},
  pages     = {287--297},
  address   = ACMAddr,
  numpages  = {11},
}

@InProceedings{FLBP:CHI18,
  author    = {Ford, Denae and Lustig, Kristina and Banks, Jeremy and Parnin, Chris},
  title     = {"We Don'T Do That Here": How Collaborative Editing with Mentors Improves Engagement in Social Q\&\#38;A Communities},
  booktitle = CHI,
  year      = {2018},
  pages     = {608:1--608:12},
  address   = ACMAddr,
  month     = {4},
  publisher = ACM,
  articleno = {608},
  isbn      = {978-1-4503-5620-6},
  location  = {Montreal, QC, Canada},
  numpages  = {12},
}

@InProceedings{TD:ECOOP16,
  author    = {John Toman and Dan Grossman},
  booktitle = {Proc. European Conf. Object-Oriented Programming (ECOOP)},
  title     = {Staccato: A Bug Finder for Dynamic Configuration Updates},
  year      = {2016},
  address   = {Dagstuhl, Germany},
  month     = jul,
  publisher = {Schloss Dagstuhl--Leibniz-Zentrum fuer Informatik},
}

@InProceedings{JJKSSWM:ICSESEIP18,
  author    = {Jaspan, Ciera and Jorde, Matthew and Knight, Andrea and Sadowski, Caitlin and Smith, Edward K. and Winter, Collin and Murphy-Hill, Emerson},
  title     = {Advantages and Disadvantages of a Monolithic Repository: A Case Study at Google},
  booktitle = {Proceedings Int'l Conf. Software Engineering: Software Engineering in Practice (ICSE-SEIP)},
  year      = {2018},
  publisher = ACM,
  location  = {Gothenburg, Sweden},
  month     = {5},
  isbn      = {978-1-4503-5659-6},
  pages     = {225--234},
  address   = ACMAddr,
  numpages  = {10},
}

@InProceedings{GFM:EASE16,
  author    = {Garousi, Vahid and Felderer, Michael and M\"{a}ntyl\"{a}, Mika V.},
  title     = {The Need for Multivocal Literature Reviews in Software Engineering: Complementing Systematic Literature Reviews with Grey Literature},
  booktitle = {Proc. Int'l Conf. Evaluation and Assessment in Software Engineering (EASE)},
  year      = {2016},
  publisher = ACM,
  location  = {Limerick, Ireland},
  month     = {6},
  isbn      = {978-1-4503-3691-8},
  pages     = {26:1--26:6},
  address   = ACMAddr,
  articleno = {26},
  numpages  = {6},
}

@Misc{VJKSSA-PIRC19,
  author       = {Velez, Miguel and Jamshidi, Pooyan and K\"{a}stner, Christian and Siegmund, Norbert and Sattler, Florian and Apel, Sven},
  title        = {White-Box Performance Discovery},
  year         = {2019},
  howpublished = {Poster. Google PhD Intern Research Conference},
  location     = {Sunnyvale, CA, USA},
  month        = jul,
}

@InProceedings{JKA:ISSTA17,
  author    = {Just, Ren{\'e} and Kurtz, Bob and Ammann, Paul},
  title     = {Inferring Mutant Utility from Program Context},
  booktitle = ISSTA,
  year      = {2017},
  publisher = ACM,
  location  = {Santa Barbara, CA, USA},
  month     = {7},
  isbn      = {978-1-4503-5076-1},
  pages     = {284--294},
  address   = ACMAddr,
  numpages  = {11},
}

@Article{X:CORR19,
  author  = {Tianyin Xu},
  title   = {Configuration Testing: Testing Configuration Values Together with Code Logic},
  journal = {CoRR},
  year    = {2019},
  volume  = {abs/1905.12195},
}

@Article{EEM:TSE13,
  author  = {N. {Esfahani} and A. {Elkhodary} and S. {Malek}},
  journal = {IEEE Transactions on Software Engineering},
  title   = {A Learning-Based Framework for Engineering Feature-Oriented Self-Adaptive Software Systems},
  year    = {2013},
  month   = nov,
  number  = {11},
  pages   = {1467-1493},
  volume  = {39},
}

@Book{H:PMDCSQTA13,
  author    = {Harchol-Balter, Mor},
  publisher = {Cambridge University Press},
  title     = {Performance Modeling and Design of Computer Systems: Queueing Theory in Action},
  year      = {2013},
  address   = {New York, NY, USA},
  edition   = {1st},
  isbn      = {1107027500},
}

@InProceedings{VPGFC:ICPE17,
  author    = {Valov, Pavel and Petkovich, Jean-Christophe and Guo, Jianmei and Fischmeister, Sebastian and Czarnecki, Krzysztof},
  booktitle = {Proc. Int'l Conf. on Performance Engineering (ICPE)},
  title     = {Transferring Performance Prediction Models Across Different Hardware Platforms},
  year      = {2017},
  address   = ACMAddr,
  month     = apr,
  pages     = {39--50},
  publisher = ACM,
  isbn      = {978-1-4503-4404-3},
  location  = {L'Aquila, Italy},
  numpages  = {12},
}

@Article{WXLM:TSE19,
  author  = {Z. {Wan} and X. {Xia} and D. {Lo} and G. C. {Murphy}},
  title   = {How does Machine Learning Change Software Development Practices?},
  journal = TSE,
  year    = {2019},
}

@Misc{VJSSAK:ASEJ20SM,
  author = {Velez, Miguel and Jamshidi, Pooyan and Sattler, Florian and Siegmund, Norbert and Apel, Sven and Kästner, Christian},
  title  = {ConfigCrusher: Towards White-Box Performance Analysis for Configurable Systems - {S}upplementary {M}aterial - {https://bit.ly/3diKZmK}},
  year   = {2019},
}

@InProceedings{AB:ASE10,
  author    = {Abi-Antoun, Marwan and Barnes, Jeffrey M.},
  title     = {Analyzing Security Architectures},
  booktitle = ASE,
  year      = {2010},
  pages     = {3--12},
  address   = ACMAddr,
  publisher = ACM,
  isbn      = {978-1-4503-0116-9},
  location  = {Antwerp, Belgium},
  numpages  = {10},
}

@InProceedings{MHAADG:SANER19,
  author    = {B. J. {Muscedere} and R. {Hackman} and D. {Anbarnam} and J. M. {Atlee} and I. J. {Davis} and M. W. {Godfrey}},
  booktitle = {Int'l Conf. Software Analysis, Evolution and Reengineering (SANER)},
  title     = {Detecting Feature-Interaction Symptoms in Automotive Software using Lightweight Analysis},
  year      = {2019},
  month     = feb,
  pages     = {175-185},
  doi       = {10.1109/SANER.2019.8668042},
}

@Article{JAVKE:ISR16,
  author    = {Jenkins, Jeffrey L and Anderson, Bonnie Brinton and Vance, Anthony and Kirwan, C Brock and Eargle, David},
  title     = {More harm than good? How messages that interrupt can make us vulnerable},
  journal   = {Information Systems Research},
  year      = {2016},
  volume    = {27},
  number    = {4},
  pages     = {880--896},
  publisher = {INFORMS},
}

@InProceedings{NSCMBL:ESECFSE19,
  author    = {Nguyen, Phu H. and Song, Hui and Chauvel, Franck and Muller, Roy and Boyar, Seref and Levin, Erik},
  title     = {Using Microservices for Non-intrusive Customization of Multi-tenant SaaS},
  booktitle = ESECFSE,
  year      = {2019},
  pages     = {905--915},
  address   = ACMAddr,
  month     = aug,
  publisher = ACM,
  location  = {Tallinn, Estonia},
  numpages  = {11},
}

@Article{BKR:JSS09,
  author     = {Becker, Steffen and Koziolek, Heiko and Reussner, Ralf},
  journal    = {J. Syst. Softw.},
  title      = {The {P}alladio Component Model for Model-driven Performance Prediction},
  year       = {2009},
  issn       = {0164-1212},
  month      = jan,
  number     = {1},
  pages      = {3--22},
  volume     = {82},
  address    = ACMAddr,
  issue_date = {January, 2009},
  numpages   = {20},
  publisher  = {Elsevier Science Inc.},
}

@InProceedings{SCBSCB:QEST06,
  author    = {G. {Serazzri} and G. {Casale} and M. {Bertoli} and G. {Serazzri} and G. {Casale} and M. {Bertoli}},
  booktitle = {Proc. Int'l Conf. the Quantitative Evaluation of Systems - (QEST'06)},
  title     = {Java Modelling Tools: {A}n Open Source Suite for Queueing Network Modelling andWorkload Analysis},
  year      = {2006},
  month     = sep,
  pages     = {119-120},
}

@InProceedings{ORGC:SPLC14,
  author    = {Olaechea, Rafael and Rayside, Derek and Guo, Jianmei and Czarnecki, Krzysztof},
  title     = {Comparison of Exact and Approximate Multi-objective Optimization for Software Product Lines},
  booktitle = SPLC,
  year      = {2014},
  pages     = {92--101},
  address   = ACMAddr,
  month     = sep,
  publisher = ACM,
  location  = {Florence, Italy},
  numpages  = {10},
}

@InProceedings{WCWHC:ICSE18,
  author    = {M. {Wen} and J. {Chen} and R. {Wu} and D. {Hao} and S. {Cheung}},
  booktitle = ICSE,
  title     = {Context-Aware Patch Generation for Better Automated Program Repair},
  year      = {2018},
  month     = may,
  pages     = {1-11},
}

@Article{O:CACM18,
  author     = {Ousterhout, John},
  title      = {Always Measure One Level Deeper},
  journal    = CACM,
  year       = {2018},
  volume     = {61},
  number     = {7},
  pages      = {74--83},
  month      = jun,
  issn       = {0001-0782},
  address    = ACMAddr,
  issue_date = {July 2018},
  numpages   = {10},
  publisher  = ACM,
}

@InProceedings{HHBDD:CHI19,
  author    = {Head, Andrew and Hohman, Fred and Barik, Titus and Drucker, Steven M. and DeLine, Robert},
  title     = {Managing Messes in Computational Notebooks},
  booktitle = CHI,
  year      = {2019},
  pages     = {270:1--270:12},
  address   = ACMAddr,
  publisher = ACM,
  articleno = {270},
  isbn      = {978-1-4503-5970-2},
  location  = {Glasgow, Scotland Uk},
  numpages  = {12},
}

@Article{S:TA18,
  author  = {Somers, James},
  title   = {The scientific paper is obsolete},
  journal = {The Atlantic},
  year    = {2018},
}

@InProceedings{TAOM:KDD10,
  author    = {Tang, Diane and Agarwal, Ashish and O'Brien, Deirdre and Meyer, Mike},
  title     = {Overlapping Experiment Infrastructure: More, Better, Faster Experimentation},
  booktitle = {Proc. Int'l Conf. Knowledge Discovery and Data Mining (KDD)},
  year      = {2010},
  pages     = {17--26},
  address   = ACMAddr,
  month     = jul,
  publisher = ACM,
  location  = {Washington, DC, USA},
  numpages  = {10},
}

@Article{AGKLMRSSTVVBGHCJ:IEEES19,
  author  = {J. {Aldrich} and D. {Garlan} and C. {Kaestner} and C. {Le Goues} and A. {Mohseni-Kabir} and I. {Ruchkin} and S. {Samuel} and B. {Schmerl} and C. S. {Timperley} and M. {Veloso} and I. {Voysey} and J. {Biswas} and A. {Guha} and J. {Holtz} and J. {Camara} and P. {Jamshidi}},
  journal = {IEEE Software},
  title   = {Model-Based Adaptation for Robotics Software},
  year    = {2019},
  month   = mar,
  number  = {2},
  pages   = {83-90},
  volume  = {36},
}

@InProceedings{WLKS:SEAMS17,
  author    = {Weisenburger, Pascal and Luthra, Manisha and Koldehofe, Boris and Salvaneschi, Guido},
  title     = {Quality-aware Runtime Adaptation in Complex Event Processing},
  booktitle = {Proc. Int'l Symp. Software Engineering for Adaptive and Self-Managing Systems (SEAMS)},
  year      = {2017},
  pages     = {140--151},
  address   = IEEEAddr,
  month     = may,
  publisher = IEEE,
  location  = {Buenos Aires, Argentina},
  numpages  = {12},
}

@Misc{VB:ARVIX19,
  author        = {Andreas Vogelsang and Markus Borg},
  title         = {Requirements Engineering for Machine Learning: Perspectives from Data Scientists},
  year          = {2019},
  archiveprefix = {arXiv},
  eprint        = {1908.04674},
}

@InProceedings{HZ:ICSME19,
  author    = {H. {Ha} and H. {Zhang}},
  booktitle = ICSME,
  title     = {Performance-Influence Model for Highly Configurable Software with Fourier Learning and Lasso Regression},
  year      = {2019},
  month     = sep,
  pages     = {470-480},
}

@Article{SZZLJW:OOPSLA19,
  author    = {Shen, Bo and Zhang, Wei and Zhao, Haiyan and Liang, Guangtai and Jin, Zhi and Wang, Qianxiang},
  title     = {IntelliMerge: A Refactoring-Aware Software Merging Technique},
  journal   = OOPSLA,
  year      = {2019},
  month     = oct,
  address   = ACMAddr,
  numpages  = {28},
  publisher = ACM,
}

@InProceedings{HLWMZLHLX:ASE19,
  author    = {D. {He} and H. {Li} and L. {Wang} and H. {Meng} and H. {Zheng} and J. {Liu} and S. {Hu} and L. {Li} and J. {Xue}},
  booktitle = ASE,
  title     = {Performance-Boosting Sparsification of the IFDS Algorithm with Applications to Taint Analysis},
  year      = {2019},
  month     = nov,
  pages     = {267-279},
}

@InProceedings{RSG:ACL1,
  author    = {Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  title     = {Semantically Equivalent Adversarial Rules for Debugging {NLP} models},
  booktitle = {Proc. Meet. Association for Computational Linguistics},
  year      = {2018},
  pages     = {856--865},
  address   = {Melbourne, Australia},
  month     = jul,
  publisher = {Association for Computational Linguistics},
}

@InProceedings{HWHB:ICSE2020,
  author    = {Katherine Hough, Gebrehiwet Welearegai, Christian Hammer and Jonathan Bell},
  title     = {Revealing Injection Vulnerabilities by Leveraging Existing Tests},
  booktitle = ICSE,
  year      = {2020},
  address   = ACMAddr,
  month     = may,
  publisher = ACM,
  location  = {Seoul, South Korea},
}

@InProceedings{JBM:ICSE2020,
  author    = {Brittany Johnson, Yuriy Brun, Alexandra Meliou},
  title     = {Causal Testing: Understanding Defects’ Root Causes},
  booktitle = ICSE,
  year      = {2020},
  address   = ACMAddr,
  month     = may,
  publisher = ACM,
  location  = {Seoul, South Korea},
}

@InProceedings{HPGV:ICSE19,
  author    = {Hellendoorn, Vincent J. and Proksch, Sebastian and Gall, Harald C. and Bacchelli, Alberto},
  title     = {When Code Completion Fails: A Case Study on Real-World Completions},
  booktitle = ICSE,
  year      = {2019},
  pages     = {960–970},
  month     = may,
  publisher = IEEE,
  location  = {Montreal, Quebec, Canada},
  numpages  = {11},
}

@Article{PLSSV:OOPSLA19,
  author     = {Padhye, Rohan and Lemieux, Caroline and Sen, Koushik and Simon, Laurent and Vijayakumar, Hayawardh},
  title      = {FuzzFactory: Domain-Specific Fuzzing with Waypoints},
  journal    = OOPSLA,
  year       = {2019},
  volume     = {3},
  month      = oct,
  address    = ACMAddr,
  issue_date = {October 2019},
  numpages   = {29},
  publisher  = ACM,
}

@InProceedings{ZSSL:NEURIPS18,
  author    = {Zhang, Xin and Solar-Lezama, Armando and Singh, Rishabh},
  booktitle = {Proc. Int'l Conf. Neural Information Processing Systems (NeurIPS)},
  title     = {Interpreting Neural Network Judgments via Minimal, Stable, and Symbolic Corrections},
  year      = {2018},
  address   = {Red Hook, NY, USA},
  month     = dec,
  pages     = {4879–4890},
  publisher = {Curran Associates Inc.},
  location  = {Montr\'{e}al, Canada},
  numpages  = {12},
}

@InProceedings{STSMP:ICSE2020,
  author    = {Staicu, Cristian-Alexandru and Torp, Martin Toldam, and Schäfer, Max and Møller, Anders and Pradel, Michael},
  booktitle = ICSE,
  title     = {Extracting Taint Specifications for JavaScript Libraries},
  year      = {2020},
  address   = ACMAddr,
  month     = may,
  publisher = ACM,
  location  = {Seoul, South Korea},
}

@InProceedings{DMMA:ESECFSE19,
  author    = {Durieux, Thomas and Madeiral, Fernanda and Martinez, Matias and Abreu, Rui},
  booktitle = ESECFSE,
  title     = {Empirical Review of Java Program Repair Tools: A Large-Scale Experiment on 2,141 Bugs and 23,551 Repair Attempts},
  year      = {2019},
  address   = ACMAddr,
  month     = aug,
  pages     = {302–313},
  publisher = ACM,
  location  = {Tallinn, Estonia},
  numpages  = {12},
}

@InProceedings{TD:ECOOP18,
  author    = {Toman, John and Grossman, Dan},
  booktitle = {European Conf. Object-Oriented Programming (ECOOP)},
  title     = {Legato: An At-Most-Once Analysis with Applications to Dynamic Configuration Updates},
  year      = {2016},
  address   = {Amsterdam, Netherlands},
  month     = {7},
}

@PhdThesis{H:PHD19,
  author = {Xue Han},
  school = {University of Kentucky},
  title  = {CONFPROFITT: A CONFIGURATIONAWAREPERFORMANCE PROFILING,TESTING, AND TUNING FRAMEWORK},
  year   = {2019},
}

@InProceedings{KGSGA:ICSE19,
  author    = {Kaltenecker, Christian and Grebhahn, Alexander and Siegmund, Norbert and Guo, Jianmei and Apel, Sven},
  booktitle = ICSE,
  title     = {Distance-Based Sampling of Software Configuration Spaces},
  year      = {2019},
  month     = may,
  publisher = IEEE,
  location  = {Montreal, Quebec, Canada},
}

@Article{KGSA:IEEESOFT20,
  author  = {C. {Kaltenecker} and A. {Grebhahn} and N. {Siegmund} and S. {Apel}},
  journal = {IEEE Software},
  title   = {The Interplay of Sampling and Machine Learning for Software Performance Prediction},
  year    = {2020},
}

@Online{MV:SM,
  title = {See supplementary material in EasyChair},
}

@InProceedings{CPHSB:CHI20,
  author    = {Chattopadhyay, Souti and Prasad, Ishita and Henley, Austin Z. and Sarma, Anita and Barik, Titus},
  booktitle = CHI,
  title     = {What's Wrong with Computational Notebooks? Pain Points, Needs, and Design Opportunities},
  year      = {2020},
  month     = apr,
}

@InProceedings{HJJGS:ICSE20,
  author    = {Hu, Jingmei and Joung, Jiwon and Jacobs, Maia and Gajos, Krzysztof and Seltzer, Margo},
  booktitle = ICSE,
  title     = {Revealing Injection Vulnerabilities by Leveraging Existing Tests},
  year      = {2020},
  address   = ACMAddr,
  month     = may,
  publisher = ACM,
  location  = {Seoul, South Korea},
}

@Article{SKPBA:ESE20,
  author  = {Sayagh, Mohammed and Kerzazi, Noureddine and Petrillo, Fabio and Bennani, Khalil and Adams, Bram},
  journal = {Empirical Software Engineering},
  title   = {What should your run-time configuration framework do to help developers?},
  year    = {2020},
  month   = jan,
  number  = {2},
  volume  = {25},
}

@Book{VN:PMAS15,
  author    = {Viswanadham, Nukala and Narahari, Yadati},
  publisher = {PHI Learning Pvt. Ltd.},
  title     = {Performance modeling of automated systems},
  year      = {2015},
}

@Article{K:PMEDCSUQPN06,
  author    = {Kounev, Samuel},
  journal   = {IEEE Transactions on Software Engineering},
  title     = {Performance modeling and evaluation of distributed component-based systems using queueing {P}etri {N}ets},
  year      = {2006},
  number    = {7},
  pages     = {486--502},
  volume    = {32},
  publisher = {IEEE},
}

@Online{L:MJP11,
  author       = {Fabian Lange},
  lastaccessed = {January 24, 2020},
  month        = jan,
  title        = {Measure {J}ava Performance – Sampling or Instrumentation?},
  year         = {2011},
}

@InProceedings{LVADL:ESECFSE13,
  author    = {J{\"o}rg Liebig and Alexander von Rhein and Christian K{\"a}stner and Sven Apel and Jens D{\"o}rre and Christian Lengauer},
  booktitle = ESECFSE,
  title     = {Scalable Analysis of Variable Software},
  year      = {2013},
  address   = ACMAddr,
  month     = {8},
  pages     = {81--91},
  publisher = ACMPress,
}

@InProceedings{GFX:ICSE2012,
  author    = {Grechanik, Mark and Fu, Chen and Xie, Qing},
  booktitle = ICSE,
  title     = {Automatically Finding Performance Problems with Feedback-Directed Learning Software Testing},
  year      = {2012},
  month     = jun,
  pages     = {156–166},
  publisher = IEEE,
  isbn      = {9781467310673},
  location  = {Zurich, Switzerland},
  numpages  = {11},
}

@InProceedings{JAH:OOPSLA11,
  author    = {Jovic, Milan and Adamoli, Andrea and Hauswirth, Matthias},
  booktitle = OOPSLA,
  title     = {Catch Me If You Can: Performance Bug Detection in the Wild},
  year      = {2011},
  address   = ACMAddr,
  month     = oct,
  pages     = {155–170},
  publisher = ACM,
  location  = {Portland, Oregon, USA},
  numpages  = {16},
}

@InProceedings{LWHL:EUROSYS20,
  author    = {Li, Chi and Wang, Shu and Hoffmann, Henry and Lu, Shan},
  booktitle = {Proc. European Conf. Computer Systems (EuroSys)},
  title     = {Statically Inferring Performance Properties of Software Configurations},
  year      = {2020},
  address   = ACMAddr,
  month     = apr,
  publisher = ACM,
  articleno = {Article 10},
  isbn      = {9781450368827},
  location  = {Heraklion, Greece},
  numpages  = {16},
}

@InProceedings{SBLB:ESECFSE15,
  author    = {Smith, Edward K. and Barr, Earl T. and Le Goues, Claire and Brun, Yuriy},
  booktitle = ESECFSE,
  title     = {Is the Cure Worse than the Disease? Overfitting in Automated Program Repair},
  year      = {2015},
  address   = ACMAddr,
  month     = aug,
  pages     = {532–543},
  publisher = ACM,
  isbn      = {9781450336758},
  location  = {Bergamo, Italy},
  numpages  = {12},
}

@InProceedings{VANTPLTR:ICSE20,
  author    = {van der Linden, Dirk and Anthonysamy, Pauline and Nuseibeh, Bashar and Tun, Thein and Petre, Marian and Levine, Mark and Towse, John and Rashid, Awais},
  booktitle = ICSE,
  title     = {Schrödinger’s Security: Opening the Box on App Developers’Security Rationale},
  year      = {2020},
  address   = ACMAddr,
  month     = may,
  publisher = ACM,
  location  = {Seoul, South Korea},
}

@Book{S:TMDS14,
  author    = {Shostack, Adam},
  publisher = {Wiley Publishing},
  title     = {Threat Modeling: Designing for Security},
  year      = {2014},
  edition   = {1st},
  isbn      = {1118809998},
}

@Article{VJSSAK:ASEJ20,
  author  = {Velez, Miguel and Jamshidi, Pooyan and Sattler, Florian and Siegmund, Norbert and Apel, Sven and Kästner, Christian},
  journal = {Autom Softw Eng},
  title   = {ConfigCrusher: Towards White-Box Performance Analysis for Configurable Systems},
  year    = {2020},
}

@InProceedings{HZ:ICSE19,
  author    = {Ha, Huong and Zhang, Hongyu},
  booktitle = ICSE,
  title     = {Deep{P}erf: Performance Prediction for Configurable Software with Deep Sparse Neural Network},
  year      = {2019},
  month     = may,
  pages     = {1095–1106},
  publisher = IEEE,
  location  = {Montreal, Quebec, Canada},
  numpages  = {12},
}

@Article{GYSASVCWY:ESE17,
  author  = {Jianmei Guo and Dingyu Yang and N. Siegmund and S. Apel and Atrisha Sarkar and Pavel Valov and K. Czarnecki and A. Wasowski and H. Yu},
  journal = {Empirical Software Engineering},
  title   = {Data-efficient performance learning for configurable systems},
  year    = {2017},
  pages   = {1826-1867},
  volume  = {23},
}

@Misc{GSA:PPSCNSB19,
  author        = {Alexander Grebhahn and Norbert Siegmund and Sven Apel},
  title         = {Predicting Performance of Software Configurations: There is no Silver Bullet},
  year          = {2019},
  archiveprefix = {arXiv},
  eprint        = {1911.12643},
  primaryclass  = {cs.SE},
}

@Book{M:IML20,
  title      = {Interpretable Machine Learning},
  author     = {Christoph Molnar},
  note       = {\url{https://christophm.github.io/interpretable-ml-book/}},
  year       = {2019},
  subtitle   = {A Guide for Making Black Box Models Explainable}
}

@Article{R:NMI19,
  author  = {Rudin, Cynthia},
  journal = {Nature Machine Intelligence},
  title   = {Stop explaining black box machine learning models for high stakes decisions and use interpretable models instead},
  year    = {2019},
  number  = {5},
  pages   = {206-215},
}

@Online{SAT4J,
  lastaccessed = {January 24, 2020},
  title        = {SAT4J},
  url          = {www.sat4j.org},
}

@Online{JPROFILER10,
  lastaccessed = {December 10, 2019},
  title        = {JProfiler 10},
  url          = {https://www.ej-technologies.com/products/jprofiler/overview.html},
  year         = {2019},
}

@TechReport{AJ:ARCHIVE18,
  author      = {Alvarez-Melis, David and Tommi S. Jaakkola},
  institution = {arXiv},
  title       = {On the robustness of interpretability methods},
  year        = {2018},
  number      = {arXiv:1806.08049},
}

@InCollection{LL:ANIPS17,
  author    = {Lundberg, Scott M and Lee, Su-In},
  booktitle = {Advances in Neural Information Processing Systems 30},
  publisher = {Curran Associates, Inc.},
  title     = {A Unified Approach to Interpreting Model Predictions},
  year      = {2017},
  pages     = {4765--4774},
}

@Article{SK:KIS14,
  author    = {{\v{S}}trumbelj, Erik and Kononenko, Igor},
  journal   = {Knowledge and information systems},
  title     = {Explaining prediction models and individual predictions with feature contributions},
  year      = {2014},
  number    = {3},
  pages     = {647--665},
  volume    = {41},
  publisher = {Springer},
}

@InProceedings{LPSS:ISSTA18,
  author    = {Lemieux, Caroline and Padhye, Rohan and Sen, Koushik and Song, Dawn},
  booktitle = ISSTA,
  title     = {Perffuzz: Automatically generating pathological inputs},
  year      = {2018},
  address   = ACMAddr,
  pages     = {254--265},
  publisher = ACM,
  location  = {Amsterdam, Netherlands},
}

@Article{DK:ARCHIVE17,
  author  = {Doshi-Velez, Finale and Kim, Been},
  journal = {arXiv preprint arXiv:1702.08608},
  title   = {Towards a rigorous science of interpretable machine learning},
  year    = {2017},
}

@Article{PZKIFKWZKCW:ARCHIVE19,
  author  = {Fotis Psallidas and Yiwen Zhu and Bojan Karlas and Matteo Interlandi and Avrilia Floratou and Konstantinos Karanasos and Wentao Wu and Ce Zhang and Subru Krishnan and Carlo Curino and Markus Weimer},
  journal = {arXiv},
  title   = {Data Science through the looking glass and what we found there},
  year    = {2019},
  number  = {1912.09536},
}

@InProceedings{CB:ATC16,
  author    = {Charlie Curtsinger and Emery D. Berger},
  booktitle = {USENIX Annual Technical Conference (ATC)},
  title     = {{COZ}: Finding Code that Counts with Causal Profiling},
  year      = {2016},
  address   = {Denver, CO, USA},
  month     = jun,
  publisher = {{USENIX} Association},
}

@InProceedings{HWDDW:CHI19,
  author    = {Holstein, Kenneth and Wortman Vaughan, Jennifer and Daum\'{e}, Hal and Dudik, Miro and Wallach, Hanna},
  booktitle = {Proc. Conference Human Factors in Computing Systems (CHI)},
  title     = {Improving Fairness in Machine Learning Systems: What Do Industry Practitioners Need?},
  year      = {2019},
  address   = ACMAddr,
  month     = may,
  pages     = {1–16},
  publisher = ACM,
  location  = {Glasgow, Scotland, UK},
  numpages  = {16},
}

@InProceedings{LR:ICSE16,
  author    = {Long, Fan and Rinard, Martin},
  booktitle = ICSE,
  title     = {An Analysis of the Search Spaces for Generate and Validate Patch Generation Systems},
  year      = {2016},
  address   = ACMAddr,
  month     = may,
  pages     = {702–713},
  publisher = ACM,
  location  = {Austin, TX, USA},
  numpages  = {12},
}

@InProceedings{KES:VLHCC20,
  author    = {A. P. {Koenzen} and N. A. {Ernst} and M. D. {Storey}},
  booktitle = {Symposium Visual Languages and Human-Centric Computing (VL/HCC)},
  title     = {Code Duplication and Reuse in Jupyter Notebooks},
  year      = {2020},
  month     = aug,
  pages     = {1-9},
}

@InProceedings{MBW:ICSE16,
  author    = {Melo, Jean and Brabrand, Claus and W\k{a}sowski, Andrzej},
  booktitle = ICSE,
  title     = {How Does the Degree of Variability Affect Bug Finding?},
  year      = {2016},
  address   = ACMAddr,
  month     = may,
  pages     = {679–690},
  publisher = ACM,
  isbn      = {9781450339001},
  location  = {Austin, TX, USA},
  numpages  = {12},
}

@InProceedings{CCLWXL:FSE20,
  author    = {Zhenpeng Chen and Yanbin Cao and Yuanqiang Liu and Haoyu Wang and Tao Xie and Xuanzhe Liu},
  booktitle = FSE,
  title     = {Understanding Challenges in Deploying Deep Learning Based Software: An Empirical Study},
  year      = {2020},
  month     = nov,
  location  = {Sacramento, CA, USA},
}

@Article{PLSPL:ISSTA19,
  author    = {Padhye, Rohan and Lemieux, Caroline and Sen, Koushik and Papadakis, Mike and Le Traon, Yves},
  title     = {Semantic Fuzzing with {Z}est},
  year      = {2019},
  month     = jun,
  pages     = {329–340},
  address   = ACMAddr,
  booktitle = ISSTA,
  location  = {Beijing, China},
  numpages  = {12},
  publisher = ACM,
}

@InProceedings{MMC:VSUA02,
  author    = {J. I. {Maletic} and A. {Marcus} and M. L. {Collard}},
  booktitle = {Proc. Int'l Workshop Visualizing Software for Understanding and Analysis},
  title     = {A task oriented view of software visualization},
  year      = {2002},
  month     = jun,
  pages     = {32-40},
}

@InProceedings{SSA:ICSE15,
  author    = {Siegmund, Janet and Siegmund, Norbert and Apel, Sven},
  booktitle = ICSE,
  title     = {Views on Internal and External Validity in Empirical Software Engineering},
  year      = {2015},
  month     = may,
  pages     = {9–19},
  publisher = IEEE,
  isbn      = {9781479919345},
  location  = {Florence, Italy},
  numpages  = {11},
}

@InProceedings{PVM:CCS20,
  author    = {Ivan Pashchenko and Duc-Ly Vu and Fabio Massacci},
  booktitle = {Conf. Cmputer and Communications Security (CCS)},
  title     = {A Qualitative Study of Dependency Management and Its Security Implications (To be appear in ACM CCS 2020)},
  year      = {2020},
  address   = ACMAddr,
  month     = nov,
  publisher = ACM,
}

@Article{LBBBRK:TSE13,
  author     = {Lawrance, Joseph and Bogart, Christopher and Burnett, Margaret and Bellamy, Rachel and Rector, Kyle and Fleming, Scott D.},
  journal    = TSE,
  title      = {How Programmers Debug, Revisited: An Information Foraging Theory Perspective},
  year       = {2013},
  month      = feb,
  number     = {2},
  pages      = {197–215},
  volume     = {39},
  issue_date = {February 2013},
  numpages   = {19},
  publisher  = IEEE,
}

@InProceedings{HJLXYYWL:ASE20,
  author    = {Haochen He and Zhouyang Jia and Shanshan Li and Erci Xu and Tingting Yu and Yue Yu and Ji Wang and Xiangke Liao},
  booktitle = ASE,
  title     = {CP-Detector: Using Configuration-related PerformanceProperties to Expose Performance Bugs},
  year      = {2020},
  month     = nov,
}

@Article{PC:CACM17,
  author    = {Pinto, Gustavo and Castor, Fernando},
  journal   = CACM,
  title     = {Energy Efficiency: A New Concern for Application Software Developers},
  year      = {2017},
  month     = nov,
  number    = {12},
  pages     = {68–75},
  volume    = {60},
  address   = ACMAddr,
  numpages  = {8},
  publisher = ACM,
}

@Article{GC:U15,
  author    = {Gelenbe, Erol and Caseau, Yves},
  journal   = {Ubiquity},
  title     = {The Impact of Information Technology on Energy Consumption and Carbon Emissions},
  year      = {2015},
  month     = jun,
  number    = {June},
  volume    = {2015},
  address   = ACMAddr,
  articleno = {1},
  numpages  = {15},
  publisher = ACM,
}

@InProceedings{VJSAK:20,
  author    = {Velez, Miguel and Jamshidi, Pooyan and Siegmund, Norbert and Apel, Sven and Kästner, Christian},
  booktitle = {Under review},
  title     = {White-box Analysis over Machine Learning: Modeling Performance of Configurable Systems},
  year      = {2020},
}

@Misc{ZMW:ARXIV20,
  author        = {Amy X. Zhang and Michael Muller and Dakuo Wang},
  title         = {How do Data Science Workers Collaborate? Roles, Workflows, and Tools},
  year          = {2020},
  archiveprefix = {arXiv},
  eprint        = {2001.06684},
}

@Book{Z:WPF09,
  author    = {Zeller, Andreas},
  publisher = {Elsevier},
  title     = {Why programs fail: a guide to systematic debugging},
  year      = {2009},
}

@InProceedings{KM:CHI04,
  author    = {Ko, Andrew J. and Myers, Brad A.},
  booktitle = {Proc. Conf Human Factors in Computing Systems (CHI)},
  title     = {Designing the Whyline: A Debugging Interface for Asking Questions about Program Behavior},
  year      = {2004},
  address   = ACMAddr,
  month     = apr,
  publisher = ACM,
  location  = {Vienna, Austria},
  numpages  = {8},
}

@InProceedings{LM:VLHCC11,
  author    = {T. D. {LaToza} and B. A. {Myers}},
  booktitle = {Symposium Visual Languages and Human-Centric Computing (VL/HCC)},
  title     = {Visualizing call graphs},
  year      = {2011},
  month     = nov,
  pages     = {117-124},
}

@Article{MWKS:ARXIV18,
  author  = {Meinicke, Jens and Wong, Chu-Pan and K{\"a}stner, Christian and Saake, Gunter},
  journal = {arXiv preprint arXiv:1807.03837},
  title   = {Understanding differences among executions with variational traces},
  year    = {2018},
}

@Article{WMLK:OOPSLA18,
  author    = {Wong, Chu-Pan and Meinicke, Jens and Lazarek, Lukas and K\"{a}stner, Christian},
  journal   = OOPSLA,
  title     = {Faster Variational Execution with Transparent Bytecode Transformation},
  year      = {2018},
  month     = oct,
  volume    = {2},
  address   = ACMAddr,
  articleno = {117},
  numpages  = {30},
  publisher = ACM,
}

@InProceedings{ACF:OSDI12,
  author    = {Attariyan, Mona and Chow, Michael and Flinn, Jason},
  booktitle = {Proc. Conf. Operating Systems Design and Implementation (OSDI)},
  title     = {X-Ray: Automating Root-Cause Diagnosis of Performance Anomalies in Production Software},
  year      = {2012},
  month     = oct,
  pages     = {307–320},
  publisher = {USENIX Association},
  isbn      = {9781931971966},
  location  = {Hollywood, CA, USA},
  numpages  = {14},
}

@InProceedings{SL:OOPSLA14,
  author    = {Song, Linhai and Lu, Shan},
  booktitle = OOPSLA,
  title     = {Statistical Debugging for Real-World Performance Problems},
  year      = {2014},
  address   = ACMAddr,
  month     = oct,
  pages     = {561–578},
  publisher = ACM,
  location  = {Portland, OR, USA},
  numpages  = {18},
}

@InProceedings{AMLZ:ECML07,
  author    = {Andrzejewski, David and Mulhern, Anne and Liblit, Ben and Zhu, Xiaojin},
  booktitle = {Proc. European Conf. Machine Learning},
  title     = {Statistical Debugging Using Latent Topic Models},
  year      = {2007},
  address   = {Berlin, Heidelberg},
  month     = sep,
  pages     = {6–17},
  publisher = {Springer-Verlag},
  location  = {Warsaw, Poland},
  numpages  = {12},
}

@InProceedings{BBKE:UIST13,
  author    = {Burg, Brian and Bailey, Richard and Ko, Andrew J. and Ernst, Michael D.},
  booktitle = {Proc. Symposium User Interface Software and Technology (UIST)},
  title     = {Interactive Record/Replay for Web Application Debugging},
  year      = {2013},
  address   = ACMAddr,
  month     = oct,
  pages     = {473–484},
  publisher = ACM,
  location  = {St. Andrews, Scotland, United Kingdom},
  numpages  = {12},
}

@InProceedings{PTP:OOPSLA07,
  author    = {Pothier, Guillaume and Tanter, \'{E}ric and Piquer, Jos\'{e}},
  booktitle = OOPSLA,
  title     = {Scalable Omniscient Debugging},
  year      = {2007},
  address   = ACMAddr,
  month     = oct,
  pages     = {535–552},
  publisher = ACM,
  location  = {Montreal, Quebec, Canada},
  numpages  = {18},
}

@InProceedings{PKRB:MSR12,
  author    = {J. {Park} and M. {Kim} and B. {Ray} and D. {Bae}},
  booktitle = MSR,
  title     = {An empirical study of supplementary bug fixes},
  year      = {2012},
  month     = jun,
  pages     = {40-49},
  location  = {Zurich, Switzerland},
}

@Misc{SSP:ARXIV19,
  author        = {Seemanta Saha and Ripon K. Saha and Mukul R. Prasad},
  title         = {Harnessing Evolution for Multi-Hunk Program Repair},
  year          = {2019},
  archiveprefix = {arXiv},
  eprint        = {1906.08903},
  primaryclass  = {cs.SE},
}

@InProceedings{HRMGD:FSE20,
  author    = {Hennie Huijgens and Ayushi Rastogi and Ernst Mulders and Georgios Gousios and Arievan Deursen},
  booktitle = ESECFSE,
  title     = {Questions for Data Scientists in Software Engineering: A Replication},
  year      = {2020},
  address   = ACMAddr,
  month     = nov,
  publisher = ACM,
}

@Article{RR:HDSR19,
  author  = {Rudin, Cynthia and Radin, Joanna},
  journal = {Harvard Data Science Review},
  title   = {Why Are We Using Black Box Models in AI When We Don’t Need To? A Lesson From An Explainable AI Competition},
  year    = {2019},
  month   = {11},
  number  = {2},
  volume  = {1},
  day     = {22},
}

@Book{SRACCGST:GSATP08,
  author    = {Saltelli, Andrea and Ratto, Marco and Andres, Terry and Campolongo, Francesca and Cariboni, Jessica and Gatelli, Debora and Saisana, Michaela and Tarantola, Stefano},
  publisher = {John Wiley \& Sons},
  title     = {Global sensitivity analysis: the primer},
  year      = {2008},
}

@Book{RS:LMS08,
  author    = {Rencher, Alvin C and Schaalje, G Bruce},
  publisher = {John Wiley \& Sons},
  title     = {Linear models in statistics},
  year      = {2008},
}

@Book{AAR:MMB04,
  author    = {Allman, Elizabeth S and Allman, Elizabeth S and Rhodes, John A},
  publisher = {Cambridge University Press},
  title     = {Mathematical models in biology: an introduction},
  year      = {2004},
}

@Book{FDM:PMAAS14,
  author    = {Frees, Edward W and Derrig, Richard A and Meyers, Glenn},
  publisher = {Cambridge University Press},
  title     = {Predictive modeling applications in actuarial science},
  year      = {2014},
  volume    = {1},
}

@InProceedings{MZG:MSR15,
  author    = {Malik, Haroon and Zhao, Peng and Godfrey, Michael},
  booktitle = MSR,
  title     = {Going Green: An Exploratory Analysis of Energy-Related Questions},
  year      = {2015},
  month     = may,
  pages     = {418–421},
  publisher = {IEEE Press},
  isbn      = {9780769555942},
  location  = {Florence, Italy},
  numpages  = {4},
}

@InProceedings{HKHSAH:ICSE16,
  author    = {Samir Hasan and Zachary King and Munawar Hafiz and Mohammed Sayagh and Bram Adams and Abram Hindle},
  booktitle = ICSE,
  title     = {Energy Profiles of Java Collections Classes},
  year      = {2016},
  address   = ACMAddr,
  month     = may,
  publisher = ACM,
  location  = {Austin, TX, USA},
}

@InProceedings{LLGH:ICSE16,
  author    = {Ding Li and Yingjun Lyu and Jiaping Gui and William G.J. Halfond},
  title     = {Automated Energy Optimization of HTTP Requests for Mobile Applications},
  year      = {2016},
  address   = ACMAddr,
  month     = may,
  publisher = ACM,
  location  = {Austin, TX, USA},
}

@InProceedings{CH:MSR16,
  author    = {Chowdhury, Shaiful Alam and Hindle, Abram},
  booktitle = MSR,
  title     = {GreenOracle: Estimating Software Energy Consumption with Energy Measurement Corpora},
  year      = {2016},
  address   = ACMAddr,
  month     = may,
  pages     = {49–60},
  publisher = ACM,
  location  = {Austin, TX, USA},
  numpages  = {12},
}

@InProceedings{PCSCF:GREENS16,
  author    = {Pereira, Rui and Couto, Marco and Saraiva, Jo\~{a}o and Cunha, J\'{a}come and Fernandes, Jo\~{a}o Paulo},
  booktitle = {Proc. Int'l Workshop Green and Sustainable Software (GREENS)},
  title     = {The Influence of the Java Collection Framework on Overall Energy Consumption},
  year      = {2016},
  address   = ACMAddr,
  month     = may,
  pages     = {15–21},
  publisher = ACM,
  location  = {Austin, TX, USA},
  numpages  = {7},
}

@Article{ZHG:IEEESOFT14,
  author  = {C. {Zhang} and A. {Hindle} and D. M. {German}},
  journal = {IEEE Software},
  title   = {The Impact of User Choice on Energy Consumption},
  year    = {2014},
  number  = {3},
  pages   = {69-75},
  volume  = {31},
  doi     = {10.1109/MS.2014.27},
}

@InBook{KDJNGFM:GSG11,
  author    = {Kern, Eva and Dick, Markus and Johann, Timo and Naumann, Stefan},
  editor    = {Golinska, Paulina and Fertsch, Marek and Marx-G{\'o}mez, Jorge},
  pages     = {199--211},
  publisher = {Springer Berlin Heidelberg},
  title     = {Green Software and Green IT: An End Users Perspective},
  year      = {2011},
  address   = {Berlin, Heidelberg},
  booktitle = {Information Technologies in Environmental Engineering: New Trends and Challenges},
}

@InProceedings{GLWH:GREENS16,
  author    = {Gui, Jiaping and Li, Ding and Wan, Mian and Halfond, William G. J.},
  booktitle = {Proc. Int'l Workshop Green and Sustainable Software (GREENS)},
  title     = {Lightweight Measurement and Estimation of Mobile Ad Energy Consumption},
  year      = {2016},
  address   = ACMAddr,
  month     = may,
  pages     = {1–7},
  publisher = ACM,
  isbn      = {9781450341615},
  location  = {Austin, TX, USA},
  numpages  = {7},
}

@InProceedings{WRGPA:GCC13,
  author    = {Wilke, Claas and Richly, Sebastian and G\"{o}tz, Sebastian and Piechnick, Christian and Amann, Uwe},
  booktitle = {Proc. Int'l Conf. Green Computing and Communications},
  title     = {Energy Consumption and Efficiency in Mobile Applications: A User Feedback Study},
  year      = {2013},
  pages     = {134–141},
  publisher = {IEEE},
  numpages  = {8},
}

@InProceedings{M:SPLC17,
  author    = {Munoz, Daniel-Jesus},
  booktitle = {Proc. Int'l Conf. Systems and Software Product Line},
  title     = {Achieving energy efficiency using a software product line approach},
  year      = {2017},
  pages     = {131--138},
}

@InProceedings{BCO:ESECFSE15,
  author    = {Behrang, Farnaz and Cohen, Myra B. and Orso, Alessandro},
  booktitle = ESECFSE,
  title     = {Users Beware: Preference Inconsistencies Ahead},
  year      = {2015},
  address   = ACMAddr,
  month     = aug,
  pages     = {295–306},
  publisher = ACM,
  isbn      = {9781450336758},
  location  = {Bergamo, Italy},
  numpages  = {12},
}

@InProceedings{MNHBW:ICPC17,
  author    = {Melo, Jean and Narcizo, Fabricio Batista and Hansen, Dan Witzner and Brabrand, Claus and Wasowski, Andrzej},
  booktitle = {Proc. Int'l Conference Program Comprehension (ICPC)},
  title     = {Variability through the Eyes of the Programmer},
  year      = {2017},
  month     = may,
  pages     = {34–44},
  publisher = IEEE,
  location  = {Buenos Aires, Argentina},
  numpages  = {11},
}

@InProceedings{NS:PLDI07,
  author    = {Nethercote, Nicholas and Seward, Julian},
  booktitle = PLDI,
  title     = {Valgrind: A Framework for Heavyweight Dynamic Binary Instrumentation},
  year      = {2007},
  address   = ACMAddr,
  month     = jun,
  pages     = {89–100},
  publisher = ACM,
  location  = {San Diego, CA, USA},
  numpages  = {12},
}

@Online{VVM,
  lastaccessed = {November 24, 2020},
  title        = {VisualVM},
  url          = {https://visualvm.github.io/},
  year         = {2020},
}

@InProceedings{YP:ISSTA16,
  author    = {Yu, Tingting and Pradel, Michael},
  booktitle = ISSTA,
  title     = {SyncProf: Detecting, Localizing, and Optimizing Synchronization Bottlenecks},
  year      = {2016},
  address   = ACMAddr,
  month     = jul,
  pages     = {389–400},
  publisher = ACM,
  location  = {Saarbr\"{u}cken, Germany},
  numpages  = {12},
}

@InProceedings{ALZM:EUROSYS17,
  author    = {Alam, Mohammad Mejbah ul and Liu, Tongping and Zeng, Guangming and Muzahid, Abdullah},
  booktitle = {Proc. European Conference on Computer Systems (EuroSys)},
  title     = {SyncPerf: Categorizing, Detecting, and Diagnosing Synchronization Performance Bugs},
  year      = {2017},
  address   = ACMAddr,
  month     = apr,
  pages     = {298–313},
  publisher = ACM,
  isbn      = {9781450349383},
  location  = {Belgrade, Serbia},
  numpages  = {16},
}

@Article{H:CACM69,
  author    = {Hoare, C. A. R.},
  journal   = {Commun. ACM},
  title     = {An Axiomatic Basis for Computer Programming},
  year      = {1969},
  month     = oct,
  number    = {10},
  pages     = {576–580},
  volume    = {12},
  address   = ACMAddr,
  numpages  = {5},
  publisher = ACM,
}

@InCollection{BT:SMT18,
  author    = {Barrett, Clark and Tinelli, Cesare},
  booktitle = {Handbook of Model Checking},
  publisher = {Springer},
  title     = {Satisfiability modulo theories},
  year      = {2018},
  pages     = {305--343},
}

@Article{GPS:PS17,
  author    = {Gulwani, Sumit and Polozov, Oleksandr and Singh, Rishabh},
  journal   = {Foundations and Trends{\textregistered} in Programming Languages},
  title     = {Program synthesis},
  year      = {2017},
  number    = {1-2},
  pages     = {1--119},
  volume    = {4},
  publisher = {Now Publishers, Inc.},
}

@InProceedings{S:ASE07,
  author    = {Sen, Koushik},
  booktitle = ASE,
  title     = {Concolic testing},
  year      = {2007},
  month     = nov,
  pages     = {571--572},
}

@Book{CGKPV:MC18,
  author    = {Clarke Jr, Edmund M and Grumberg, Orna and Kroening, Daniel and Peled, Doron and Veith, Helmut},
  publisher = {MIT press},
  title     = {Model Checking},
  year      = {2018},
}

@Article{AH:ASP90,
  author    = {Agrawal, Hiralal and Horgan, Joseph R},
  journal   = {ACM SIGPlan Notices},
  title     = {Dynamic program slicing},
  year      = {1990},
  number    = {6},
  pages     = {246--256},
  volume    = {25},
  address   = ACMAddr,
  publisher = ACM,
}

@Article{KL:IPL88,
  author    = {Korel, Bogdan and Laski, Janusz},
  journal   = {Information processing letters},
  title     = {Dynamic program slicing},
  year      = {1988},
  number    = {3},
  pages     = {155--163},
  volume    = {29},
  publisher = {Elsevier},
}

@Article{XQZWC:SEN05,
  author    = {Xu, Baowen and Qian, Ju and Zhang, Xiaofang and Wu, Zhongqiang and Chen, Lin},
  journal   = {ACM SIGSOFT Software Engineering Notes},
  title     = {A brief survey of program slicing},
  year      = {2005},
  number    = {2},
  pages     = {1--36},
  volume    = {30},
  address   = ACMAddr,
  publisher = ACM,
}

@InProceedings{BPSZ:CSCW10,
  author    = {Breu, Silvia and Premraj, Rahul and Sillito, Jonathan and Zimmermann, Thomas},
  booktitle = {Proc. Conf. Computer Supported Cooperative Work (CSCW)},
  title     = {Information Needs in Bug Reports: Improving Cooperation between Developers and Users},
  year      = {2010},
  address   = ACMAddr,
  month     = feb,
  pages     = {301–310},
  publisher = ACM,
  location  = {Savannah, GA, USA},
  numpages  = {10},
}

@Article{SFPBBL:USENMT11,
  author = {Scaffidi, Chris and Fleming, Scott and Piorkowski, David and Burnett, Margaret and Bellamy, Rachel and Lawrance, Joseph},
  title  = {Unifying Software Engineering Methods and Tools: Principles and Patterns from Information Foraging},
  year   = {2011},
  month  = {05},
}

@Article{KMCA:TSE06,
  author    = {Ko, Andrew J. and Myers, Brad A. and Coblenz, Michael J. and Aung, Htet Htet},
  journal   = {IEEE Trans. Softw. Eng.},
  title     = {An Exploratory Study of How Developers Seek, Relate, and Collect Relevant Information during Software Maintenance Tasks},
  year      = {2006},
  issn      = {0098-5589},
  month     = dec,
  number    = {12},
  pages     = {971–987},
  volume    = {32},
  numpages  = {17},
  publisher = IEEE,
}

@InProceedings{LM:PLATEAU10,
  author    = {LaToza, Thomas D. and Myers, Brad A.},
  booktitle = {Evaluation and Usability of Programming Languages and Tools},
  title     = {Hard-to-Answer Questions about Code},
  year      = {2010},
  address   = ACMAddr,
  month     = oct,
  publisher = ACM,
  articleno = {8},
  location  = {Reno, NV, USA},
  numpages  = {6},
}

@Book{S:CMQR15,
  author    = {Salda{\~n}a, Johnny},
  publisher = {Sage},
  title     = {The coding manual for qualitative researchers},
  year      = {2015},
}

@Book{S:QCAP12,
  author    = {Schreier, Margrit},
  publisher = {Sage publications},
  title     = {Qualitative content analysis in practice},
  year      = {2012},
}

@InProceedings{LGHM:ESECFSE07,
  author    = {LaToza, Thomas D. and Garlan, David and Herbsleb, James D. and Myers, Brad A.},
  booktitle = ESECFSE,
  title     = {Program Comprehension as Fact Finding},
  year      = {2007},
  address   = ACMAddr,
  month     = sep,
  pages     = {361–370},
  publisher = ACM,
  location  = {Dubrovnik, Croatia},
  numpages  = {10},
}

@Manual{V:TP20,
  title        = {White-box Analysis for Modeling and Debugging the Performance of Configurable Systems},
  author       = {Miguel Velez},
  month        = dec,
  year         = {2020},
  howpublished = {Ph.D. Thesis Proposal},
  school       = {Carnegie Mellon Univesity},
}

@InProceedings{ABBDGKNNZ:ICSESEIP19,
  author    = {Amershi, Saleema and Begel, Andrew and Bird, Christian and DeLine, Robert and Gall, Harald and Kamar, Ece and Nagappan, Nachiappan and Nushi, Besmira and Zimmermann, Thomas},
  booktitle = {Proc. Int'l Conf. Software Engineering: Software Engineering in Practice},
  title     = {Software Engineering for Machine Learning: A Case Study},
  year      = {2019},
  month     = may,
  pages     = {291–300},
  publisher = IEEE,
  location  = {Montreal, Quebec, Canada},
  numpages  = {10},
}

@Misc{NKHK:ARXIV16,
  author        = {Besmira Nushi and Ece Kamar and Eric Horvitz and Donald Kossmann},
  title         = {On Human Intellect and Machine Failures: Troubleshooting Integrative Machine Learning Systems},
  year          = {2016},
  archiveprefix = {arXiv},
  eprint        = {1611.08309},
  primaryclass  = {cs.LG},
}

@InProceedings{LCLLV:ESECFSE17,
  author    = {Le, Xuan-Bach D. and Chu, Duc-Hiep and Lo, David and Le Goues, Claire and Visser, Willem},
  booktitle = {Proceedings of the 2017 11th Joint Meeting on Foundations of Software Engineering},
  title     = {S3: Syntax- and Semantic-Guided Repair Synthesis via Programming by Examples},
  year      = {2017},
  address   = ACMAddr,
  month     = aug,
  pages     = {593–604},
  publisher = ACM,
  location  = {Paderborn, Germany},
  numpages  = {12},
}

@Misc{VJSAK:ICSE21SM,
  author = {Velez, Miguel and Jamshidi, Pooyan and Siegmund, Norbert and Apel, Sven and Kästner, Christian},
  title  = {White-Box Analysis over Machine Learning: Modeling Performance of Configurable Systems - {S}upplementary {M}aterial - {https://bit.ly/3bbbgG8}},
  year   = {2021},
}

@Misc{KIJRJ:CADET20,
  author        = {Rahul Krishna and Md Shahriar Iqbal and Mohammad Ali Javidian and Baishakhi Ray and Pooyan Jamshidi},
  title         = {{CADET}: A Systematic Method For Debugging Misconfigurations using Counterfactual Reasoning},
  year          = {2020},
  archiveprefix = {arXiv},
  eprint        = {2010.06061},
  primaryclass  = {cs.SE},
}

@Book{S:SE10,
  author    = {Sommerville, Ian},
  publisher = {Addison-Wesley Publishing Company},
  title     = {Software Engineering},
  year      = {2010},
  address   = {USA},
  edition   = {9th},
  isbn      = {0137035152},
}

@InProceedings{KZDB:ICSE16,
  author    = {Kim, Miryung and Zimmermann, Thomas and DeLine, Robert and Begel, Andrew},
  booktitle = ICSE,
  title     = {The Emerging Role of Data Scientists on Software Development Teams},
  address   = ACMAddr,
  month     = may,
  pages     = {96–107},
  publisher = ACM,
  location  = {Austin, TX, USA},
  numpages  = {12},
}

@InProceedings{CCGWWH:PPOPP21,
  author    = {Copik, Marcin and Calotoiu, Alexandru and Grosser, Tobias and Wicki, Nicolas and Wolf, Felix and Hoefler, Torsten},
  booktitle = {Proc Symposium Principles and Practice of Parallel Programming (PPoPP)},
  title     = {Extracting Clean Performance Models from Tainted Programs},
  year      = {2021},
  address   = {ACMAddr},
  month     = feb,
  publisher = {ACM},
  location  = {Seoul, South Korea},
}

@InProceedings{WAS:ICSE21,
  author    = {Weber, Max and Apel, Sven and Siegmund, Norbert},
  booktitle = ICSE,
  title     = {White-Box Performance-Influence Models},
  year      = {2021},
  month     = may,
  publisher = IEEE,
  location  = {Madrid, Spain},
  numpages  = {11},
}

@InProceedings{VJSAK:ICSE21,
  author    = {Velez, Miguel and Jamshidi, Pooyan and Siegmund, Norbert and Apel, Sven and Kästner, Christian},
  booktitle = ICSE,
  title     = {White-Box Analysis over Machine Learning: Modeling Performance of Configurable Systems},
  year      = {2021},
  month     = may,
  publisher = IEEE,
  location  = {Madrid, Spain},
  numpages  = {11},
}

@Comment{jabref-meta: databaseType:bibtex;}

